Deep Learning in Mobile and Wireless Networking: A Survey

The rapid uptake of mobile devices and the rising popularity of mobile applications and services pose unprecedented demands on mobile and wireless networking infrastructure. Upcoming 5G systems are evolving to support exploding mobile traffic volumes, agile management of network resource to maximize user experience, and extraction of fine-grained real-time analytics. Fulfilling these tasks is challenging, as mobile environments are increasingly complex, heterogeneous, and evolving. One potential solution is to resort to advanced machine learning techniques to help managing the rise in data volumes and algorithm-driven applications. The recent success of deep learning underpins new and powerful tools that tackle problems in this space. In this paper we bridge the gap between deep learning and mobile and wireless networking research, by presenting a comprehensive survey of the crossovers between the two areas. We first briefly introduce essential background and state-of-the-art in deep learning techniques with potential applications to networking. We then discuss several techniques and platforms that facilitate the efficient deployment of deep learning onto mobile systems. Subsequently, we provide an encyclopedic review of mobile and wireless networking research based on deep learning, which we categorize by different domains. Drawing from our experience, we discuss how to tailor deep learning to mobile environments. We complete this survey by pinpointing current challenges and open future directions for research.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Communications Society subset of the full
IEEEtran package and is intended for use with IEEE Communications Society
publications. The included version of the IEEEtran_HOWTO.pdf has been
specially formatted in IEEE Communications Society (comsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf,
                   bare_jrnl_comsoc.tex.
***************************************************************************


==> ref.tex <==
\begin{thebibliography}{100}

\bibitem{cisco2017}
{Cisco}.
\newblock {Cisco Visual Networking Index: Forecast and Methodology, 2016-2021},
  June 2017.

\bibitem{wang2015backhauling}
Ning Wang, Ekram Hossain, and Vijay~K Bhargava.
\newblock Backhauling {5G} small cells: A radio resource management
  perspective.
\newblock {\em IEEE Wireless Communications}, 22(5):41--49, 2015.

\bibitem{giust2015distributed}
Fabio Giust, Luca Cominardi, and Carlos~J Bernardos.
\newblock Distributed mobility management for future {5G} networks: overview
  and analysis of existing approaches.
\newblock {\em IEEE Communications Magazine}, 53(1):142--149, 2015.

\bibitem{agiwal2016next}
Mamta Agiwal, Abhishek Roy, and Navrati Saxena.
\newblock Next generation {5G} wireless networks: A comprehensive survey.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 18(3):1617--1655,
  2016.

\bibitem{gupta2015survey}
Akhil Gupta and Rakesh~Kumar Jha.
\newblock A survey of {5G} network: Architecture and emerging technologies.
\newblock {\em IEEE access}, 3:1206--1232, 2015.

\bibitem{zheng2016big}
Kan Zheng, Zhe Yang, Kuan Zhang, Periklis Chatzimisios, Kan Yang, and Wei
  Xiang.
\newblock Big data-driven optimization for mobile networks toward {5G}.
\newblock {\em IEEE network}, 30(1):44--51, 2016.

\bibitem{jiang2017machine}
Chunxiao Jiang, Haijun Zhang, Yong Ren, Zhu Han, Kwang-Cheng Chen, and Lajos
  Hanzo.
\newblock Machine learning paradigms for next-generation wireless networks.
\newblock {\em IEEE Wireless Communications}, 24(2):98--105, 2017.

\bibitem{nguyen2017reinforcement}
Duong~D Nguyen, Hung~X Nguyen, and Langford~B White.
\newblock Reinforcement learning with network-assisted feedback for
  heterogeneous rat selection.
\newblock {\em IEEE Transactions on Wireless Communications}, 2017.

\bibitem{narudin2016evaluation}
Fairuz~Amalina Narudin, Ali Feizollah, Nor~Badrul Anuar, and Abdullah Gani.
\newblock Evaluation of machine learning classifiers for mobile malware
  detection.
\newblock {\em Soft Computing}, 20(1):343--357, 2016.

\bibitem{hsieh2017gaia}
Kevin Hsieh, Aaron Harlap, Nandita Vijaykumar, Dimitris Konomis, Gregory~R
  Ganger, Phillip~B Gibbons, and Onur Mutlu.
\newblock Gaia: Geo-distributed machine learning approaching {LAN} speeds.
\newblock In {\em USENIX Symposium on Networked Systems Design and
  Implementation (NSDI)}, pages 629--647, 2017.

\bibitem{xiao2017tux2}
Wencong Xiao, Jilong Xue, Youshan Miao, Zhen Li, Cheng Chen, Ming Wu, Wei Li,
  and Lidong Zhou.
\newblock Tux2: Distributed graph computation for machine learning.
\newblock In {\em USENIX Symposium on Networked Systems Design and
  Implementation (NSDI)}, pages 669--682, 2017.

\bibitem{anareport}
{Paolini, Monica and Fili, Senza }.
\newblock {Mastering Analytics: How to benefit from big data and network
  complexity: An Analyst Report}.
\newblock {\em RCR Wireless News}, 2017.

\bibitem{zhang2015convolutional}
{\color{black}Zhang, Chaoyun and Zhou, Pan and Li, Chenghua and Liu, Lijun}.
\newblock {\color{black}A convolutional neural network for leaves recognition
  using data augmentation}.
\newblock In {\em {\color{black}IEEE International Conference on Pervasive
  Intelligence and Computing (PICOM)}}, pages~{\color{black}2143--2150},
  {\color{black}2015}.

\bibitem{socher2012deep}
Richard Socher, Yoshua Bengio, and Christopher~D Manning.
\newblock Deep learning for {NLP} (without magic).
\newblock In {\em Tutorial Abstracts of ACL 2012}, pages 5--5. Association for
  Computational Linguistics.

\bibitem{specialissue}
{IEEE Network special issue: Exploring Deep Learning for Efficient and Reliable
  Mobile Sensing}.
\newblock
  \url{http://www.comsoc.org/netmag/cfp/exploring-deep-learning-efficient-and-reliable-mobile-sensing},
  2017.
\newblock [Online; accessed 14-July-2017].

\bibitem{wang2017machine}
Mowei Wang, Yong Cui, Xin Wang, Shihan Xiao, and Junchen Jiang.
\newblock Machine learning for networking: Workflow, advances and
  opportunities.
\newblock {\em IEEE Network}, 32(2):92--99, 2018.

\bibitem{alsheikh2016mobile}
Mohammad~Abu Alsheikh, Dusit Niyato, Shaowei Lin, Hwee-Pink Tan, and Zhu Han.
\newblock Mobile big data analytics using deep learning and {Apache Spark}.
\newblock {\em IEEE network}, 30(3):22--29, 2016.

\bibitem{goodfellow2016deep}
Ian Goodfellow, Yoshua Bengio, and Aaron Courville.
\newblock {\em Deep learning}.
\newblock MIT press, 2016.

\bibitem{mnih2015human}
Volodymyr Mnih, Koray Kavukcuoglu, David Silver, Andrei~A Rusu, Joel Veness,
  Marc~G Bellemare, Alex Graves, Martin Riedmiller, Andreas~K Fidjeland, Georg
  Ostrovski, et~al.
\newblock Human-level control through deep reinforcement learning.
\newblock {\em Nature}, 518(7540):529--533, 2015.

\bibitem{lecun2015deep}
Yann LeCun, Yoshua Bengio, and Geoffrey Hinton.
\newblock Deep learning.
\newblock {\em Nature}, 521(7553):436--444, 2015.

\bibitem{schmidhuber2015deep}
J{\"u}rgen Schmidhuber.
\newblock Deep learning in neural networks: {An} overview.
\newblock {\em Neural networks}, 61:85--117, 2015.

\bibitem{liu2017survey}
Weibo Liu, Zidong Wang, Xiaohui Liu, Nianyin Zeng, Yurong Liu, and Fuad~E
  Alsaadi.
\newblock A survey of deep neural network architectures and their applications.
\newblock {\em Neurocomputing}, 234:11--26, 2017.

\bibitem{deng2014deep}
Li~Deng, Dong Yu, et~al.
\newblock Deep learning: methods and applications.
\newblock {\em Foundations and Trends{\textregistered} in Signal Processing},
  7(3--4):197--387, 2014.

\bibitem{deng2014tutorial}
Li~Deng.
\newblock A tutorial survey of architectures, algorithms, and applications for
  deep learning.
\newblock {\em APSIPA Transactions on Signal and Information Processing}, 3,
  2014.

\bibitem{Pouyanfar:2018:SDL:3271482.3234150}
{\color{blue}Pouyanfar, Samira and Sadiq, Saad and Yan, Yilin and Tian, Haiman
  and Tao, Yudong and Reyes, Maria Presa and Shyu, Mei-Ling and Chen, Shu-Ching
  and Iyengar, S. S.}
\newblock {\color{blue}A Survey on Deep Learning: Algorithms, Techniques, and
  Applications}.
\newblock {\em {\color{blue}ACM Computing Surveys (CSUR)}},
  {\color{blue}51}({\color{blue}5}):{\color{blue}92:1--92:36},
  {\color{blue}2018}.

\bibitem{kai2017brief}
Kai Arulkumaran, Marc~Peter Deisenroth, Miles Brundage, and Anil~Anthony
  Bharath.
\newblock Deep reinforcement learning: A brief survey.
\newblock {\em IEEE Signal Processing Magazine}, 34(6):26--38, 2017.

\bibitem{hussein2017imitation}
\color{black}{Hussein, Ahmed and Gaber, Mohamed Medhat and Elyan, Eyad and
  Jayne, Chrisina}.
\newblock Imitation learning: A survey of learning methods.
\newblock {\em ACM Computing Surveys (CSUR)}, 50(2):21, 2017\color{black}.

\bibitem{chen2014big}
Xue-Wen Chen and Xiaotong Lin.
\newblock Big data deep learning: challenges and perspectives.
\newblock {\em IEEE access}, 2:514--525, 2014.

\bibitem{najafabadi2015deep}
Maryam~M Najafabadi, Flavio Villanustre, Taghi~M Khoshgoftaar, Naeem Seliya,
  Randall Wald, and Edin Muharemagic.
\newblock Deep learning applications and challenges in big data analytics.
\newblock {\em Journal of Big Data}, 2(1):1, 2015.

\bibitem{hordri2017systematic}
NF~Hordri, A~Samar, SS~Yuhaniz, and SM~Shamsuddin.
\newblock A systematic literature review on features of deep learning in big
  data analytics.
\newblock {\em International Journal of Advances in Soft Computing \& Its
  Applications}, 9(1), 2017.

\bibitem{gheisari2017survey}
Mehdi Gheisari, Guojun Wang, and Md~Zakirul~Alam Bhuiyan.
\newblock A survey on deep learning in big data.
\newblock In {\em IEEE International Conference on Computational Science and
  Engineering (CSE) and Embedded and Ubiquitous Computing (EUC)}, volume~2,
  pages 173--180, 2017.

\bibitem{zhang2017deep}
\color{black}{Zhang, Shuai and Yao, Lina and Sun, Aixin}.
\newblock Deep learning based recommender system: A survey and new
  perspectives.
\newblock {\em arXiv preprint arXiv:1707.07435}, 2017\color{black}.

\bibitem{yu2017networking}
Shui Yu, Meng Liu, Wanchun Dou, Xiting Liu, and Sanming Zhou.
\newblock Networking for big data: A survey.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 19(1):531--549, 2017.

\bibitem{alsheikh2014machine}
Mohammad~Abu Alsheikh, Shaowei Lin, Dusit Niyato, and Hwee-Pink Tan.
\newblock Machine learning in wireless sensor networks: Algorithms, strategies,
  and applications.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 16(4):1996--2018,
  2014.

\bibitem{tsai2014data}
Chun-Wei Tsai, Chin-Feng Lai, Ming-Chao Chiang, Laurence~T Yang, et~al.
\newblock Data mining for {Internet} of things: A survey.
\newblock {\em IEEE Communications Surveys and Tutorials}, 16(1):77--97, 2014.

\bibitem{cheng2017exploiting}
Xiang Cheng, Luoyang Fang, Xuemin Hong, and Liuqing Yang.
\newblock Exploiting mobile big data: Sources, features, and applications.
\newblock {\em IEEE Network}, 31(1):72--79, 2017.

\bibitem{bkassiny2013survey}
Mario Bkassiny, Yang Li, and Sudharman~K Jayaweera.
\newblock A survey on machine-learning techniques in cognitive radios.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 15(3):1136--1159,
  2013.

\bibitem{andrews2014will}
Jeffrey~G Andrews, Stefano Buzzi, Wan Choi, Stephen~V Hanly, Angel Lozano,
  Anthony~CK Soong, and Jianzhong~Charlie Zhang.
\newblock What will {5G} be?
\newblock {\em IEEE Journal on selected areas in communications},
  32(6):1065--1082, 2014.

\bibitem{panwar2016survey}
Nisha Panwar, Shantanu Sharma, and Awadhesh~Kumar Singh.
\newblock A survey on {5G}: The next generation of mobile communication.
\newblock {\em Physical Communication}, 18:64--84, 2016.

\bibitem{elijah2016comprehensive}
Olakunle Elijah, Chee~Yen Leow, Tharek~Abdul Rahman, Solomon Nunoo, and
  Solomon~Zakwoi Iliya.
\newblock A comprehensive survey of pilot contamination in massive {MIMO--5G}
  system.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 18(2):905--923, 2016.

\bibitem{buzzi2016survey}
Stefano Buzzi, I~Chih-Lin, Thierry~E Klein, H~Vincent Poor, Chenyang Yang, and
  Alessio Zappone.
\newblock A survey of energy-efficient techniques for {5G} networks and
  challenges ahead.
\newblock {\em IEEE Journal on Selected Areas in Communications},
  34(4):697--709, 2016.

\bibitem{peng2015system}
Mugen Peng, Yong Li, Zhongyuan Zhao, and Chonggang Wang.
\newblock System architecture and key technologies for {5G} heterogeneous cloud
  radio access networks.
\newblock {\em IEEE network}, 29(2):6--14, 2015.

\bibitem{niu2015survey}
Yong Niu, Yong Li, Depeng Jin, Li~Su, and Athanasios~V Vasilakos.
\newblock A survey of millimeter wave communications (mmwave) for {5G}:
  opportunities and challenges.
\newblock {\em Wireless Networks}, 21(8):2657--2676, 2015.

\bibitem{foukas2017network}
Xenofon Foukas, Georgios Patounas, Ahmed Elmokashfi, and Mahesh~K Marina.
\newblock Network slicing in {5G}: Survey and challenges.
\newblock {\em IEEE Communications Magazine}, 55(5):94--100, 2017.

\bibitem{taleb2017multi}
Tarik Taleb, Konstantinos Samdanis, Badr Mada, Hannu Flinck, Sunny Dutta, and
  Dario Sabella.
\newblock On multi-access edge computing: A survey of the emerging {5G} network
  edge architecture \& orchestration.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 2017.

\bibitem{mach2017mobile}
Pavel Mach and Zdenek Becvar.
\newblock Mobile edge computing: A survey on architecture and computation
  offloading.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 2017.

\bibitem{mao2017survey}
Yuyi Mao, Changsheng You, Jun Zhang, Kaibin Huang, and Khaled~B Letaief.
\newblock A survey on mobile edge computing: The communication perspective.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 2017.

\bibitem{wang2017data}
Ying Wang, Peilong Li, Lei Jiao, Zhou Su, Nan Cheng, Xuemin~Sherman Shen, and
  Ping Zhang.
\newblock A data-driven architecture for personalized {QoE} management in {5G}
  wireless networks.
\newblock {\em IEEE Wireless Communications}, 24(1):102--110, 2017.

\bibitem{han2015mobile}
Qilong Han, Shuang Liang, and Hongli Zhang.
\newblock Mobile cloud sensing, big data, and {5G} networks make an intelligent
  and smart world.
\newblock {\em IEEE Network}, 29(2):40--45, 2015.

\bibitem{singh2017survey}
Sukhdeep Singh, Navrati Saxena, Abhishek Roy, and HanSeok Kim.
\newblock A survey on {5G} network technologies from social perspective.
\newblock {\em IETE Technical Review}, 34(1):30--39, 2017.

\bibitem{chen20175g}
Min Chen, Jun Yang, Yixue Hao, Shiwen Mao, and Kai Hwang.
\newblock A {5G} cognitive system for healthcare.
\newblock {\em Big Data and Cognitive Computing}, 1(1):2, 2017.

\bibitem{chen2015energy}
\color{black}{Chen, Xianfu and Wu, Jinsong and Cai, Yueming and Zhang, Honggang
  and Chen, Tao}.
\newblock {Energy-efficiency oriented traffic offloading in wireless networks:
  A brief survey and a learning approach for heterogeneous cellular networks}.
\newblock {\em IEEE Journal on Selected Areas in Communications},
  33(4):627--640, {2015}\color{black}.

\bibitem{wu2016big}
\color{black}{Wu, Jinsong and Guo, Song and Li, Jie and Zeng, Deze}.
\newblock Big data meet green challenges: big data toward green applications.
\newblock {\em IEEE Systems Journal}, 10(3):888--900, 2016\color{black}.

\bibitem{buda2016can}
Teodora~Sandra Buda, Haytham Assem, Lei Xu, Danny Raz, Udi Margolin, Elisha
  Rosensweig, Diego~R Lopez, Marius-Iulian Corici, Mikhail Smirnov, Robert
  Mullins, et~al.
\newblock Can machine learning aid in delivering new use cases and scenarios in
  {5G}?
\newblock In {\em IEEE/IFIP Network Operations and Management Symposium
  (NOMS)}, pages 1279--1284, 2016.

\bibitem{imran2014challenges}
Ali Imran, Ahmed Zoha, and Adnan Abu-Dayya.
\newblock {Challenges in 5G: how to empower SON with big data for enabling 5G}.
\newblock {\em IEEE Network}, 28(6):27--33, 2014.

\bibitem{keshavamurthy2016conceptual}
Bharath Keshavamurthy and Mohammad Ashraf.
\newblock Conceptual design of proactive {SONs} based on the big data framework
  for {5G} cellular networks: A novel machine learning perspective facilitating
  a shift in the son paradigm.
\newblock In {\em IEEE International Conference on System Modeling \&
  Advancement in Research Trends (SMART)}, pages 298--304, 2016.

\bibitem{valente2017survey}
Paulo Valente~Klaine, Muhammad~Ali Imran, Oluwakayode Onireti, and Richard~Demo
  Souza.
\newblock A survey of machine learning techniques applied to self organizing
  cellular networks.
\newblock {\em IEEE Communications Surveys and Tutorials}, 2017.

\bibitem{li2017intelligent}
Rongpeng Li, Zhifeng Zhao, Xuan Zhou, Guoru Ding, Yan Chen, Zhongyao Wang, and
  Honggang Zhang.
\newblock Intelligent {5G}: When cellular networks meet artificial
  intelligence.
\newblock {\em IEEE Wireless communications}, 24(5):175--183, 2017.

\bibitem{bui2017survey}
Nicola Bui, Matteo Cesana, S~Amir Hosseini, Qi~Liao, Ilaria Malanchini, and
  Joerg Widmer.
\newblock A survey of anticipatory mobile networking: Context-based
  classification, prediction methodologies, and optimization techniques.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 19(3):1790--1821,
  2017.

\bibitem{kasnesis2017changing}
Panagiotis Kasnesis, Charalampos Patrikakis, and Iakovos Venieris.
\newblock Changing the game of mobile data analysis with deep learning.
\newblock {\em IT Professional}, 2017.

\bibitem{cheng2017mobile}
Xiang Cheng, Luoyang Fang, Liuqing Yang, and Shuguang Cui.
\newblock Mobile big data: the fuel for data-driven wireless.
\newblock {\em IEEE Internet of Things Journal}, 4(5):1489--1516, 2017.

\bibitem{wang2017big}
Lidong Wang and Randy Jones.
\newblock Big data analytics for network intrusion detection: A survey.
\newblock {\em International Journal of Networks and Communications},
  7(1):24--31, 2017.

\bibitem{kato2017deep}
Nei Kato, Zubair~Md Fadlullah, Bomin Mao, Fengxiao Tang, Osamu Akashi, Takeru
  Inoue, and Kimihiro Mizutani.
\newblock The deep learning vision for heterogeneous network traffic control:
  proposal, challenges, and future perspective.
\newblock {\em IEEE Wireless Communications}, 24(3):146--153, 2017.

\bibitem{zorzi2015cognition}
Michele Zorzi, Andrea Zanella, Alberto Testolin, Michele De~Filippo De~Grazia,
  and Marco Zorzi.
\newblock Cognition-based networks: A new perspective on network optimization
  using learning and distributed intelligence.
\newblock {\em IEEE Access}, 3:1512--1530, 2015.

\bibitem{fadlullah2017state}
Zubair Fadlullah, Fengxiao Tang, Bomin Mao, Nei Kato, Osamu Akashi, Takeru
  Inoue, and Kimihiro Mizutani.
\newblock State-of-the-art deep learning: Evolving machine intelligence toward
  tomorrow's intelligent network traffic control systems.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 19(4):2432--2455,
  2017.

\bibitem{mohammadi2018deep}
\color{black}{Mohammadi, Mehdi and Al-Fuqaha, Ala and Sorour, Sameh and
  Guizani, Mohsen}.
\newblock {Deep Learning for IoT Big Data and Streaming Analytics: A Survey}.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 2018\color{black}.

\bibitem{ahad2016neural}
Nauman Ahad, Junaid Qadir, and Nasir Ahsan.
\newblock Neural networks in wireless networks: Techniques, applications and
  guidelines.
\newblock {\em Journal of Network and Computer Applications}, 68:1--27, 2016.

\bibitem{mao2018deep}
\color{black}{Mao, Qian and Hu, Fei and Hao, Qi}.
\newblock Deep learning for intelligent wireless networks: A comprehensive
  survey.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 2018\color{black}.

\bibitem{luong2018applications}
{\color{blue}Luong, Nguyen Cong and Hoang, Dinh Thai and Gong, Shimin and
  Niyato, Dusit and Wang, Ping and Liang, Ying-Chang and Kim, Dong In}.
\newblock {\color{blue}Applications of Deep Reinforcement Learning in
  Communications and Networking: A Survey}.
\newblock {\em {\color{blue}arXiv preprint arXiv:1810.07862}},
  {\color{blue}2018}.

\bibitem{zhou2017intelligent2}
\color{black}{Zhou, Xiangwei and Sun, Mingxuan and Li, Ye Geoffrey and Juang,
  Biing-Hwang}.
\newblock {Intelligent Wireless Communications Enabled by Cognitive Radio and
  Machine Learning}.
\newblock {\em arXiv preprint arXiv:1710.11240}, 2017\color{black}.

\bibitem{chen2017machine2}
\color{black}{Chen, Mingzhe and Challita, Ursula and Saad, Walid and Yin,
  Changchuan and Debbah, M{\'e}rouane}.
\newblock Machine learning for wireless networks with artificial intelligence:
  A tutorial on neural networks.
\newblock {\em arXiv preprint arXiv:1710.02913}, 2017\color{black}.

\bibitem{gharaibeh2017smart}
Ammar Gharaibeh, Mohammad~A Salahuddin, Sayed~Jahed Hussini, Abdallah
  Khreishah, Issa Khalil, Mohsen Guizani, and Ala Al-Fuqaha.
\newblock Smart cities: A survey on data management, security, and enabling
  technologies.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 19(4):2456--2501,
  2017.

\bibitem{lane2015can}
Nicholas~D Lane and Petko Georgiev.
\newblock Can deep learning revolutionize mobile sensing?
\newblock In {\em Proceedings of the 16th ACM International Workshop on Mobile
  Computing Systems and Applications}, pages 117--122, 2015.

\bibitem{ota2017deep}
Kaoru Ota, Minh~Son Dao, Vasileios Mezaris, and Francesco~GB De~Natale.
\newblock Deep learning for mobile multimedia: A survey.
\newblock {\em ACM Transactions on Multimedia Computing, Communications, and
  Applications (TOMM)}, 13(3s):34, 2017.

\bibitem{mishra2018detailed}
\color{black}{Mishra, Preeti and Varadharajan, Vijay and Tupakula, Uday and
  Pilli, Emmanuel S}.
\newblock A detailed investigation and analysis of using machine learning
  techniques for intrusion detection.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 2018\color{black}.

\bibitem{li2017deeprl}
Yuxi Li.
\newblock Deep reinforcement learning: An overview.
\newblock {\em arXiv preprint arXiv:1701.07274}, 2017.

\bibitem{chen2018deep0}
Longbiao Chen, Dingqi Yang, Daqing Zhang, Cheng Wang, Jonathan Li, et~al.
\newblock Deep mobile traffic forecast and complementary base station
  clustering for {C-RAN} optimization.
\newblock {\em Journal of Network and Computer Applications}, 121:59--69, 2018.

\bibitem{mnih2016asynchronous}
Volodymyr Mnih, Adria~Puigdomenech Badia, Mehdi Mirza, Alex Graves, Timothy
  Lillicrap, Tim Harley, David Silver, and Koray Kavukcuoglu.
\newblock Asynchronous methods for deep reinforcement learning.
\newblock In {\em International Conference on Machine Learning (ICML)}, pages
  1928--1937, 2016.

\bibitem{arjovsky2017wasserstein}
Martin Arjovsky, Soumith Chintala, and L{\'e}on Bottou.
\newblock Wasserstein generative adversarial networks.
\newblock In {\em International Conference on Machine Learning}, pages
  214--223, 2017.

\bibitem{damianou2013deep2}
\color{black}{Damianou, Andreas and Lawrence, Neil}.
\newblock Deep {Gaussian} processes.
\newblock In {\em Artificial Intelligence and Statistics}, pages 207--215,
  2013\color{black}.

\bibitem{garnelo2018neural}
\color{black}{Garnelo, Marta and Schwarz, Jonathan and Rosenbaum, Dan and
  Viola, Fabio and Rezende, Danilo J and Eslami, SM and Teh, Yee Whye}.
\newblock Neural processes.
\newblock {\em arXiv preprint arXiv:1807.01622}, 2018\color{black}.

\bibitem{zhou2017deep2}
\color{black}{Zhou, Zhi-Hua and Feng, Ji}.
\newblock Deep forest: towards an alternative to deep neural networks.
\newblock In {\em Proceedings of the 26th International Joint Conference on
  Artificial Intelligence}, pages 3553--3559. AAAI Press, 2017\color{black}.

\bibitem{mcculloch:1943}
W.~McCulloch and W.~Pitts.
\newblock A logical calculus of the ideas immanent in nervous activity.
\newblock {\em Bulletin of Mathematical Biophysics}, (5).

\bibitem{williams1986learning}
David~E Rumelhart, Geoffrey~E Hinton, and Ronald~J Williams.
\newblock Learning representations by back-propagating errors.
\newblock {\em Nature}, 323(6088):533, 1986.

\bibitem{lecun1995convolutional}
Yann LeCun, Yoshua Bengio, et~al.
\newblock Convolutional networks for images, speech, and time series.
\newblock {\em The handbook of brain theory and neural networks},
  3361(10):1995, 1995.

\bibitem{krizhevsky2012imagenet}
Alex Krizhevsky, Ilya Sutskever, and Geoffrey~E Hinton.
\newblock Imagenet classification with deep convolutional neural networks.
\newblock In {\em Advances in neural information processing systems}, pages
  1097--1105, 2012.

\bibitem{Domingos:2012}
Pedro Domingos.
\newblock A few useful things to know about machine learning.
\newblock {\em Communications of the ACM}, 55(10):78--87, 2012.

\bibitem{tsang2005core}
Ivor~W Tsang, James~T Kwok, and Pak-Ming Cheung.
\newblock {Core vector machines: Fast {SVM} training on very large data sets}.
\newblock {\em Journal of Machine Learning Research}, 6:363--392, 2005.

\bibitem{rasmussen2006gaussian}
Carl~Edward Rasmussen and Christopher~KI Williams.
\newblock {\em Gaussian processes for machine learning}, volume~1.
\newblock MIT press Cambridge, 2006.

\bibitem{le2008representational}
Nicolas Le~Roux and Yoshua Bengio.
\newblock Representational power of restricted boltzmann machines and deep
  belief networks.
\newblock {\em Neural computation}, 20(6):1631--1649, 2008.

\bibitem{goodfellow2014generative}
Ian Goodfellow, Jean Pouget-Abadie, Mehdi Mirza, Bing Xu, David Warde-Farley,
  Sherjil Ozair, Aaron Courville, and Yoshua Bengio.
\newblock Generative adversarial nets.
\newblock In {\em Advances in neural information processing systems}, pages
  2672--2680, 2014.

\bibitem{schroff2015facenet}
Florian Schroff, Dmitry Kalenichenko, and James Philbin.
\newblock Facenet: A unified embedding for face recognition and clustering.
\newblock In {\em Proceedings of the IEEE Conference on Computer Vision and
  Pattern Recognition}, pages 815--823, 2015.

\bibitem{kingma2014semi}
Diederik~P Kingma, Shakir Mohamed, Danilo~Jimenez Rezende, and Max Welling.
\newblock Semi-supervised learning with deep generative models.
\newblock In {\em Advances in Neural Information Processing Systems}, pages
  3581--3589, 2014.

\bibitem{stewart2017label}
Russell Stewart and Stefano Ermon.
\newblock Label-free supervision of neural networks with physics and domain
  knowledge.
\newblock In {\em National Conference on Artificial Intelligence (AAAI)}, pages
  2576--2582, 2017.

\bibitem{rezende2016one}
Danilo Rezende, Ivo Danihelka, Karol Gregor, Daan Wierstra, et~al.
\newblock One-shot generalization in deep generative models.
\newblock In {\em International Conference on Machine Learning (ICML)}, pages
  1521--1529, 2016.

\bibitem{socher2013zero}
Richard Socher, Milind Ganjoo, Christopher~D Manning, and Andrew Ng.
\newblock Zero-shot learning through cross-modal transfer.
\newblock In {\em Advances in neural information processing systems}, pages
  935--943, 2013.

\bibitem{georgiev2017low}
Petko Georgiev, Sourav Bhattacharya, Nicholas~D Lane, and Cecilia Mascolo.
\newblock Low-resource multi-task audio sensing for mobile and embedded devices
  via shared deep neural network representations.
\newblock {\em Proceedings of the ACM on Interactive, Mobile, Wearable and
  Ubiquitous Technologies}, 1(3):50, 2017.

\bibitem{monti2017geometric}
{\color{blue}Monti, Federico and Boscaini, Davide and Masci, Jonathan and
  Rodola, Emanuele and Svoboda, Jan and Bronstein, Michael M}.
\newblock {\color{blue}Geometric deep learning on graphs and manifolds using
  mixture model {CNNs}}.
\newblock In {\em {\color{blue}IEEE Conference on Computer Vision and Pattern
  Recognition (CVPR)}}, volume~{\color{blue}1}, page~{\color{blue}3},
  {\color{blue}2017}.

\bibitem{le2004geometric}
{\color{blue}Le Roux, Brigitte and Rouanet, Henry}.
\newblock {\em {\color{blue}Geometric data analysis: from correspondence
  analysis to structured data analysis}}.
\newblock {\color{blue}Springer Science \& Business Media}, {\color{blue}2004}.

\bibitem{qi2017pointnet}
{\color{blue}Qi, Charles Ruizhongtai and Yi, Li and Su, Hao and Guibas,
  Leonidas J}.
\newblock {\color{blue}Pointnet++: Deep hierarchical feature learning on point
  sets in a metric space}.
\newblock In {\em {\color{blue}Advances in Neural Information Processing
  Systems}}, pages~{\color{blue}5099--5108}, {\color{blue}2017}.

\bibitem{kipf2016semi}
{\color{blue}Kipf, Thomas N and Welling, Max}.
\newblock {\color{blue}Semi-supervised classification with graph convolutional
  networks}.
\newblock {\em {\color{blue}International Conference on Learning
  Representations (ICLR)}}, {\color{blue}2017}.

\bibitem{wang2018spatio}
{\color{blue}Wang, Xu and Zhou, Zimu and Xiao, Fu and Xing, Kai and Yang, Zheng
  and Liu, Yunhao and Peng, Chunyi}.
\newblock {\color{blue}Spatio-temporal analysis and prediction of cellular
  traffic in metropolis}.
\newblock {\em {\color{blue}IEEE Transactions on Mobile Computing}},
  {\color{blue}2018}.

\bibitem{nguyen2015deep}
{\color{blue}Nguyen, Anh and Yosinski, Jason and Clune, Jeff}.
\newblock {\color{blue}Deep neural networks are easily fooled: High confidence
  predictions for unrecognizable images}.
\newblock In {\em {\color{blue}Proceedings of the IEEE Conference on Computer
  Vision and Pattern Recognition}}, pages~{\color{blue}427--436},
  {\color{blue}2015}.

\bibitem{behzadan2017vulnerability}
{\color{blue}Behzadan, Vahid and Munir, Arslan}.
\newblock {\color{blue}Vulnerability of deep reinforcement learning to policy
  induction attacks}.
\newblock In {\em {\color{blue}International Conference on Machine Learning and
  Data Mining in Pattern Recognition}}, pages~{\color{blue}262--275}.
  {\color{blue}Springer}, {\color{blue}2017}.

\bibitem{madani2018robustness}
{\color{blue}Madani, Pooria and Vlajic, Natalija}.
\newblock {\color{blue}Robustness of deep autoencoder in intrusion detection
  under adversarial contamination}.
\newblock In {\em {\color{blue}Proceedings of the 5th ACM Annual Symposium and
  Bootcamp on Hot Topics in the Science of Security}}, page~{\color{blue}1},
  {\color{blue}2018}.

\bibitem{bau2017network}
{\color{blue}Bau, David and Zhou, Bolei and Khosla, Aditya and Oliva, Aude and
  Torralba, Antonio}.
\newblock {\color{blue}Network Dissection: Quantifying Interpretability of Deep
  Visual Representations}.
\newblock In {\em {\color{blue}IEEE Conference on Computer Vision and Pattern
  Recognition (CVPR)}}, pages~{\color{blue}3319--3327}, {\color{blue}2017}.

\bibitem{wu2017beyond}
{\color{blue}Wu, Mike and Hughes, Michael C and Parbhoo, Sonali and Zazzi,
  Maurizio and Roth, Volker and Doshi-Velez, Finale}.
\newblock {\color{blue}Beyond sparsity: Tree regularization of deep models for
  interpretability}.
\newblock {\color{blue}2018}.

\bibitem{chakraborty2017interpretability}
{\color{blue}Chakraborty, Supriyo and Tomsett, Richard and Raghavendra, Ramya
  and Harborne, Daniel and Alzantot, Moustafa and Cerutti, Federico and
  Srivastava, Mani and Preece, Alun and Julier, Simon and Rao, Raghuveer M and
  others}.
\newblock {\color{blue}Interpretability of deep learning models: a survey of
  results}.
\newblock In {\em {\color{blue}IEEE Smart World Congress 2017 Workshop: DAIS}},
  {\color{blue}2017}.

\bibitem{perez2017effectiveness}
{\color{blue}Perez, Luis and Wang, Jason}.
\newblock {\color{blue}The effectiveness of data augmentation in image
  classification using deep learning}.
\newblock {\em {\color{blue}arXiv preprint arXiv:1712.04621}},
  {\color{blue}2017}.

\bibitem{liu2017progressive}
\color{black}{Liu, Chenxi and Zoph, Barret and Shlens, Jonathon and Hua, Wei
  and Li, Li-Jia and Fei-Fei, Li and Yuille, Alan and Huang, Jonathan and
  Murphy, Kevin}.
\newblock Progressive neural architecture search.
\newblock {\em arXiv preprint arXiv:1712.00559}, 2017\color{black}.

\bibitem{zhang2016deep3}
Wei Zhang, Kan Liu, Weidong Zhang, Youmei Zhang, and Jason Gu.
\newblock Deep neural networks for wireless localization in indoor and outdoor
  environments.
\newblock {\em Neurocomputing}, 194:279--287, 2016.

\bibitem{ordonez2016deep}
Francisco~Javier Ord{\'o}{\~n}ez and Daniel Roggen.
\newblock Deep convolutional and {LSTM} recurrent neural networks for
  multimodal wearable activity recognition.
\newblock {\em Sensors}, 16(1):115, 2016.

\bibitem{de2016distributed}
Elias De~Coninck, Tim Verbelen, Bert Vankeirsbilck, Steven Bohez, Pieter
  Simoens, Piet Demeester, and Bart Dhoedt.
\newblock Distributed neural networks for {Internet of Things}: the big-little
  approach.
\newblock In {\em Internet of Things. IoT Infrastructures: Second International
  Summit, IoT 360$^{\circ}$ 2015, Rome, Italy, October 27-29, Revised Selected
  Papers, Part II}, pages 484--492. Springer, 2016.

\bibitem{jouppi2017datacenter}
Norman~P Jouppi, Cliff Young, Nishant Patil, David Patterson, Gaurav Agrawal,
  Raminder Bajwa, Sarah Bates, Suresh Bhatia, Nan Boden, Al~Borchers, et~al.
\newblock In-datacenter performance analysis of a tensor processing unit.
\newblock In {\em ACM/IEEE 44th Annual International Symposium on Computer
  Architecture (ISCA)}, pages 1--12, 2017.

\bibitem{nickolls2008scalable}
John Nickolls, Ian Buck, Michael Garland, and Kevin Skadron.
\newblock Scalable parallel programming with {CUDA}.
\newblock {\em Queue}, 6(2):40--53, 2008.

\bibitem{chetlur2014cudnn}
Sharan Chetlur, Cliff Woolley, Philippe Vandermersch, Jonathan Cohen, John
  Tran, Bryan Catanzaro, and Evan Shelhamer.
\newblock {cuDNN}: Efficient primitives for deep learning.
\newblock {\em arXiv preprint arXiv:1410.0759}, 2014.

\bibitem{tensorflow2015-whitepaper}
Mart{\'\i}n Abadi, Paul Barham, Jianmin Chen, Zhifeng Chen, Andy Davis, Jeffrey
  Dean, Matthieu Devin, Sanjay Ghemawat, Geoffrey Irving, Michael Isard, et~al.
\newblock {TensorFlow}: A system for large-scale machine learning.
\newblock In {\em USENIX Symposium on Operating Systems Design and
  Implementation (OSDI)}, volume~16, pages 265--283, 2016.

\bibitem{2016arXiv160502688short}
{Theano Development Team}.
\newblock {Theano: A {Python} framework for fast computation of mathematical
  expressions}.
\newblock {\em arXiv e-prints}, abs/1605.02688, May 2016.

\bibitem{jia2014caffe}
Yangqing Jia, Evan Shelhamer, Jeff Donahue, Sergey Karayev, Jonathan Long, Ross
  Girshick, Sergio Guadarrama, and Trevor Darrell.
\newblock Caffe: Convolutional architecture for fast feature embedding.
\newblock {\em arXiv preprint arXiv:1408.5093}, 2014.

\bibitem{torch}
R.~Collobert, K.~Kavukcuoglu, and C.~Farabet.
\newblock Torch7: A {Matlab}-like environment for machine learning.
\newblock In {\em BigLearn, NIPS Workshop}, 2011.

\bibitem{gokhale2014240}
Vinayak Gokhale, Jonghoon Jin, Aysegul Dundar, Berin Martini, and Eugenio
  Culurciello.
\newblock A 240 {G}-ops/s mobile coprocessor for deep neural networks.
\newblock In {\em Proceedings of the IEEE Conference on Computer Vision and
  Pattern Recognition Workshops}, pages 682--687, 2014.

\bibitem{ncnn}
{ncnn is a high-performance neural network inference framework optimized for
  the mobile platform }.
\newblock \url{https://github.com/Tencent/ncnn}, 2017.
\newblock [Online; accessed 25-July-2017].

\bibitem{huawei2017kirin}
{Huawei announces the {Kirin} 970- new flagship {SoC} with {AI} capabilities}.
\newblock
  \url{http://www.androidauthority.com/huawei-announces-kirin-970-797788/},
  2017.
\newblock [Online; accessed 01-Sep-2017].

\bibitem{coreml}
{Core ML: Integrate machine learning models into your app.}
\newblock \url{https://developer.apple.com/documentation/coreml}, 2017.
\newblock [Online; accessed 25-July-2017].

\bibitem{sutskever2013importance}
Ilya Sutskever, James Martens, George~E Dahl, and Geoffrey~E Hinton.
\newblock On the importance of initialization and momentum in deep learning.
\newblock {\em Proceedings of the international conference on machine learning
  (ICML)}, 28:1139--1147, 2013.

\bibitem{dean2012large}
Jeffrey Dean, Greg Corrado, Rajat Monga, Kai Chen, Matthieu Devin, Mark Mao,
  Andrew Senior, Paul Tucker, Ke~Yang, Quoc~V Le, et~al.
\newblock Large scale distributed deep networks.
\newblock In {\em Advances in neural information processing systems}, pages
  1223--1231, 2012.

\bibitem{kingma2015adam}
Diederik Kingma and Jimmy Ba.
\newblock {Adam: A method for stochastic optimization}.
\newblock {\em International Conference on Learning Representations (ICLR)},
  2015.

\bibitem{kraska2013mlbase}
Tim Kraska, Ameet Talwalkar, John~C Duchi, Rean Griffith, Michael~J Franklin,
  and Michael~I Jordan.
\newblock {MLbase}: A distributed machine-learning system.
\newblock In {\em CIDR}, volume~1, pages 2--1, 2013.

\bibitem{chilimbi2014project}
Trishul~M Chilimbi, Yutaka Suzue, Johnson Apacible, and Karthik Kalyanaraman.
\newblock Project adam: Building an efficient and scalable deep learning
  training system.
\newblock In {\em USENIX Symposium on Operating Systems Design and
  Implementation (OSDI)}, volume~14, pages 571--582, 2014.

\bibitem{cui2016geeps}
Henggang Cui, Hao Zhang, Gregory~R Ganger, Phillip~B Gibbons, and Eric~P Xing.
\newblock Geeps: Scalable deep learning on distributed {GPUs} with a
  {GPU}-specialized parameter server.
\newblock In {\em Proceedings of the Eleventh ACM European Conference on
  Computer Systems}, page~4, 2016.

\bibitem{Lineaat8084}
\color{black}{Lin, Xing and Rivenson, Yair and Yardimci, Nezih T. and Veli,
  Muhammed and Luo, Yi and Jarrahi, Mona and Ozcan, Aydogan}.
\newblock All-optical machine learning using diffractive deep neural networks.
\newblock {\em Science}, 2018\color{black}.

\bibitem{spring2017scalable}
Ryan Spring and Anshumali Shrivastava.
\newblock Scalable and sustainable deep learning via randomized hashing.
\newblock {\em ACM SIGKDD Conference on Knowledge Discovery and Data Mining},
  2017.

\bibitem{mirhoseini2017device}
Azalia Mirhoseini, Hieu Pham, Quoc~V Le, Benoit Steiner, Rasmus Larsen, Yuefeng
  Zhou, Naveen Kumar, Mohammad Norouzi, Samy Bengio, and Jeff Dean.
\newblock Device placement optimization with reinforcement learning.
\newblock {\em International Conference on Machine Learning}, 2017.

\bibitem{xing2015petuum}
Eric~P Xing, Qirong Ho, Wei Dai, Jin~Kyu Kim, Jinliang Wei, Seunghak Lee, Xun
  Zheng, Pengtao Xie, Abhimanu Kumar, and Yaoliang Yu.
\newblock Petuum: A new platform for distributed machine learning on big data.
\newblock {\em IEEE Transactions on Big Data}, 1(2):49--67, 2015.

\bibitem{moritz2018ray}
{\color{blue}Moritz, Philipp and Nishihara, Robert and Wang, Stephanie and
  Tumanov, Alexey and Liaw, Richard and Liang, Eric and Elibol, Melih and Yang,
  Zongheng and Paul, William and Jordan, Michael I and others}.
\newblock {\color{blue}Ray: A Distributed Framework for Emerging {AI}
  Applications}.
\newblock In {\em {\color{blue}13th USENIX Symposium on Operating Systems
  Design and Implementation (OSDI 18)}}, pages~{\color{blue}561--577},
  {\color{blue}2018}.

\bibitem{alzantot2017rstensorflow}
Moustafa Alzantot, Yingnan Wang, Zhengshuang Ren, and Mani~B Srivastava.
\newblock {RSTensorFlow}: {GPU} enabled tensorflow for deep learning on
  commodity {Android} devices.
\newblock In {\em Proceedings of the 1st ACM International Workshop on Deep
  Learning for Mobile Systems and Applications}, pages 7--12, 2017.

\bibitem{tensorlayer}
Hao Dong, Akara Supratak, Luo Mai, Fangde Liu, Axel Oehmichen, Simiao Yu, and
  Yike Guo.
\newblock {TensorLayer}: A versatile library for efficient deep learning
  development.
\newblock In {\em Proceedings of the ACM on Multimedia Conference}, MM '17,
  pages 1201--1204, 2017.

\bibitem{paszke2017automatic}
Adam Paszke, Sam Gross, Soumith Chintala, Gregory Chanan, Edward Yang, Zachary
  DeVito, Zeming Lin, Alban Desmaison, Luca Antiga, and Adam Lerer.
\newblock Automatic differentiation in {PyTorch}.
\newblock 2017.

\bibitem{chen2015mxnet}
Tianqi Chen, Mu~Li, Yutian Li, Min Lin, Naiyan Wang, Minjie Wang, Tianjun Xiao,
  Bing Xu, Chiyuan Zhang, and Zheng Zhang.
\newblock Mxnet: A flexible and efficient machine learning library for
  heterogeneous distributed systems.
\newblock {\em arXiv preprint arXiv:1512.01274}, 2015.

\bibitem{ruder2016overview}
Sebastian Ruder.
\newblock An overview of gradient descent optimization algorithms.
\newblock {\em arXiv preprint arXiv:1609.04747}, 2016.

\bibitem{zeiler2012adadelta}
\color{black}{Zeiler, Matthew D}.
\newblock {ADADELTA}: an adaptive learning rate method.
\newblock {\em arXiv preprint arXiv:1212.5701}, 2012\color{black}.

\bibitem{dozat2016incorporating}
\color{black}{Dozat, Timothy}.
\newblock Incorporating {Nesterov} momentum into {Adam}.
\newblock 2016\color{black}.

\bibitem{andrychowicz2016learning}
Marcin Andrychowicz, Misha Denil, Sergio Gomez, Matthew~W Hoffman, David Pfau,
  Tom Schaul, and Nando de~Freitas.
\newblock Learning to learn by gradient descent by gradient descent.
\newblock In {\em Advances in Neural Information Processing Systems}, pages
  3981--3989, 2016.

\bibitem{szegedy2015going}
Christian Szegedy, Wei Liu, Yangqing Jia, Pierre Sermanet, Scott Reed, Dragomir
  Anguelov, Dumitru Erhan, Vincent Vanhoucke, and Andrew Rabinovich.
\newblock Going deeper with convolutions.
\newblock In {\em Proceedings of the IEEE conference on computer vision and
  pattern recognition}, pages 1--9, 2015.

\bibitem{stable2018zhou}
\color{black} {Zhou, Yingxue and Chen, Sheng and Banerjee, Arindam}.
\newblock Stable gradient descent.
\newblock In {\em Conference on Uncertainty in Artificial Intelligence},
  2018\color{black}.

\bibitem{wen2017terngrad}
Wei Wen, Cong Xu, Feng Yan, Chunpeng Wu, Yandan Wang, Yiran Chen, and Hai Li.
\newblock {TernGrad}: Ternary gradients to reduce communication in distributed
  deep learning.
\newblock In {\em Advances in neural information processing systems}, 2017.

\bibitem{bonomi2014fog}
Flavio Bonomi, Rodolfo Milito, Preethi Natarajan, and Jiang Zhu.
\newblock Fog computing: A platform for internet of things and analytics.
\newblock In {\em Big Data and Internet of Things: A Roadmap for Smart
  Environments}, pages 169--186. Springer, 2014.

\bibitem{mao2017modnn}
Jiachen Mao, Xiang Chen, Kent~W Nixon, Christopher Krieger, and Yiran Chen.
\newblock {MoDNN}: Local distributed mobile computing system for deep neural
  network.
\newblock In {\em IEEE Design, Automation \& Test in Europe Conference \&
  Exhibition (DATE)}, pages 1396--1401, 2017.

\bibitem{mukherjee2018survey}
\color{black}{Mukherjee, Mithun and Shu, Lei and Wang, Di}.
\newblock Survey of fog computing: Fundamental, network applications, and
  research challenges.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 2018\color{black}.

\bibitem{vaquero2014finding}
\color{black}{Vaquero, Luis M and Rodero-Merino, Luis}.
\newblock Finding your way in the fog: Towards a comprehensive definition of
  fog computing.
\newblock {\em ACM SIGCOMM Computer Communication Review}, 44(5):27--32,
  2014\color{black}.

\bibitem{aazam2018offloading}
{\color{blue}Aazam, Mohammad and Zeadally, Sherali and Harras, Khaled A}.
\newblock {\color{blue}Offloading in fog computing for {IoT}: Review, enabling
  technologies, and research opportunities}.
\newblock {\em {\color{blue}Future Generation Computer Systems}},
  {\color{blue}87}:{\color{blue}278--289}, {\color{blue}2018}.

\bibitem{Buyya2018Manifesto}
{\color{blue}Buyya, Rajkumar and Srirama, Satish Narayana and Casale, Giuliano
  and Calheiros, Rodrigo and Simmhan, Yogesh and Varghese, Blesson and Gelenbe,
  Erol and Javadi, Bahman and Vaquero, Luis Miguel and Netto, Marco A. S. and
  Toosi, Adel Nadjaran and Rodriguez, Maria Alejandra and Llorente, Ignacio M.
  and Vimercati, Sabrina De Capitani Di and Samarati, Pierangela and Milojicic,
  Dejan and Varela, Carlos and Bahsoon, Rami and Assuncao, Marcos Dias De and
  Rana, Omer and Zhou, Wanlei and Jin, Hai and Gentzsch, Wolfgang and Zomaya,
  Albert Y. and Shen, Haiying}.
\newblock {\color{blue}A Manifesto for Future Generation Cloud Computing:
  Research Directions for the Next Decade}.
\newblock {\em {\color{blue}ACM Computing Survey}},
  {\color{blue}51}({\color{blue}5}):{\color{blue}105:1--105:38}.

\bibitem{sze2017efficient}
{\color{blue}Sze, Vivienne and Chen, Yu-Hsin and Yang, Tien-Ju and Emer, Joel
  S}.
\newblock {\color{blue}Efficient processing of deep neural networks: A tutorial
  and survey}.
\newblock {\em {\color{blue}Proceedings of the IEEE}},
  {\color{blue}105}({\color{blue}12}):{\color{blue}2295--2329},
  {\color{blue}2017}.

\bibitem{bang201714}
Suyoung Bang, Jingcheng Wang, Ziyun Li, Cao Gao, Yejoong Kim, Qing Dong, Yen-Po
  Chen, Laura Fick, Xun Sun, Ron Dreslinski, et~al.
\newblock 14.7 a 288$\mu$w programmable deep-learning processor with 270kb
  on-chip weight storage using non-uniform memory hierarchy for mobile
  intelligence.
\newblock In {\em IEEE International Conference on Solid-State Circuits
  (ISSCC)}, pages 250--251, 2017.

\bibitem{akopyan2016design}
Filipp Akopyan.
\newblock Design and tool flow of {IBM}'s truenorth: an ultra-low power
  programmable neurosynaptic chip with 1 million neurons.
\newblock In {\em Proceedings of the International Symposium on Physical
  Design}, pages 59--60. ACM, 2016.

\bibitem{latifi2016cnndroid}
Seyyed~Salar Latifi~Oskouei, Hossein Golestani, Matin Hashemi, and Soheil
  Ghiasi.
\newblock Cnndroid: {GPU}-accelerated execution of trained deep convolutional
  neural networks on {A}ndroid.
\newblock In {\em Proceedings of the ACM on Multimedia Conference}, pages
  1201--1205, 2016.

\bibitem{cortes2017adanet}
Corinna Cortes, Xavi Gonzalvo, Vitaly Kuznetsov, Mehryar Mohri, and Scott Yang.
\newblock Adanet: Adaptive structural learning of artificial neural networks.
\newblock {\em International Conference on Machine Learning (ICML)}, 2017.

\bibitem{hinton2006fast}
Geoffrey~E Hinton, Simon Osindero, and Yee-Whye Teh.
\newblock A fast learning algorithm for deep belief nets.
\newblock {\em Neural computation}, 18(7):1527--1554, 2006.

\bibitem{lee2009convolutional}
Honglak Lee, Roger Grosse, Rajesh Ranganath, and Andrew~Y Ng.
\newblock Convolutional deep belief networks for scalable unsupervised learning
  of hierarchical representations.
\newblock In {\em Proceedings of the 26th ACM annual international conference
  on machine learning}, pages 609--616, 2009.

\bibitem{vincent2010stacked}
Pascal Vincent, Hugo Larochelle, Isabelle Lajoie, Yoshua Bengio, and
  Pierre-Antoine Manzagol.
\newblock Stacked denoising autoencoders: Learning useful representations in a
  deep network with a local denoising criterion.
\newblock {\em Journal of Machine Learning Research}, 11(Dec):3371--3408, 2010.

\bibitem{kingma2014auto}
Diederik~P Kingma and Max Welling.
\newblock {Auto-encoding variational bayes}.
\newblock {\em International Conference on Learning Representations (ICLR)},
  2014.

\bibitem{he2016deep}
Kaiming He, Xiangyu Zhang, Shaoqing Ren, and Jian Sun.
\newblock Deep residual learning for image recognition.
\newblock In {\em Proceedings of the IEEE conference on computer vision and
  pattern recognition}, pages 770--778, 2016.

\bibitem{ji20133d}
Shuiwang Ji, Wei Xu, Ming Yang, and Kai Yu.
\newblock {3D} convolutional neural networks for human action recognition.
\newblock {\em IEEE transactions on pattern analysis and machine intelligence},
  35(1):221--231, 2013.

\bibitem{huang2017densely}
Gao Huang, Zhuang Liu, Kilian~Q Weinberger, and Laurens van~der Maaten.
\newblock Densely connected convolutional networks.
\newblock {\em IEEE Conference on Computer Vision and Pattern Recognition},
  2017.

\bibitem{gers1999learning}
Felix~A Gers, J{\"u}rgen Schmidhuber, and Fred Cummins.
\newblock Learning to forget: Continual prediction with {LSTM}.
\newblock 1999.

\bibitem{sutskever2014sequence}
Ilya Sutskever, Oriol Vinyals, and Quoc~V Le.
\newblock Sequence to sequence learning with neural networks.
\newblock In {\em Advances in neural information processing systems}, pages
  3104--3112, 2014.

\bibitem{xingjian2015convolutional}
Shi Xingjian, Zhourong Chen, Hao Wang, Dit-Yan Yeung, Wai-Kin Wong, and
  Wang-chun Woo.
\newblock Convolutional {LSTM} network: A machine learning approach for
  precipitation nowcasting.
\newblock In {\em Advances in neural information processing systems}, pages
  802--810, 2015.

\bibitem{qi2017loss}
Guo-Jun Qi.
\newblock Loss-sensitive generative adversarial networks on {Lipschitz}
  densities.
\newblock {\em arXiv preprint arXiv:1701.06264}, 2017.

\bibitem{brock2018large}
{\color{blue}Brock, Andrew and Donahue, Jeff and Simonyan, Karen}.
\newblock {\color{blue}Large scale {GAN} training for high fidelity natural
  image synthesis}.
\newblock {\em {\color{blue}arXiv preprint arXiv:1809.11096}},
  {\color{blue}2018}.

\bibitem{silver2016mastering}
David Silver, Aja Huang, Chris~J Maddison, Arthur Guez, Laurent Sifre, George
  Van Den~Driessche, Julian Schrittwieser, Ioannis Antonoglou, Veda
  Panneershelvam, Marc Lanctot, et~al.
\newblock Mastering the game of {Go} with deep neural networks and tree search.
\newblock {\em Nature}, 529(7587):484--489, 2016.

\bibitem{hessel2017rainbow}
\color{black}{Hessel, Matteo and Modayil, Joseph and Van Hasselt, Hado and
  Schaul, Tom and Ostrovski, Georg and Dabney, Will and Horgan, Dan and Piot,
  Bilal and Azar, Mohammad and Silver, David}.
\newblock Rainbow: Combining improvements in deep reinforcement learning.
\newblock 2017\color{black}.

\bibitem{schulman2017proximal}
\color{black}{Schulman, John and Wolski, Filip and Dhariwal, Prafulla and
  Radford, Alec and Klimov, Oleg}.
\newblock Proximal policy optimization algorithms.
\newblock {\em arXiv preprint arXiv:1707.06347}, 2017\color{black}.

\bibitem{collobert2004links}
Ronan Collobert and Samy Bengio.
\newblock Links between perceptrons, {MLP}s and {SVM}s.
\newblock In {\em Proceedings of the twenty-first ACM international conference
  on Machine learning}, page~23, 2004.

\bibitem{glorot2011deep}
booktitle={Proceedings of the fourteenth international conference on artificial
  intelligence and statistics} \color{black}{Glorot, Xavier and Bordes, Antoine
  and Bengio, Yoshua}.
\newblock Deep sparse rectifier neural networks.
\newblock pages 315--323, 2011\color{black}.

\bibitem{klambauer2017self}
\color{black}{Klambauer, G{\"u}nter and Unterthiner, Thomas and Mayr, Andreas
  and Hochreiter, Sepp}.
\newblock Self-normalizing neural networks.
\newblock In {\em Advances in Neural Information Processing Systems}, pages
  971--980, 2017\color{black}.

\bibitem{ioffe2015batch}
{\color{blue}Ioffe, Sergey and Szegedy, Christian}.
\newblock {\color{blue}Batch Normalization: Accelerating Deep Network Training
  by Reducing Internal Covariate Shift}.
\newblock In {\em {\color{blue}Proceedings of the International Conference on
  Machine Learning}}, pages~{\color{blue}448--456}, {\color{blue}2015}.

\bibitem{hinton2002training}
Geoffrey~E Hinton.
\newblock Training products of experts by minimizing contrastive divergence.
\newblock {\em Neural computation}, 14(8):1771--1800, 2002.

\bibitem{casella1992explaining}
George Casella and Edward~I George.
\newblock Explaining the {Gibbs} sampler.
\newblock {\em The American Statistician}, 46(3):167--174, 1992.

\bibitem{kuremoto2014forecast}
Takashi Kuremoto, Masanao Obayashi, Kunikazu Kobayashi, Takaomi Hirata, and
  Shingo Mabu.
\newblock Forecast chaotic time series data by {DBNs}.
\newblock In {\em 7th IEEE International Congress on Image and Signal
  Processing (CISP)}, pages 1130--1135, 2014.

\bibitem{dauphin2013stochastic}
Yann Dauphin and Yoshua Bengio.
\newblock Stochastic ratio matching of {RBMs} for sparse high-dimensional
  inputs.
\newblock In {\em Advances in Neural Information Processing Systems}, pages
  1340--1348, 2013.

\bibitem{sainath2011making}
Tara~N Sainath, Brian Kingsbury, Bhuvana Ramabhadran, Petr Fousek, Petr Novak,
  and Abdel-rahman Mohamed.
\newblock Making deep belief networks effective for large vocabulary continuous
  speech recognition.
\newblock In {\em IEEE Workshop on Automatic Speech Recognition and
  Understanding (ASRU)}, pages 30--35, 2011.

\bibitem{bengio2009learning}
Yoshua Bengio et~al.
\newblock Learning deep architectures for {AI}.
\newblock {\em Foundations and trends{\textregistered} in Machine Learning},
  2(1):1--127, 2009.

\bibitem{sakurada2014anomaly}
Mayu Sakurada and Takehisa Yairi.
\newblock Anomaly detection using autoencoders with nonlinear dimensionality
  reduction.
\newblock In {\em Proceedings Workshop on Machine Learning for Sensory Data
  Analysis (MLSDA)}, page~4. ACM, 2014.

\bibitem{nicolau2016hybrid}
Miguel Nicolau, James McDermott, et~al.
\newblock A hybrid autoencoder and density estimation model for anomaly
  detection.
\newblock In {\em International Conference on Parallel Problem Solving from
  Nature}, pages 717--726. Springer, 2016.

\bibitem{thing2017ieee}
Vrizlynn~LL Thing.
\newblock {IEEE} 802.11 network anomaly detection and attack classification: A
  deep learning approach.
\newblock In {\em IEEE Wireless Communications and Networking Conference
  (WCNC)}, pages 1--6, 2017.

\bibitem{mao2017routing}
Bomin Mao, Zubair~Md Fadlullah, Fengxiao Tang, Nei Kato, Osamu Akashi, Takeru
  Inoue, and Kimihiro Mizutani.
\newblock Routing or computing? the paradigm shift towards intelligent computer
  network packet transmission based on deep learning.
\newblock {\em IEEE Transactions on Computers}, 66(11):1946--1960, 2017.

\bibitem{radu2016towards}
Valentin Radu, Nicholas~D Lane, Sourav Bhattacharya, Cecilia Mascolo, Mahesh~K
  Marina, and Fahim Kawsar.
\newblock Towards multimodal deep learning for activity recognition on mobile
  devices.
\newblock In {\em Proceedings of ACM International Joint Conference on
  Pervasive and Ubiquitous Computing: Adjunct}, pages 185--188, 2016.

\bibitem{radu2018multimodal}
Valentin Radu, Catherine Tong, Sourav Bhattacharya, Nicholas~D Lane, Cecilia
  Mascolo, Mahesh~K Marina, and Fahim Kawsar.
\newblock Multimodal deep learning for activity and context recognition.
\newblock {\em Proceedings of the ACM on Interactive, Mobile, Wearable and
  Ubiquitous Technologies}, 1(4):157, 2018.

\bibitem{raghavendra2016learning}
Ramachandra Raghavendra and Christoph Busch.
\newblock Learning deeply coupled autoencoders for smartphone based robust
  periocular verification.
\newblock In {\em IEEE International Conference on Image Processing (ICIP)},
  pages 325--329, 2016.

\bibitem{li2016wavelet}
Jing Li, Jingyuan Wang, and Zhang Xiong.
\newblock Wavelet-based stacked denoising autoencoders for cell phone base
  station user number prediction.
\newblock In {\em IEEE International Conference on Internet of Things (iThings)
  and IEEE Green Computing and Communications (GreenCom) and IEEE Cyber,
  Physical and Social Computing (CPSCom) and IEEE Smart Data (SmartData)},
  pages 833--838, 2016.

\bibitem{ILSVRC15}
Olga Russakovsky, Jia Deng, Hao Su, Jonathan Krause, Sanjeev Satheesh, Sean Ma,
  Zhiheng Huang, Andrej Karpathy, Aditya Khosla, Michael Bernstein,
  Alexander~C. Berg, and Li~Fei-Fei.
\newblock {ImageNet Large Scale Visual Recognition Challenge}.
\newblock {\em International Journal of Computer Vision (IJCV)},
  115(3):211--252, 2015.

\bibitem{active2017yunho}
Junmo~Kim Yunho~Jeon.
\newblock Active convolution: Learning the shape of convolution for image
  classification.
\newblock In {\em Proceedings of the IEEE Conference on Computer Vision and
  Pattern Recognition}, 2017.

\bibitem{dai2017deformable}
Jifeng Dai, Haozhi Qi, Yuwen Xiong, Yi~Li, Guodong Zhang, Han Hu, and Yichen
  Wei.
\newblock Deformable convolutional networks.
\newblock In {\em Proceedings of the IEEE International Conference on Computer
  Vision}, pages 764--773, 2017.

\bibitem{Zhu2018morel}
{\color{blue}Zhu, Xizhou and Hu, Han and Lin, Stephen and Dai, Jifeng}.
\newblock {\color{blue}Deformable ConvNets v2: More Deformable, Better
  Results}.
\newblock {\em {\color{blue}arXiv preprint arXiv:1811.11168}},
  {\color{blue}2018}.

\bibitem{bengio1994learning}
Yoshua Bengio, Patrice Simard, and Paolo Frasconi.
\newblock Learning long-term dependencies with gradient descent is difficult.
\newblock {\em IEEE transactions on neural networks}, 5(2):157--166, 1994.

\bibitem{graves2013hybrid}
Alex Graves, Navdeep Jaitly, and Abdel-rahman Mohamed.
\newblock Hybrid speech recognition with deep bidirectional {LSTM}.
\newblock In {\em IEEE Workshop on Automatic Speech Recognition and
  Understanding (ASRU)}, pages 273--278, 2013.

\bibitem{johnson2016supervised}
Rie Johnson and Tong Zhang.
\newblock Supervised and semi-supervised text categorization using {LSTM} for
  region embeddings.
\newblock In {\em International Conference on Machine Learning (ICML)}, pages
  526--534, 2016.

\bibitem{goodfellow2016nips}
{\color{blue}Goodfellow, Ian}.
\newblock {\color{blue}{NIPS} 2016 tutorial: Generative adversarial networks}.
\newblock {\em {\color{blue}arXiv preprint arXiv:1701.00160}},
  {\color{blue}2016}.

\bibitem{ledig2017photo}
Christian Ledig, Lucas Theis, Ferenc Husz{\'a}r, Jose Caballero, Andrew
  Cunningham, Alejandro Acosta, Andrew Aitken, Alykhan Tejani, Johannes Totz,
  Zehan Wang, et~al.
\newblock Photo-realistic single image super-resolution using a generative
  adversarial network.
\newblock In {\em IEEE Conference on Computer Vision and Pattern Recognition},
  2017.

\bibitem{li2017perceptual}
Jianan Li, Xiaodan Liang, Yunchao Wei, Tingfa Xu, Jiashi Feng, and Shuicheng
  Yan.
\newblock Perceptual generative adversarial networks for small object
  detection.
\newblock In {\em IEEE Conference on Computer Vision and Pattern Recognition},
  2017.

\bibitem{li2017generative}
Yijun Li, Sifei Liu, Jimei Yang, and Ming-Hsuan Yang.
\newblock Generative face completion.
\newblock In {\em IEEE Conference on Computer Vision and Pattern Recognition},
  2017.

\bibitem{gawlowicz2018ns3}
{\color{blue}Gaw{\l}owicz, Piotr and Zubow, Anatolij}.
\newblock {\color{blue}{NS3-Gym}: Extending {OpenAI Gym} for Networking
  Research}.
\newblock {\em {\color{blue}arXiv preprint arXiv:1810.03943}},
  {\color{blue}2018}.

\bibitem{gu2016continuous}
Shixiang Gu, Timothy Lillicrap, Ilya Sutskever, and Sergey Levine.
\newblock Continuous deep {Q}-learning with model-based acceleration.
\newblock In {\em International Conference on Machine Learning}, pages
  2829--2838, 2016.

\bibitem{moravvcik2017deepstack}
Matej Morav{\v{c}}{\'\i}k, Martin Schmid, Neil Burch, Viliam Lis{\`y}, Dustin
  Morrill, Nolan Bard, Trevor Davis, Kevin Waugh, Michael Johanson, and Michael
  Bowling.
\newblock Deepstack: Expert-level artificial intelligence in heads-up no-limit
  poker.
\newblock {\em Science}, 356(6337):508--513, 2017.

\bibitem{levine2016learning}
Sergey Levine, Peter Pastor, Alex Krizhevsky, Julian Ibarz, and Deirdre
  Quillen.
\newblock Learning hand-eye coordination for robotic grasping with deep
  learning and large-scale data collection.
\newblock {\em The International Journal of Robotics Research},
  37(4-5):421--436, 2018.

\bibitem{sallab2017deep}
Ahmad~EL Sallab, Mohammed Abdou, Etienne Perot, and Senthil Yogamani.
\newblock Deep reinforcement learning framework for autonomous driving.
\newblock {\em Electronic Imaging}, (19):70--76, 2017.

\bibitem{li2014tact}
Rongpeng Li, Zhifeng Zhao, Xianfu Chen, Jacques Palicot, and Honggang Zhang.
\newblock Tact: A transfer actor-critic learning framework for energy saving in
  cellular radio access networks.
\newblock {\em IEEE Transactions on Wireless Communications}, 13(4):2000--2011,
  2014.

\bibitem{al2015application}
Hasan~AA Al-Rawi, Ming~Ann Ng, and Kok-Lim~Alvin Yau.
\newblock Application of reinforcement learning to routing in distributed
  wireless networks: a review.
\newblock {\em Artificial Intelligence Review}, 43(3):381--416, 2015.

\bibitem{liu2015reinforcement}
Yan-Jun Liu, Li~Tang, Shaocheng Tong, CL~Philip Chen, and Dong-Juan Li.
\newblock Reinforcement learning design-based adaptive tracking control with
  less learning parameters for nonlinear discrete-time {MIMO} systems.
\newblock {\em IEEE Transactions on Neural Networks and Learning Systems},
  26(1):165--176, 2015.

\bibitem{pierucci2016neural}
Laura Pierucci and Davide Micheli.
\newblock A neural network for quality of experience estimation in mobile
  communications.
\newblock {\em IEEE MultiMedia}, 23(4):42--49, 2016.

\bibitem{gwon2014inferring}
Youngjune~L Gwon and HT~Kung.
\newblock Inferring origin flow patterns in wi-fi with deep learning.
\newblock In {\em 11th IEEE International Conference on Autonomic Computing
  (ICAC))}, pages 73--83, 2014.

\bibitem{nie2017network}
Laisen Nie, Dingde Jiang, Shui Yu, and Houbing Song.
\newblock Network traffic prediction based on deep belief network in wireless
  mesh backbone networks.
\newblock In {\em Wireless Communications and Networking Conference (WCNC),
  IEEE}, pages 1--5, 2017.

\bibitem{moyo2015generalization}
Vusumuzi Moyo et~al.
\newblock The generalization ability of artificial neural networks in
  forecasting {TCP/IP} traffic trends: How much does the size of learning rate
  matter?
\newblock {\em International Journal of Computer Science and Application},
  2015.

\bibitem{wangspatiotemporal}
Jing Wang, Jian Tang, Zhiyuan Xu, Yanzhi Wang, Guoliang Xue, Xing Zhang, and
  Dejun Yang.
\newblock Spatiotemporal modeling and prediction in cellular networks: A big
  data enabled deep learning approach.
\newblock In {\em 36th Annual IEEE International Conference on Computer
  Communications (INFOCOM)}, 2017.

\bibitem{zhang2017long}
Chaoyun Zhang and Paul Patras.
\newblock Long-term mobile traffic forecasting using deep spatio-temporal
  neural networks.
\newblock In {\em Proceedings of the Eighteenth ACM International Symposium on
  Mobile Ad Hoc Networking and Computing}, pages 231--240, 2018.

\bibitem{chaoyun2017zipnet}
Chaoyun Zhang, Xi~Ouyang, and Paul Patras.
\newblock {ZipNet-GAN}: Inferring fine-grained mobile traffic patterns via a
  generative adversarial neural network.
\newblock In {\em Proceedings of the 13th ACM Conference on Emerging Networking
  Experiments and Technologies}, 2017.

\bibitem{huang2017study}
\color{black}{Huang, Chih-Wei and Chiang, Chiu-Ti and Li, Qiuhui}.
\newblock A study of deep learning networks on mobile traffic forecasting.
\newblock In {\em 28th IEEE Annual International Symposium on Personal, Indoor,
  and Mobile Radio Communications (PIMRC)}, pages 1--6, 2017\color{black}.

\bibitem{zhang2018citywide}
\color{black}{Zhang, Chuanting and Zhang, Haixia and Yuan, Dongfeng and Zhang,
  Minggao}.
\newblock Citywide cellular traffic prediction based on densely connected
  convolutional neural networks.
\newblock {\em IEEE Communications Letters}, 2018\color{black}.

\bibitem{navabi2018predicting}
\color{black}{Navabi, Shiva and Wang, Chenwei and Bursalioglu, Ozgun Y and
  Papadopoulos, Haralabos}.
\newblock Predicting wireless channel features using neural networks.
\newblock {\em arXiv preprint arXiv:1802.00107}, 2018\color{black}.

\bibitem{wang2015applications}
Zhanyi Wang.
\newblock The applications of deep learning on traffic identification.
\newblock {\em BlackHat USA}, 2015.

\bibitem{wang2017end}
Wei Wang, Ming Zhu, Jinlin Wang, Xuewen Zeng, and Zhongzhen Yang.
\newblock End-to-end encrypted traffic classification with one-dimensional
  convolution neural networks.
\newblock In {\em IEEE International Conference on Intelligence and Security
  Informatics (ISI)}, pages 43--48, 2017.

\bibitem{lotfollahi2017deep}
Mohammad Lotfollahi, Ramin Shirali, Mahdi~Jafari Siavoshani, and Mohammdsadegh
  Saberian.
\newblock Deep packet: A novel approach for encrypted traffic classification
  using deep learning.
\newblock {\em arXiv preprint arXiv:1709.02656}, 2017.

\bibitem{wang2017malware}
Wei Wang, Ming Zhu, Xuewen Zeng, Xiaozhou Ye, and Yiqiang Sheng.
\newblock Malware traffic classification using convolutional neural network for
  representation learning.
\newblock In {\em IEEE International Conference on Information Networking
  (ICOIN)}, pages 712--717, 2017.

\bibitem{liang2016mercury}
Victor~C Liang, Richard~TB Ma, Wee~Siong Ng, Li~Wang, Marianne Winslett, Huayu
  Wu, Shanshan Ying, and Zhenjie Zhang.
\newblock Mercury: Metro density prediction with recurrent neural network on
  streaming {CDR} data.
\newblock In {\em IEEE 32nd International Conference on Data Engineering
  (ICDE)}, pages 1374--1377, 2016.

\bibitem{felbo2016using}
Bjarke Felbo, P{\aa}l Sunds{\o}y, Alex'Sandy' Pentland, Sune Lehmann, and
  Yves-Alexandre de~Montjoye.
\newblock Using deep learning to predict demographics from mobile phone
  metadata.
\newblock {\em workshop track of the International Conference on Learning
  Representations (ICLR)}, 2016.

\bibitem{chen2017comprehensive}
Nai~Chun Chen, Wanqin Xie, Roy~E Welsch, Kent Larson, and Jenny Xie.
\newblock Comprehensive predictions of tourists' next visit location based on
  call detail records using machine learning and deep learning methods.
\newblock In {\em IEEE International Congress on Big Data (BigData Congress)},
  pages 1--6, 2017.

\bibitem{lin2017deep}
Ziheng Lin, Mogeng Yin, Sidney Feygin, Madeleine Sheehan, Jean-Francois
  Paiement, and Alexei Pozdnoukhov.
\newblock Deep generative models of urban mobility.
\newblock {\em IEEE Transactions on Intelligent Transportation Systems}, 2017.

\bibitem{xu2017large}
Chang Xu, Kuiyu Chang, Khee-Chin Chua, Meishan Hu, and Zhenxiang Gao.
\newblock Large-scale {Wi-Fi} hotspot classification via deep learning.
\newblock In {\em Proceedings of the 26th International Conference on World
  Wide Web Companion}, pages 857--858. International World Wide Web Conferences
  Steering Committee, 2017.

\bibitem{meng2018qoe}
Qianyu Meng, Kun Wang, Bo~Liu, Toshiaki Miyazaki, and Xiaoming He.
\newblock {QoE}-based big data analysis with deep learning in pervasive edge
  environment.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018.

\bibitem{fang2018mobile}
{\color{blue}Fang, Luoyang and Cheng, Xiang and Wang, Haonan and Yang,
  Liuqing}.
\newblock {\color{blue}Mobile Demand Forecasting via Deep Graph-Sequence
  Spatiotemporal Modeling in Cellular Networks}.
\newblock {\em {\color{blue}IEEE Internet of Things Journal}},
  {\color{blue}2018}.

\bibitem{luo2018channel}
{\color{blue}Luo, Changqing and Ji, Jinlong and Wang, Qianlong and Chen, Xuhui
  and Li, Pan}.
\newblock {\color{blue}Channel state information prediction for {5G} wireless
  communications: A deep learning approach}.
\newblock {\em {\color{blue}IEEE Transactions on Network Science and
  Engineering}}, {\color{blue}2018}.

\bibitem{8553650}
{\color{blue}Li, Peng and Chen, Zhikui and Yang, Laurence T. and Gao, Jing and
  Zhang, Qingchen and Deen, M. Jamal }.
\newblock {\color{blue}An Improved Stacked Auto-Encoder for Network Traffic
  Flow Classification}.
\newblock {\em {\color{blue}IEEE Network}},
  {\color{blue}32}({\color{blue}6}):{\color{blue}22--27}, {\color{blue}2018}.

\bibitem{feng2018deeptp}
{\color{blue}Feng, Jie and Chen, Xinlei and Gao, Rundong and Zeng, Ming and Li,
  Yong}.
\newblock {\color{blue}{DeepTP}: An End-to-End Neural Network for Mobile
  Cellular Traffic Prediction}.
\newblock {\em {\color{blue}IEEE Network}},
  {\color{blue}32}({\color{blue}6}):{\color{blue}108--115}, {\color{blue}2018}.

\bibitem{zhu2018deep}
{\color{blue}Zhu, Hao and Cao, Yang and Wang, Wei and Jiang, Tao and Jin, Shi}.
\newblock {\color{blue}Deep Reinforcement Learning for Mobile Edge Caching:
  Review, New Features, and Open Issues}.
\newblock {\em {\color{blue}IEEE Network}},
  {\color{blue}32}({\color{blue}6}):{\color{blue}50--57}, {\color{blue}2018}.

\bibitem{liu2016poster}
Sicong Liu and Junzhao Du.
\newblock Poster: Mobiear-building an environment-independent acoustic sensing
  platform for the deaf using deep learning.
\newblock In {\em Proceedings of the 14th ACM Annual International Conference
  on Mobile Systems, Applications, and Services Companion}, pages 50--50, 2016.

\bibitem{sicong2017ubiear}
Liu Sicong, Zhou Zimu, Du~Junzhao, Shangguan Longfei, Jun Han, and Xin Wang.
\newblock Ubiear: Bringing location-independent sound awareness to the
  hard-of-hearing people with smartphones.
\newblock {\em Proceedings of the ACM on Interactive, Mobile, Wearable and
  Ubiquitous Technologies}, 1(2):17, 2017.

\bibitem{jindal2016integrating}
Vasu Jindal.
\newblock Integrating mobile and cloud for {PPG} signal selection to monitor
  heart rate during intensive physical exercise.
\newblock In {\em Proceedings of the ACM International Workshop on Mobile
  Software Engineering and Systems}, pages 36--37, 2016.

\bibitem{kim2016deep}
Edward Kim, Miguel Corte-Real, and Zubair Baloch.
\newblock A deep semantic mobile application for thyroid cytopathology.
\newblock In {\em Medical Imaging 2016: PACS and Imaging Informatics: Next
  Generation and Innovations}, volume 9789, page 97890A. International Society
  for Optics and Photonics, 2016.

\bibitem{sathyanarayana2016sleep}
Aarti Sathyanarayana, Shafiq Joty, Luis Fernandez-Luque, Ferda Ofli, Jaideep
  Srivastava, Ahmed Elmagarmid, Teresa Arora, and Shahrad Taheri.
\newblock Sleep quality prediction from wearable data using deep learning.
\newblock {\em JMIR mHealth and uHealth}, 4(4), 2016.

\bibitem{li2017personal}
Honggui Li and Maria Trocan.
\newblock Personal health indicators by deep learning of smart phone sensor
  data.
\newblock In {\em 3rd IEEE International Conference on Cybernetics (CYBCONF)},
  pages 1--5, 2017.

\bibitem{hosseini2017deep}
Mohammad-Parsa Hosseini, Tuyen~X Tran, Dario Pompili, Kost Elisevich, and Hamid
  Soltanian-Zadeh.
\newblock Deep learning with edge computing for localization of
  epileptogenicity using multimodal rs-{fMRI} and {EEG} big data.
\newblock In {\em IEEE International Conference on Autonomic Computing (ICAC)},
  pages 83--92, 2017.

\bibitem{stamate2017deep}
Cosmin Stamate, George~D Magoulas, Stefan K{\"u}ppers, Effrosyni Nomikou,
  Ioannis Daskalopoulos, Marco~U Luchini, Theano Moussouri, and George Roussos.
\newblock Deep learning parkinson's from smartphone data.
\newblock In {\em IEEE International Conference on Pervasive Computing and
  Communications (PerCom)}, pages 31--40, 2017.

\bibitem{quisel2017collecting}
Tom Quisel, Luca Foschini, Alessio Signorini, and David~C Kale.
\newblock Collecting and analyzing millions of mhealth data streams.
\newblock In {\em Proceedings of the 23rd ACM SIGKDD International Conference
  on Knowledge Discovery and Data Mining}, pages 1971--1980, 2017.

\bibitem{khan2017deep}
Usman~Mahmood Khan, Zain Kabir, Syed~Ali Hassan, and Syed~Hassan Ahmed.
\newblock A deep learning framework using passive {WiFi} sensing for
  respiration monitoring.
\newblock In {\em Global Communications Conference (GLOBECOM)}, pages 1--6.
  IEEE, 2017.

\bibitem{li2016deepcham}
Dawei Li, Theodoros Salonidis, Nirmit~V Desai, and Mooi~Choo Chuah.
\newblock Deepcham: Collaborative edge-mediated adaptive deep learning for
  mobile object recognition.
\newblock In {\em IEEE/ACM Symposium on Edge Computing (SEC)}, pages 64--76,
  2016.

\bibitem{tobias2016convolutional}
Luis Tob{\'\i}as, Aur{\'e}lien Ducournau, Fran{\c{c}}ois Rousseau, Gr{\'e}goire
  Mercier, and Ronan Fablet.
\newblock Convolutional neural networks for object recognition on mobile
  devices: A case study.
\newblock In {\em 23rd IEEE International Conference on Pattern Recognition
  (ICPR)}, pages 3530--3535, 2016.

\bibitem{pouladzadeh2017mobile}
Parisa Pouladzadeh and Shervin Shirmohammadi.
\newblock Mobile multi-food recognition using deep learning.
\newblock {\em ACM Transactions on Multimedia Computing, Communications, and
  Applications (TOMM)}, 13(3s):36, 2017.

\bibitem{tanno2016deepfoodcam}
Ryosuke Tanno, Koichi Okamoto, and Keiji Yanai.
\newblock {DeepFoodCam}: A {DCNN}-based real-time mobile food recognition
  system.
\newblock In {\em Proceedings of the 2nd ACM International Workshop on
  Multimedia Assisted Dietary Management}, pages 89--89, 2016.

\bibitem{kuhad2015using}
Pallavi Kuhad, Abdulsalam Yassine, and Shervin Shimohammadi.
\newblock Using distance estimation and deep learning to simplify calibration
  in food calorie measurement.
\newblock In {\em IEEE International Conference on Computational Intelligence
  and Virtual Environments for Measurement Systems and Applications (CIVEMSA)},
  pages 1--6, 2015.

\bibitem{teng2016facial}
Teng Teng and Xubo Yang.
\newblock Facial expressions recognition based on convolutional neural networks
  for mobile virtual reality.
\newblock In {\em Proceedings of the 15th ACM SIGGRAPH Conference on
  Virtual-Reality Continuum and Its Applications in Industry-Volume 1}, pages
  475--478, 2016.

\bibitem{rao2017mobile}
Jinmeng Rao, Yanjun Qiao, Fu~Ren, Junxing Wang, and Qingyun Du.
\newblock A mobile outdoor augmented reality method combining deep learning
  object detection and spatial relationships for geovisualization.
\newblock {\em Sensors}, 17(9):1951, 2017.

\bibitem{zeng2014convolutional}
Ming Zeng, Le~T Nguyen, Bo~Yu, Ole~J Mengshoel, Jiang Zhu, Pang Wu, and Joy
  Zhang.
\newblock Convolutional neural networks for human activity recognition using
  mobile sensors.
\newblock In {\em 6th IEEE International Conference on Mobile Computing,
  Applications and Services (MobiCASE)}, pages 197--205, 2014.

\bibitem{almaslukh2017effective}
Bandar Almaslukh, Jalal AlMuhtadi, and Abdelmonim Artoli.
\newblock An effective deep autoencoder approach for online smartphone-based
  human activity recognition.
\newblock {\em International Journal of Computer Science and Network Security
  (IJCSNS)}, 17(4):160, 2017.

\bibitem{li2016deep22}
Xinyu Li, Yanyi Zhang, Ivan Marsic, Aleksandra Sarcevic, and Randall~S Burd.
\newblock Deep learning for {RFID}-based activity recognition.
\newblock In {\em Proceedings of the 14th ACM Conference on Embedded Network
  Sensor Systems CD-ROM}, pages 164--175, 2016.

\bibitem{bhattacharya2016smart}
Sourav Bhattacharya and Nicholas~D Lane.
\newblock From smart to deep: Robust activity recognition on smartwatches using
  deep learning.
\newblock In {\em IEEE International Conference on Pervasive Computing and
  Communication Workshops (PerCom Workshops)}, pages 1--6, 2016.

\bibitem{antoniou2016general}
Antreas Antoniou and Plamen Angelov.
\newblock A general purpose intelligent surveillance system for mobile devices
  using deep learning.
\newblock In {\em IEEE International Joint Conference on Neural Networks
  (IJCNN)}, pages 2879--2886, 2016.

\bibitem{wang2016interacting}
Saiwen Wang, Jie Song, Jaime Lien, Ivan Poupyrev, and Otmar Hilliges.
\newblock Interacting with {Soli}: Exploring fine-grained dynamic gesture
  recognition in the radio-frequency spectrum.
\newblock In {\em Proceedings of the 29th ACM Annual Symposium on User
  Interface Software and Technology}, pages 851--860, 2016.

\bibitem{gao2016ihear}
Yang Gao, Ning Zhang, Honghao Wang, Xiang Ding, Xu~Ye, Guanling Chen, and
  Yu~Cao.
\newblock ihear food: Eating detection using commodity bluetooth headsets.
\newblock In {\em IEEE First International Conference on Connected Health:
  Applications, Systems and Engineering Technologies (CHASE)}, pages 163--172,
  2016.

\bibitem{zhu2015using}
Jindan Zhu, Amit Pande, Prasant Mohapatra, and Jay~J Han.
\newblock Using deep learning for energy expenditure estimation with wearable
  sensors.
\newblock In {\em 17th IEEE International Conference on E-health Networking,
  Application \& Services (HealthCom)}, pages 501--506, 2015.

\bibitem{sundsoy2016deep}
P{\aa}l Sunds{\o}y, Johannes Bjelland, B~Reme, A~Iqbal, and Eaman Jahani.
\newblock Deep learning applied to mobile phone data for individual income
  classification.
\newblock {\em ICAITA doi}, 10, 2016.

\bibitem{chen2015deep}
Yuqing Chen and Yang Xue.
\newblock A deep learning approach to human activity recognition based on
  single accelerometer.
\newblock In {\em IEEE International Conference on Systems, Man, and
  Cybernetics (SMC)}, pages 1488--1492, 2015.

\bibitem{ha2016convolutional}
Sojeong Ha and Seungjin Choi.
\newblock Convolutional neural networks for human activity recognition using
  multiple accelerometer and gyroscope sensors.
\newblock In {\em IEEE International Joint Conference on Neural Networks
  (IJCNN)}, pages 381--388, 2016.

\bibitem{edel2016binarized}
Marcus Edel and Enrico K{\"o}ppe.
\newblock Binarized-{BLSTM-RNN} based human activity recognition.
\newblock In {\em IEEE International Conference on Indoor Positioning and
  Indoor Navigation (IPIN)}, pages 1--7, 2016.

\bibitem{xue2018appdna}
{\color{blue}Xue, Shuangshuang and Zhang, Lan and Li, Anran and Li, Xiang-Yang
  and Ruan, Chaoyi and Huang, Wenchao}.
\newblock {\color{blue}{AppDNA}: App behavior profiling via graph-based deep
  learning}.
\newblock In {\em {\color{blue}IEEE Conference on Computer Communications}},
  pages~{\color{blue}1475--1483}, {\color{blue}2018}.

\bibitem{liu2018finding}
{\color{blue}Liu, Huiqi and Li, Xiang-Yang and Zhang, Lan and Xie, Yaochen and
  Wu, Zhenan and Dai, Qian and Chen, Ge and Wan, Chunxiao}.
\newblock {\color{blue}Finding the stars in the fireworks: Deep understanding
  of motion sensor fingerprint}.
\newblock In {\em {\color{blue}IEEE Conference on Computer Communications}},
  pages~{\color{blue}126--134}, {\color{blue}2018}.

\bibitem{okita2017recognition}
Tsuyoshi Okita and Sozo Inoue.
\newblock Recognition of multiple overlapping activities using compositional
  cnn-lstm model.
\newblock In {\em Proceedings of the ACM International Joint Conference on
  Pervasive and Ubiquitous Computing and Proceedings of the ACM International
  Symposium on Wearable Computers}, pages 165--168. ACM, 2017.

\bibitem{mittal2016spotgarbage}
Gaurav Mittal, Kaushal~B Yagnik, Mohit Garg, and Narayanan~C Krishnan.
\newblock Spotgarbage: smartphone app to detect garbage using deep learning.
\newblock In {\em Proceedings of the ACM International Joint Conference on
  Pervasive and Ubiquitous Computing}, pages 940--945, 2016.

\bibitem{seidenari2017deep}
Lorenzo Seidenari, Claudio Baecchi, Tiberio Uricchio, Andrea Ferracani, Marco
  Bertini, and Alberto~Del Bimbo.
\newblock Deep artwork detection and retrieval for automatic context-aware
  audio guides.
\newblock {\em ACM Transactions on Multimedia Computing, Communications, and
  Applications (TOMM)}, 13(3s):35, 2017.

\bibitem{zeng2017mobiledeeppill}
Xiao Zeng, Kai Cao, and Mi~Zhang.
\newblock Mobiledeeppill: A small-footprint mobile deep learning system for
  recognizing unconstrained pill images.
\newblock In {\em Proceedings of the 15th ACM Annual International Conference
  on Mobile Systems, Applications, and Services}, pages 56--67, 2017.

\bibitem{zoudeepsense}
\color{black}{Zou, Han and Zhou, Yuxun and Yang, Jianfei and Jiang, Hao and
  Xie, Lihua and Spanos, Costas J}.
\newblock Deepsense: Device-free human activity recognition via autoencoder
  long-term recurrent convolutional network.
\newblock 2018\color{black}.

\bibitem{zeng2017mobile}
Xiao Zeng.
\newblock Mobile sensing through deep learning.
\newblock In {\em Proceedings of the Workshop on MobiSys Ph. D. Forum}, pages
  5--6. ACM, 2017.

\bibitem{wang2015phasefi}
Xuyu Wang, Lingjun Gao, and Shiwen Mao.
\newblock {PhaseFi}: Phase fingerprinting for indoor localization with a deep
  learning approach.
\newblock In {\em IEEE Global Communications Conference (GLOBECOM)}, pages
  1--6, 2015.

\bibitem{wang2016csi}
Xuyu Wang, Lingjun Gao, and Shiwen Mao.
\newblock {CSI} phase fingerprinting for indoor localization with a deep
  learning approach.
\newblock {\em IEEE Internet of Things Journal}, 3(6):1113--1123, 2016.

\bibitem{feng2018evaluation}
\color{black}{Feng, Chunhai and Arshad, Sheheryar and Yu, Ruiyun and Liu,
  Yonghe}.
\newblock Evaluation and improvement of activity detection systems with
  recurrent neural network.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{cao2017deepmood}
Bokai Cao, Lei Zheng, Chenwei Zhang, Philip~S Yu, Andrea Piscitello, John
  Zulueta, Olu Ajilore, Kelly Ryan, and Alex~D Leow.
\newblock Deepmood: Modeling mobile phone typing dynamics for mood detection.
\newblock In {\em Proceedings of the 23rd ACM SIGKDD International Conference
  on Knowledge Discovery and Data Mining}, pages 747--755, 2017.

\bibitem{ran2018deepdecision}
\color{black}{Ran, Xukan and Chen, Haoliang and Zhu, Xiaodan and Liu, Zhenming
  and Chen, Jiasi}.
\newblock Deepdecision: A mobile deep learning framework for edge video
  analytics.
\newblock In {\em IEEE International Conference on Computer Communications},
  2018\color{black}.

\bibitem{siri}
Siri Team.
\newblock {Deep Learning for Siri's Voice: On-device Deep Mixture Density
  Networks for Hybrid Unit Selection Synthesis}.
\newblock \url{https://machinelearning.apple.com/2017/08/06/siri-voices.html},
  2017.
\newblock [Online; accessed 16-Sep-2017].

\bibitem{mcgraw2016personalized}
Ian McGraw, Rohit Prabhavalkar, Raziel Alvarez, Montse~Gonzalez Arenas,
  Kanishka Rao, David Rybach, Ouais Alsharif, Ha{\c{s}}im Sak, Alexander
  Gruenstein, Fran{\c{c}}oise Beaufays, et~al.
\newblock Personalized speech recognition on mobile devices.
\newblock In {\em IEEE International Conference on Acoustics, Speech and Signal
  Processing (ICASSP)}, pages 5955--5959, 2016.

\bibitem{prabhavalkar2016compression}
Rohit Prabhavalkar, Ouais Alsharif, Antoine Bruguier, and Lan McGraw.
\newblock On the compression of recurrent neural networks with an application
  to {LVCSR} acoustic modeling for embedded speech recognition.
\newblock In {\em IEEE International Conference on Acoustics, Speech and Signal
  Processing (ICASSP)}, pages 5970--5974, 2016.

\bibitem{yoshioka2015ntt}
Takuya Yoshioka, Nobutaka Ito, Marc Delcroix, Atsunori Ogawa, Keisuke
  Kinoshita, Masakiyo Fujimoto, Chengzhu Yu, Wojciech~J Fabian, Miquel Espi,
  Takuya Higuchi, et~al.
\newblock The {NTT CHiME}-3 system: Advances in speech enhancement and
  recognition for mobile multi-microphone devices.
\newblock In {\em IEEE Workshop on Automatic Speech Recognition and
  Understanding (ASRU)}, pages 436--443, 2015.

\bibitem{ruan2016speech}
Sherry Ruan, Jacob~O Wobbrock, Kenny Liou, Andrew Ng, and James Landay.
\newblock Speech is 3x faster than typing for english and mandarin text entry
  on mobile devices.
\newblock {\em arXiv preprint arXiv:1608.07323}, 2016.

\bibitem{ignatov2017dslr}
Andrey Ignatov, Nikolay Kobyshev, Radu Timofte, Kenneth Vanhoey, and Luc
  Van~Gool.
\newblock {DSLR}-quality photos on mobile devices with deep convolutional
  networks.
\newblock In {\em IEEE International Conference on Computer Vision (ICCV)},
  2017.

\bibitem{lu2017demo}
Zongqing Lu, Noor Felemban, Kevin Chan, and Thomas La~Porta.
\newblock Demo abstract: On-demand information retrieval from videos using deep
  learning in wireless networks.
\newblock In {\em IEEE/ACM Second International Conference on
  Internet-of-Things Design and Implementation (IoTDI)}, pages 279--280, 2017.

\bibitem{lee2016reducing}
Jemin Lee, Jinse Kwon, and Hyungshin Kim.
\newblock Reducing distraction of smartwatch users with deep learning.
\newblock In {\em Proceedings of the 18th ACM International Conference on
  Human-Computer Interaction with Mobile Devices and Services Adjunct}, pages
  948--953, 2016.

\bibitem{vu2016transportation}
Toan~H Vu, Le~Dung, and Jia-Ching Wang.
\newblock Transportation mode detection on mobile devices using recurrent nets.
\newblock In {\em Proceedings of the ACM on Multimedia Conference}, pages
  392--396, 2016.

\bibitem{fang2017learning}
Shih-Hau Fang, Yu-Xaing Fei, Zhezhuang Xu, and Yu~Tsao.
\newblock Learning transportation modes from smartphone sensors based on deep
  neural network.
\newblock {\em IEEE Sensors Journal}, 17(18):6111--6118, 2017.

\bibitem{zhao2018rf}
\color{black}{Zhao, Mingmin and Tian, Yonglong and Zhao, Hang and Alsheikh,
  Mohammad Abu and Li, Tianhong and Hristov, Rumen and Kabelac, Zachary and
  Katabi, Dina and Torralba, Antonio}.
\newblock {RF}-based {3D} skeletons.
\newblock In {\em Proceedings of the ACM Conference of the ACM Special Interest
  Group on Data Communication (SIGCOMM)}, pages 267--281, 2018\color{black}.

\bibitem{katevas2017practical}
Kleomenis Katevas, Ilias Leontiadis, Martin Pielot, and Joan Serr{\`a}.
\newblock Practical processing of mobile sensor data for continual deep
  learning predictions.
\newblock In {\em Proceedings of the 1st ACM International Workshop on Deep
  Learning for Mobile Systems and Applications}, 2017.

\bibitem{yao2017deepsense}
Shuochao Yao, Shaohan Hu, Yiran Zhao, Aston Zhang, and Tarek Abdelzaher.
\newblock Deepsense: A unified deep learning framework for time-series mobile
  sensing data processing.
\newblock In {\em Proceedings of the 26th International Conference on World
  Wide Web}, pages 351--360. International World Wide Web Conferences Steering
  Committee, 2017.

\bibitem{ohara2017detecting}
Kazuya Ohara, Takuya Maekawa, and Yasuyuki Matsushita.
\newblock Detecting state changes of indoor everyday objects using {Wi-Fi}
  channel state information.
\newblock {\em Proceedings of the ACM on Interactive, Mobile, Wearable and
  Ubiquitous Technologies}, 1(3):88, 2017.

\bibitem{liu2017deep}
Wu~Liu, Huadong Ma, Heng Qi, Dong Zhao, and Zhineng Chen.
\newblock Deep learning hashing for mobile visual search.
\newblock {\em EURASIP Journal on Image and Video Processing}, (1):17, 2017.

\bibitem{ouyang2016deepspace}
Xi~Ouyang, Chaoyun Zhang, Pan Zhou, and Hao Jiang.
\newblock {DeepSpace}: An online deep learning framework for mobile big data to
  understand human mobility patterns.
\newblock {\em arXiv preprint arXiv:1610.07009}, 2016.

\bibitem{yang2017neural}
Hua Yang, Zhimei Li, and Zhiyong Liu.
\newblock Neural networks for {MANET AODV}: an optimization approach.
\newblock {\em Cluster Computing}, pages 1--9, 2017.

\bibitem{song2016deeptransport}
Xuan Song, Hiroshi Kanasugi, and Ryosuke Shibasaki.
\newblock {DeepTransport}: Prediction and simulation of human mobility and
  transportation mode at a citywide level.
\newblock In {\em International Joint Conference on Artificial Intelligence},
  pages 2618--2624, 2016.

\bibitem{zhang2017deep123}
Junbo Zhang, Yu~Zheng, and Dekang Qi.
\newblock Deep spatio-temporal residual networks for citywide crowd flows
  prediction.
\newblock In {\em Thirty-First Association for the Advancement of Artificial
  Intelligence (AAAI) Conference on Artificial Intelligence}, 2017.

\bibitem{subramanian2014implementation}
J~Venkata Subramanian and M~Abdul~Karim Sadiq.
\newblock Implementation of artificial neural network for mobile movement
  prediction.
\newblock {\em Indian Journal of science and Technology}, 7(6):858--863, 2014.

\bibitem{ezema2017artificial}
Longinus~S Ezema and Cosmas~I Ani.
\newblock Artificial neural network approach to mobile location estimation in
  {GSM} network.
\newblock {\em International Journal of Electronics and Telecommunications},
  63(1):39--44, 2017.

\bibitem{shao2018depedo}
\color{black}{Shao, Wenhua and Luo, Haiyong and Zhao, Fang and Wang, Cong and
  Crivello, Antonino and Tunio, Muhammad Zahid}.
\newblock {DePedo}: Anti periodic negative-step movement pedometer with deep
  convolutional neural networks.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{yayeh2018mobility}
{\color{blue}Yayeh, Yirga and Lin, Hsin-piao and Berie, Getaneh and Adege,
  Abebe Belay and Yen, Lei and Jeng, Shiann-Shiun}.
\newblock {\color{blue}Mobility prediction in mobile {Ad-hoc} network using
  deep learning}.
\newblock In {\em {\color{blue}IEEE International Conference on Applied System
  Invention (ICASI)}}, pages~{\color{blue}1203--1206}, {\color{blue}2018}.

\bibitem{chen2016learning2}
{\color{blue}Chen, Quanjun and Song, Xuan and Yamada, Harutoshi and Shibasaki,
  Ryosuke}.
\newblock {\color{blue}Learning Deep Representation from Big and Heterogeneous
  Data for Traffic Accident Inference}.
\newblock In {\em {\color{blue}National Conference on Artificial Intelligence
  (AAAI)}}, pages~{\color{blue}338--344}, {\color{blue}2016}.

\bibitem{song2017deepmob}
{\color{blue}Song, Xuan and Shibasaki, Ryosuke and Yuan, Nicholos Jing and Xie,
  Xing and Li, Tao and Adachi, Ryutaro}.
\newblock {\color{blue}{DeepMob}: learning deep knowledge of human emergency
  behavior and mobility from big and heterogeneous data}.
\newblock {\em {\color{blue}ACM Transactions on Information Systems (TOIS)}},
  {\color{blue}35}({\color{blue}4}):{\color{blue}41}, {\color{blue}2017}.

\bibitem{yao2017trajectory}
{\color{blue}Yao, Di and Zhang, Chao and Zhu, Zhihua and Huang, Jianhui and Bi,
  Jingping}.
\newblock {\color{blue}Trajectory clustering via deep representation learning}.
\newblock In {\em {\color{blue}IEEE International Joint Conference on Neural
  Networks (IJCNN)}}, pages~{\color{blue}3880--3887}, {\color{blue}2017}.

\bibitem{liu2018urban}
{\color{blue}Liu, Zhidan and Li, Zhenjiang and Wu, Kaishun and Li, Mo}.
\newblock {\color{blue}Urban Traffic Prediction from Mobility Data Using Deep
  Learning}.
\newblock {\em {\color{blue}IEEE Network}},
  {\color{blue}32}({\color{blue}4}):{\color{blue}40--46}, {\color{blue}2018}.

\bibitem{wickramasuriya2017base}
Dilranjan~S Wickramasuriya, Calvin~A Perumalla, Kemal Davaslioglu, and
  Richard~D Gitlin.
\newblock Base station prediction and proactive mobility management in virtual
  cells using recurrent neural networks.
\newblock In {\em IEEE Wireless and Microwave Technology Conference (WAMICON)},
  pages 1--6.

\bibitem{tkavcik2016neural}
{\color{blue}Tka{\v{c}}{\'\i}k, Jan and Kord{\'\i}k, Pavel}.
\newblock {\color{blue}Neural turing machine for sequential learning of human
  mobility patterns}.
\newblock In {\em {\color{blue}IEEE International Joint Conference on Neural
  Networks (IJCNN)}}, pages~{\color{blue}2790--2797}, {\color{blue}2016}.

\bibitem{kim2018method}
{\color{blue}Kim, Dong Yup and Song, Ha Yoon}.
\newblock {\color{blue}Method of predicting human mobility patterns using deep
  learning}.
\newblock {\em {\color{blue}Neurocomputing}},
  {\color{blue}280}:{\color{blue}56--64}, {\color{blue}2018}.

\bibitem{jiang2018deepurbanmomentum}
{\color{blue}Jiang, Renhe and Song, Xuan and Fan, Zipei and Xia, Tianqi and
  Chen, Quanjun and Miyazawa, Satoshi and Shibasaki, Ryosuke}.
\newblock {\color{blue}{DeepUrbanMomentum}: An Online Deep-Learning System for
  Short-Term Urban Mobility Prediction}.
\newblock In {\em {\color{blue}National Conference on Artificial Intelligence
  (AAAI)}}, {\color{blue}2018}.

\bibitem{wang2018deep1231}
{\color{blue}Wang, Chujie and Zhao, Zhifeng and Sun, Qi and Zhang, Honggang}.
\newblock {\color{blue}Deep Learning-based Intelligent Dual Connectivity for
  Mobility Management in Dense Network}.
\newblock {\em {\color{blue}arXiv preprint arXiv:1806.04584}},
  {\color{blue}2018}.

\bibitem{jiang2018deep}
{\color{blue}Jiang, Renhe and Song, Xuan and Fan, Zipei and Xia, Tianqi and
  Chen, Quanjun and Chen, Qi and Shibasaki, Ryosuke}.
\newblock {\color{blue}Deep {ROI}-Based Modeling for Urban Human Mobility
  Prediction}.
\newblock {\em {\color{blue}Proceedings of the ACM on Interactive, Mobile,
  Wearable and Ubiquitous Technologies}},
  {\color{blue}2}({\color{blue}1}):{\color{blue}14}, {\color{blue}2018}.

\bibitem{feng2018deepmove}
{\color{blue}Feng, Jie and Li, Yong and Zhang, Chao and Sun, Funing and Meng,
  Fanchao and Guo, Ang and Jin, Depeng}.
\newblock {\color{blue}{DeepMove}: Predicting Human Mobility with Attentional
  Recurrent Networks}.
\newblock In {\em {\color{blue}Proceedings of the 2018 World Wide Web
  Conference on World Wide Web}}, pages~{\color{blue}1459--1468}.
  {\color{blue}International World Wide Web Conferences Steering Committee},
  {\color{blue}2018}.

\bibitem{wang2015deepfi}
Xuyu Wang, Lingjun Gao, Shiwen Mao, and Santosh Pandey.
\newblock {DeepFi}: Deep learning for indoor fingerprinting using channel state
  information.
\newblock In {\em IEEE Wireless Communications and Networking Conference
  (WCNC)}, pages 1666--1671, 2015.

\bibitem{wang2017cifi}
Xuyu Wang, Xiangyu Wang, and Shiwen Mao.
\newblock {CiFi}: Deep convolutional neural networks for indoor localization
  with 5 {GHz} {Wi-Fi}.
\newblock In {\em 2017 IEEE International Conference on Communications (ICC)},
  pages 1--6.

\bibitem{wang2017biloc}
Xuyu Wang, Lingjun Gao, and Shiwen Mao.
\newblock {BiLoc}: Bi-modal deep learning for indoor localization with
  commodity {5GHz WiFi}.
\newblock {\em IEEE Access}, 5:4209--4220, 2017.

\bibitem{nowicki2017low}
Micha{\l} Nowicki and Jan Wietrzykowski.
\newblock Low-effort place recognition with {WiFi} fingerprints using deep
  learning.
\newblock In {\em International Conference Automation}, pages 575--584.
  Springer, 2017.

\bibitem{zhang2016device}
Xiao Zhang, Jie Wang, Qinghua Gao, Xiaorui Ma, and Hongyu Wang.
\newblock Device-free wireless localization and activity recognition with deep
  learning.
\newblock In {\em IEEE International Conference on Pervasive Computing and
  Communication Workshops (PerCom Workshops)}, pages 1--5, 2016.

\bibitem{wang2017device}
Jie Wang, Xiao Zhang, Qinhua Gao, Hao Yue, and Hongyu Wang.
\newblock Device-free wireless localization and activity recognition: A deep
  learning approach.
\newblock {\em IEEE Transactions on Vehicular Technology}, 66(7):6258--6267,
  2017.

\bibitem{mohammadi2017semi}
Mehdi Mohammadi, Ala Al-Fuqaha, Mohsen Guizani, and Jun-Seok Oh.
\newblock Semi-supervised deep reinforcement learning in support of {IoT} and
  smart city services.
\newblock {\em IEEE Internet of Things Journal}, 2017.

\bibitem{anzum2018zone}
\color{black}{Anzum, Nafisa and Afroze, Syeda Farzia and Rahman, Ashikur}.
\newblock Zone-based indoor localization using neural networks: A view from a
  real testbed.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--7, 2018\color{black}.

\bibitem{wang2018deepml}
\color{black}{Wang, Xuyu and Yu, Zhitao and Mao, Shiwen}.
\newblock {DeepML}: Deep {LSTM} for indoor localization with smartphone
  magnetic and light sensors.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{kumar2016indoor}
Anil Kumar Tirumala~Ravi Kumar, Bernd Sch{\"a}ufele, Daniel Becker, Oliver
  Sawade, and Ilja Radusch.
\newblock Indoor localization of vehicles using deep learning.
\newblock In {\em 17th IEEE International Symposium on World of Wireless,
  Mobile and Multimedia Networks (WoWMoM)}, pages 1--6.

\bibitem{zhengj2016mobile}
Zejia Zhengj and Juyang Weng.
\newblock Mobile device based outdoor navigation with on-line learning neural
  network: A comparison with convolutional neural network.
\newblock In {\em Proceedings of the IEEE Conference on Computer Vision and
  Pattern Recognition Workshops}, pages 11--18, 2016.

\bibitem{vieira2017deep}
Joao Vieira, Erik Leitinger, Muris Sarajlic, Xuhong Li, and Fredrik Tufvesson.
\newblock Deep convolutional neural networks for massive {MIMO}
  fingerprint-based positioning.
\newblock In {\em 28th IEEE Annual International Symposium on Personal, Indoor
  and Mobile Radio Communications}, 2017.

\bibitem{wang2017csi}
{\color{blue}Wang, Xuyu and Gao, Lingjun and Mao, Shiwen and Pandey, Santosh}.
\newblock {\color{blue}{CSI}-based fingerprinting for indoor localization: A
  deep learning approach}.
\newblock {\em {\color{blue}IEEE Transactions on Vehicular Technology}},
  {\color{blue}66}({\color{blue}1}):{\color{blue}763--776}, {\color{blue}2017}.

\bibitem{chen2017confi}
{\color{blue}Chen, Hao and Zhang, Yifan and Li, Wei and Tao, Xiaofeng and
  Zhang, Ping}.
\newblock {\color{blue}{ConFi}: Convolutional neural networks based indoor
  {wi-fi} localization using channel state information}.
\newblock {\em {\color{blue}IEEE Access}},
  {\color{blue}5}:{\color{blue}18066--18074}, {\color{blue}2017}.

\bibitem{shokry2018deeploc}
{\color{blue}Shokry, Ahmed and Torki, Marwan and Youssef, Moustafa}.
\newblock {\color{blue}{DeepLoc}: A ubiquitous accurate and low-overhead
  outdoor cellular localization system}.
\newblock In {\em {\color{blue}Proceedings of the 26th ACM SIGSPATIAL
  International Conference on Advances in Geographic Information Systems}},
  pages~{\color{blue}339--348}, {\color{blue}2018}.

\bibitem{zhou2018device}
{\color{blue}Zhou, Rui and Hao, Meng and Lu, Xiang and Tang, Mingjie and Fu,
  Yang}.
\newblock {\color{blue}Device-Free Localization Based on {CSI} Fingerprints and
  Deep Neural Networks}.
\newblock In {\em {\color{blue}15th Annual IEEE International Conference on
  Sensing, Communication, and Networking (SECON)}}, pages~{\color{blue}1--9},
  {\color{blue}2018}.

\bibitem{zhang2017deeppositioning}
{\color{blue}Zhang, Wei and Sengupta, Rahul and Fodero, John and Li, Xiaolin}.
\newblock {\color{blue}{DeepPositioning}: Intelligent Fusion of Pervasive
  Magnetic Field and {WiFi} Fingerprinting for Smartphone Indoor Localization
  via Deep Learning}.
\newblock In {\em {\color{blue}16th IEEE International Conference on Machine
  Learning and Applications (ICMLA)}}, pages~{\color{blue}7--13},
  {\color{blue}2017}.

\bibitem{adege2018applying}
{\color{blue}Adege, Abebe and Lin, Hsin-Piao and Tarekegn, Getaneh and Jeng,
  Shiann-Shiun}.
\newblock {\color{blue}Applying Deep Neural Network {(DNN)} for Robust Indoor
  Localization in Multi-Building Environment}.
\newblock {\em {\color{blue}Applied Sciences}},
  {\color{blue}8}({\color{blue}7}):{\color{blue}1062}, {\color{blue}2018}.

\bibitem{ibrahim2018cnn}
{\color{blue}Ibrahim, Mai and Torki, Marwan and ElNainay, Mustafa}.
\newblock {\color{blue}{CNN} based Indoor Localization using {RSS}
  Time-Series}.
\newblock In {\em {\color{blue}IEEE Symposium on Computers and Communications
  (ISCC)}}, pages~{\color{blue}1044--1049}, {\color{blue}2018}.

\bibitem{niitsoo2018convolutional}
{\color{blue}Niitsoo, Arne and Edelh{\"a}u$\beta$er, Thorsten and Mutschler,
  Christopher}.
\newblock {\color{blue}Convolutional neural networks for position estimation in
  {TDoA}-based locating systems}.
\newblock In {\em {\color{blue}IEEE International Conference on Indoor
  Positioning and Indoor Navigation (IPIN)}}, pages~{\color{blue}1--8},
  {\color{blue}2018}.

\bibitem{wang2018deep6}
{\color{blue}Wang, Xuyu and Wang, Xiangyu and Mao, Shiwen}.
\newblock {\color{blue}Deep convolutional neural networks for indoor
  localization with {CSI} images}.
\newblock {\em {\color{blue}IEEE Transactions on Network Science and
  Engineering}}, {\color{blue}2018}.

\bibitem{xiao20173}
{\color{blue}Xiao, Chao and Yang, Daiqin and Chen, Zhenzhong and Tan, Guang}.
\newblock {\color{blue}{3-D BLE} indoor localization based on denoising
  autoencoder}.
\newblock {\em {\color{blue}IEEE Access}},
  {\color{blue}5}:{\color{blue}12751--12760}, {\color{blue}2017}.

\bibitem{Hsu:2017:ZIS:3139486.3130924}
{\color{blue}Hsu, Chen-Yu and Ahuja, Aayush and Yue, Shichao and Hristov, Rumen
  and Kabelac, Zachary and Katabi, Dina}.
\newblock {\color{blue}Zero-Effort In-Home Sleep and Insomnia Monitoring Using
  Radio Signals}.
\newblock {\em {\color{blue}Proceedings of ACM Interactive, Mobile, Wearable
  and Ubiquitous Technologies (IMWUT)}}, {\color{blue}1}({\color{blue}3}),
  September {\color{blue}2017}.

\bibitem{guan2017high}
{\color{blue}Guan, Weipeng and Wu, Yuxiang and Xie, Canyu and Chen, Hao and
  Cai, Ye and Chen, Yingcong}.
\newblock {\color{blue}High-precision approach to localization scheme of
  visible light communication based on artificial neural networks and modified
  genetic algorithms}.
\newblock {\em {\color{blue}Optical Engineering}},
  {\color{blue}56}({\color{blue}10}):{\color{blue}106103}, {\color{blue}2017}.

\bibitem{chuang2014effective}
Po-Jen Chuang and Yi-Jun Jiang.
\newblock Effective neural network-based node localisation scheme for wireless
  sensor networks.
\newblock {\em IET Wireless Sensor Systems}, 4(2):97--103, 2014.

\bibitem{bernas2015fully}
Marcin Bernas and Bart{\l}omiej P{\l}aczek.
\newblock Fully connected neural networks ensemble with signal strength
  clustering for indoor localization in wireless sensor networks.
\newblock {\em International Journal of Distributed Sensor Networks},
  11(12):403242, 2015.

\bibitem{payal2015analysis}
Ashish Payal, Chandra~Shekhar Rai, and BV~Ramana Reddy.
\newblock Analysis of some feedforward artificial neural network training
  algorithms for developing localization framework in wireless sensor networks.
\newblock {\em Wireless Personal Communications}, 82(4):2519--2536, 2015.

\bibitem{dong2017range}
Yuhan Dong, Zheng Li, Rui Wang, and Kai Zhang.
\newblock Range-based localization in underwater wireless sensor networks using
  deep neural network.
\newblock In {\em IPSN}, pages 321--322, 2017.

\bibitem{yan2016real}
Xiaofei Yan, Hong Cheng, Yandong Zhao, Wenhua Yu, Huan Huang, and Xiaoliang
  Zheng.
\newblock Real-time identification of smoldering and flaming combustion phases
  in forest using a wireless sensor network-based multi-sensor system and
  artificial neural network.
\newblock {\em Sensors}, 16(8):1228, 2016.

\bibitem{wang2017temperature}
Baowei Wang, Xiaodu Gu, Li~Ma, and Shuangshuang Yan.
\newblock Temperature error correction based on {BP} neural network in
  meteorological wireless sensor network.
\newblock {\em International Journal of Sensor Networks}, 23(4):265--278, 2017.

\bibitem{lee2017deep222}
Ki-Seong Lee, Sun-Ro Lee, Youngmin Kim, and Chan-Gun Lee.
\newblock Deep learning--based real-time query processing for wireless sensor
  network.
\newblock {\em International Journal of Distributed Sensor Networks}, 13(5),
  2017.

\bibitem{li2016adaptive}
Jiakai Li and Gursel Serpen.
\newblock Adaptive and intelligent wireless sensor networks through neural
  networks: an illustration for infrastructure adaptation through hopfield
  network.
\newblock {\em Applied Intelligence}, 45(2):343--362, 2016.

\bibitem{khorasani2017energy}
Fereshteh Khorasani and Hamid~Reza Naji.
\newblock Energy efficient data aggregation in wireless sensor networks using
  neural networks.
\newblock {\em International Journal of Sensor Networks}, 24(1):26--42, 2017.

\bibitem{li2015distributed}
Chunlin Li, Xiaofu Xie, Yuejiang Huang, Hong Wang, and Changxi Niu.
\newblock Distributed data mining based on deep neural network for wireless
  sensor network.
\newblock {\em International Journal of Distributed Sensor Networks},
  11(7):157453, 2015.

\bibitem{luo2018distributed}
\color{black}{Luo, Tie and Nagarajany, Sai G}.
\newblock Distributed anomaly detection using autoencoder neural networks in
  {WSN for IoT}.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{kumar2019machine}
{\color{blue}Kumar, D Praveen and Amgoth, Tarachand and Annavarapu, Chandra
  Sekhara Rao}.
\newblock {\color{blue}Machine learning algorithms for wireless sensor
  networks: A survey}.
\newblock {\em {\color{blue}Information Fusion}},
  {\color{blue}49}:{\color{blue}1--25}, {\color{blue}2019}.

\bibitem{heydari2017reduce}
{\color{blue}Heydari, Nasim and Minaei-Bidgoli, Behrouz}.
\newblock {\color{blue}Reduce energy consumption and send secure data wireless
  multimedia sensor networks using a combination of techniques for multi-layer
  watermark and deep learning}.
\newblock {\em {\color{blue}International Journal of Computer Science and
  Network Security (IJCSNS)}},
  {\color{blue}17}({\color{blue}2}):{\color{blue}98--105}, {\color{blue}2017}.

\bibitem{phoemphon2018hybrid}
{\color{blue}Phoemphon, Songyut and So-In, Chakchai and Niyato, Dusit Tao}.
\newblock {\color{blue}A hybrid model using fuzzy logic and an extreme learning
  machine with vector particle swarm optimization for wireless sensor network
  localization}.
\newblock {\em {\color{blue}Applied Soft Computing}},
  {\color{blue}65}:{\color{blue}101--120}, {\color{blue}2018}.

\bibitem{banihashemian2018new}
{\color{blue}Banihashemian, Seyed Saber and Adibnia, Fazlollah and Sarram,
  Mehdi A}.
\newblock {\color{blue}A new range-free and storage-efficient localization
  algorithm using neural networks in wireless sensor networks}.
\newblock {\em {\color{blue}Wireless Personal Communications}},
  {\color{blue}98}({\color{blue}1}):{\color{blue}1547--1568},
  {\color{blue}2018}.

\bibitem{sun2017wnn}
{\color{blue}Sun, Wei and Lu, Wei and Li, Qiyue and Chen, Liangfeng and Mu,
  Daoming and Yuan, Xiaojing}.
\newblock {\color{blue}{WNN-LQE}: Wavelet-Neural-Network-Based Link Quality
  Estimation for Smart Grid {WSNs}}.
\newblock {\em {\color{blue}IEEE Access}},
  {\color{blue}5}:{\color{blue}12788--12797}, {\color{blue}2017}.

\bibitem{kang2018novel}
{\color{blue}Kang, Jiheon and Park, Youn-Jong and Lee, Jaeho and Wang, Soo-Hyun
  and Eom, Doo-Seop}.
\newblock {\color{blue}Novel Leakage Detection by Ensemble {CNN-SVM} and
  Graph-based Localization in Water Distribution Systems}.
\newblock {\em {\color{blue}IEEE Transactions on Industrial Electronics}},
  {\color{blue}65}({\color{blue}5}):{\color{blue}4279--4289},
  {\color{blue}2018}.

\bibitem{mehmood2017eldc}
{\color{blue}Mehmood, Amjad and Lv, Zhihan and Lloret, Jaime and Umar, Muhammad
  Muneer}.
\newblock {\color{blue}{ELDC}: An artificial neural network based
  energy-efficient and robust routing scheme for pollution monitoring in WSNs}.
\newblock {\em {\color{blue}IEEE Transactions on Emerging Topics in
  Computing}}, {\color{blue}2017}.

\bibitem{alsheikh2016rate}
{\color{blue}Alsheikh, Mohammad Abu and Lin, Shaowei and Niyato, Dusit and Tan,
  Hwee-Pink}.
\newblock {\color{blue}Rate-distortion balanced data compression for wireless
  sensor networks}.
\newblock {\em {\color{blue}IEEE Sensors Journal}},
  {\color{blue}16}({\color{blue}12}):{\color{blue}5072--5083},
  {\color{blue}2016}.

\bibitem{el2016robust}
{\color{blue}El Assaf, Ahmad and Zaidi, Slim and Affes, Sofi{\`e}ne and Kandil,
  Nahi}.
\newblock {\color{blue}Robust {ANNs-Based WSN} Localization in the Presence of
  Anisotropic Signal Attenuation}.
\newblock {\em {\color{blue}IEEE Wireless Communications Letters}},
  {\color{blue}5}({\color{blue}5}):{\color{blue}504--507}, {\color{blue}2016}.

\bibitem{wang2017deep3}
{\color{blue}Wang, Yuzhi and Yang, Anqi and Chen, Xiaoming and Wang, Pengjun
  and Wang, Yu and Yang, Huazhong}.
\newblock {\color{blue}A deep learning approach for blind drift calibration of
  sensor networks}.
\newblock {\em {\color{blue}IEEE Sensors Journal}},
  {\color{blue}17}({\color{blue}13}):{\color{blue}4158--4171},
  {\color{blue}2017}.

\bibitem{jia2018continuous}
{\color{blue}Jia, Zhenhua and Lyu, Xinmeng and Zhang, Wuyang and Martin,
  Richard P and Howard, Richard E and Zhang, Yanyong}.
\newblock {\color{blue}Continuous Low-Power Ammonia Monitoring Using Long
  Short-Term Memory Neural Networks}.
\newblock In {\em {\color{blue}Proceedings of the 16th ACM Conference on
  Embedded Networked Sensor Systems}}, pages~{\color{blue}224--236},
  {\color{blue}2018}.

\bibitem{liu2017deep222}
Lu~Liu, Yu~Cheng, Lin Cai, Sheng Zhou, and Zhisheng Niu.
\newblock Deep learning based optimization in wireless network.
\newblock In {\em 2017 IEEE International Conference on Communications (ICC)},
  pages 1--6.

\bibitem{subramanian2016poster}
Shivashankar Subramanian and Arindam Banerjee.
\newblock Poster: Deep learning enabled {M2M} gateway for network optimization.
\newblock In {\em Proceedings of the 14th ACM Annual International Conference
  on Mobile Systems, Applications, and Services Companion}, pages 144--144,
  2016.

\bibitem{he2017optimization}
Ying He, Chengchao Liang, F~Richard Yu, Nan Zhao, and Hongxi Yin.
\newblock Optimization of cache-enabled opportunistic interference alignment
  wireless networks: A big data deep reinforcement learning approach.
\newblock In {\em 2017 IEEE International Conference on Communications (ICC)},
  pages 1--6.

\bibitem{he2017deep3}
Ying He, Zheng Zhang, F~Richard Yu, Nan Zhao, Hongxi Yin, Victor~CM Leung, and
  Yanhua Zhang.
\newblock Deep reinforcement learning-based optimization for cache-enabled
  opportunistic interference alignment wireless networks.
\newblock {\em IEEE Transactions on Vehicular Technology}, 2017.

\bibitem{mismar2017deep}
Faris~B Mismar and Brian~L Evans.
\newblock Deep reinforcement learning for improving downlink mmwave
  communication performance.
\newblock {\em arXiv preprint arXiv:1707.02329}, 2017.

\bibitem{wang2018handover}
\color{black}{Wang, Zhi and Li, Lihua and Xu, Yue and Tian, Hui and Cui,
  Shuguang}.
\newblock Handover optimization via asynchronous multi-user deep reinforcement
  learning.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{chen2018heterogeneous}
\color{black}{Chen, Ziqi and Smith, David B}.
\newblock Heterogeneous machine-type communications in cellular networks:
  Random access optimization by deep reinforcement learning.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{chen2018auto}
\color{black}{Chen, Li and Lingys, Justinas and Chen, Kai and Liu, Feng}.
\newblock {AuTO}: scaling deep reinforcement learning for datacenter-scale
  automatic traffic optimization.
\newblock In {\em Proceedings of the ACM Conference of the ACM Special Interest
  Group on Data Communication (SIGCOMM)}, pages 191--205, 2018\color{black}.

\bibitem{lee2017classification}
YangMin Lee.
\newblock Classification of node degree based on deep learning and routing
  method applied for virtual route assignment.
\newblock {\em Ad Hoc Networks}, 58:70--85, 2017.

\bibitem{tang2017removing}
Fengxiao Tang, Bomin Mao, Zubair~Md Fadlullah, Nei Kato, Osamu Akashi, Takeru
  Inoue, and Kimihiro Mizutani.
\newblock On removing routing protocol from future wireless networks: A
  real-time deep learning approach for intelligent traffic control.
\newblock {\em IEEE Wireless Communications}, 2017.

\bibitem{zhang2017energy}
Qingchen Zhang, Man Lin, Laurence~T Yang, Zhikui Chen, and Peng Li.
\newblock Energy-efficient scheduling for real-time systems based on deep
  {Q}-learning model.
\newblock {\em IEEE Transactions on Sustainable Computing}, 2017.

\bibitem{atallah2017deep}
Ribal Atallah, Chadi Assi, and Maurice Khabbaz.
\newblock Deep reinforcement learning-based scheduling for roadside
  communication networks.
\newblock In {\em 15th IEEE International Symposium on Modeling and
  Optimization in Mobile, Ad Hoc, and Wireless Networks (WiOpt)}, pages 1--8,
  2017.

\bibitem{chinchali2018}
Sandeep Chinchali, Pan Hu, Tianshu Chu, Manu Sharma, Manu Bansal, Rakesh Misra,
  Marco Pavone, and Katti Sachin.
\newblock Cellular network traffic scheduling with deep reinforcement learning.
\newblock In {\em National Conference on Artificial Intelligence (AAAI)}, 2018.

\bibitem{wei2018joint}
\color{black}{Wei, Yifei and Zhang, Zhiqiang and Yu, F Richard and Han, Zhu}.
\newblock Joint user scheduling and content caching strategy for mobile edge
  networks using deep reinforcement learning.
\newblock In {\em IEEE International Conference on Communications Workshops
  (ICC Workshops)}, 2018\color{black}.

\bibitem{sun2017learning}
Haoran Sun, Xiangyi Chen, Qingjiang Shi, Mingyi Hong, Xiao Fu, and Nikos~D
  Sidiropoulos.
\newblock Learning to optimize: Training deep neural networks for wireless
  resource management.
\newblock In {\em 18th IEEE International Workshop on Signal Processing
  Advances in Wireless Communications (SPAWC)}, pages 1--6, 2017.

\bibitem{xu2017deep3}
Zhiyuan Xu, Yanzhi Wang, Jian Tang, Jing Wang, and Mustafa~Cenk Gursoy.
\newblock A deep reinforcement learning based framework for power-efficient
  resource allocation in cloud {RANs}.
\newblock In {\em 2017 IEEE International Conference on Communications (ICC)},
  pages 1--6.

\bibitem{ferreira2017multi}
Paulo Victor~R Ferreira, Randy Paffenroth, Alexander~M Wyglinski, Timothy~M
  Hackett, Sven~G Bil{\'e}n, Richard~C Reinhart, and Dale~J Mortensen.
\newblock Multi-objective reinforcement learning-based deep neural networks for
  cognitive space communications.
\newblock In {\em Cognitive Communications for Aerospace Applications Workshop
  (CCAA)}, pages 1--8. IEEE, 2017.

\bibitem{ye2018deep12}
\color{black}{Ye, Hao and Li, Geoffrey Ye}.
\newblock Deep reinforcement learning for resource allocation in {V2V}
  communications.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{challita2018proactive}
\color{black}{Challita, Ursula and Dong, Li and Saad, Walid}.
\newblock Proactive resource management for {LTE} in unlicensed spectrum: A
  deep learning perspective.
\newblock {\em IEEE Transactions on Wireless Communications},
  2018\color{black}.

\bibitem{naparstek2017deep}
Oshri Naparstek and Kobi Cohen.
\newblock Deep multi-user reinforcement learning for dynamic spectrum access in
  multichannel wireless networks.
\newblock In {\em IEEE Global Communications Conference}, pages 1--7, 2017.

\bibitem{o2016deep}
Timothy~J O'Shea and T~Charles Clancy.
\newblock Deep reinforcement learning radio control and signal detection with
  {KeRLym}, a gym {RL} agent.
\newblock {\em arXiv preprint arXiv:1605.09221}, 2016.

\bibitem{wijaya2015intercell}
Michael~Andri Wijaya, Kazuhiko Fukawa, and Hiroshi Suzuki.
\newblock Intercell-interference cancellation and neural network transmit power
  optimization for {MIMO} channels.
\newblock In {\em IEEE 82nd Vehicular Technology Conference (VTC Fall)}, pages
  1--5, 2015.

\bibitem{rutagemwa2018dynamic}
\color{black}{Rutagemwa, Humphrey and Ghasemi, Amir and Liu, Shuo}.
\newblock Dynamic spectrum assignment for land mobile radio with deep recurrent
  neural networks.
\newblock In {\em IEEE International Conference on Communications Workshops
  (ICC Workshops)}, 2018\color{black}.

\bibitem{wijaya2016neural}
Michael~Andri Wijaya, Kazuhiko Fukawa, and Hiroshi Suzuki.
\newblock Neural network based transmit power control and interference
  cancellation for {MIMO} small cell networks.
\newblock {\em IEICE Transactions on Communications}, 99(5):1157--1169, 2016.

\bibitem{mao2017neural}
Hongzi Mao, Ravi Netravali, and Mohammad Alizadeh.
\newblock Neural adaptive video streaming with pensieve.
\newblock In {\em Proceedings of the Conference of the ACM Special Interest
  Group on Data Communication (SIGCOMM)}, pages 197--210. ACM, 2017.

\bibitem{oda2017design}
Tetsuya Oda, Ryoichiro Obukata, Makoto Ikeda, Leonard Barolli, and Makoto
  Takizawa.
\newblock Design and implementation of a simulation system based on deep
  {Q}-network for mobile actor node control in wireless sensor and actor
  networks.
\newblock In {\em 31st IEEE International Conference on Advanced Information
  Networking and Applications Workshops (WAINA)}, pages 195--200, 2017.

\bibitem{oda2017performance}
Tetsuya Oda, Donald Elmazi, Miralda Cuka, Elis Kulla, Makoto Ikeda, and Leonard
  Barolli.
\newblock Performance evaluation of a deep {Q}-network based simulation system
  for actor node mobility control in wireless sensor and actor networks
  considering three-dimensional environment.
\newblock In {\em International Conference on Intelligent Networking and
  Collaborative Systems}, pages 41--52. Springer, 2017.

\bibitem{kim2017load}
Hye-Young Kim and Jong-Min Kim.
\newblock A load balancing scheme based on deep-learning in {IoT}.
\newblock {\em Cluster Computing}, 20(1):873--878, 2017.

\bibitem{challita2018deep}
\color{black}{Challita, Ursula and Saad, Walid and Bettstetter, Christian}.
\newblock Deep reinforcement learning for interference-aware path planning of
  cellular connected {UAVs}.
\newblock In {\em IEEE International Conference on Communications (ICC)},
  2018\color{black}.

\bibitem{luo2018online}
\color{black}{Luo, Changqing and Ji, Jinlong and Wang, Qianlong and Yu, Lixing
  and Li, Pan}.
\newblock Online power control for {5G} wireless communications: A deep
  {Q}-network approach.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{yu2018deep2}
\color{black}{Yu, Yiding and Wang, Taotao and Liew, Soung Chang}.
\newblock Deep-reinforcement learning multiple access for heterogeneous
  wireless networks.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--7, 2018\color{black}.

\bibitem{xu2018experience}
\color{black}{Xu, Zhiyuan and Tang, Jian and Meng, Jingsong and Zhang, Weiyi
  and Wang, Yanzhi and Liu, Chi Harold and Yang, Dejun}.
\newblock Experience-driven networking: A deep reinforcement learning based
  approach.
\newblock In {\em IEEE International Conference on Computer Communications},
  2018\color{black}.

\bibitem{liu2018deepnap}
\color{black}{Liu, Jingchu and Krishnamachari, Bhaskar and Zhou, Sheng and Niu,
  Zhisheng}.
\newblock {DeepNap}: Data-driven base station sleeping operations through deep
  reinforcement learning.
\newblock {\em IEEE Internet of Things Journal}, 2018\color{black}.

\bibitem{zhao2018deep}
{\color{blue}Zhao, Zhifeng and Li, Rongpeng and Sun, Qi and Yang, Yangchen and
  Chen, Xianfu and Zhao, Minjian and Zhang, Honggang and others}.
\newblock {\color{blue}Deep Reinforcement Learning for Network Slicing}.
\newblock {\em {\color{blue}arXiv preprint arXiv:1805.06591}},
  {\color{blue}2018}.

\bibitem{li2018deep}
{\color{blue}Li, Ji and Gao, Hui and Lv, Tiejun and Lu, Yueming}.
\newblock {\color{blue}Deep reinforcement learning based computation offloading
  and resource allocation for {MEC}}.
\newblock In {\em {\color{blue}IEEE Wireless Communications and Networking
  Conference (WCNC)}}, pages~{\color{blue}1--6}, {\color{blue}2018}.

\bibitem{mennes2018neural}
Steven {\color{blue}Mennes, Ruben and Camelo, Miguel and Claeys, Maxim and
  Latr{\'e}}.
\newblock {\color{blue}A neural-network-based {MF-TDMA MAC} scheduler for
  collaborative wireless networks}.

\bibitem{8553651}
{\color{blue}Zhou, Yibo and Fadlullah, Zubair Md. and Mao, Bomin and Kato,
  Nei}.
\newblock {\color{blue}A Deep-Learning-Based Radio Resource Assignment
  Technique for {5G} Ultra Dense Networks}.
\newblock {\em {\color{blue}IEEE Network}},
  {\color{blue}32}({\color{blue}6}):{\color{blue}28--34}, {\color{blue}2018}.

\bibitem{mao2017tensor}
{\color{blue}Mao, Bomin and Fadlullah, Zubair Md and Tang, Fengxiao and Kato,
  Nei and Akashi, Osamu and Inoue, Takeru and Mizutani, Kimihiro}.
\newblock {\color{blue}A Tensor Based Deep Learning Technique for Intelligent
  Packet Routing}.
\newblock In {\em {\color{blue}IEEE Global Communications Conference}},
  pages~{\color{blue}1--6}. {\color{blue}IEEE}, {\color{blue}2017}.

\bibitem{geyer2018learning}
{\color{blue}Geyer, Fabien and Carle, Georg}.
\newblock {\color{blue}Learning and Generating Distributed Routing Protocols
  Using Graph-Based Deep Learning}.
\newblock In {\em {\color{blue}Proceedings of the ACM Workshop on Big Data
  Analytics and Machine Learning for Data Communication Networks}},
  pages~{\color{blue}40--45}, {\color{blue}2018}.

\bibitem{luong2018joint}
{\color{blue}Luong, Nguyen Cong and Anh, Tran The and Binh, Huynh Thi Thanh and
  Niyato, Dusit and Kim, Dong In and Liang, Ying-Chang}.
\newblock {\color{blue}Joint Transaction Transmission and Channel Selection in
  Cognitive Radio Based Blockchain Networks: A Deep Reinforcement Learning
  Approach}.
\newblock {\em {\color{blue}arXiv preprint arXiv:1810.10139}},
  {\color{blue}2018}.

\bibitem{li2017intelligent2}
{\color{blue}Li, Xingjian and Fang, Jun and Cheng, Wen and Duan, Huiping and
  Chen, Zhi and Li, Hongbin}.
\newblock {\color{blue}Intelligent Power Control for Spectrum Sharing in
  Cognitive Radios: A Deep Reinforcement Learning Approach}.
\newblock {\em {\color{blue}IEEE access}}, {\color{blue}2018}.

\bibitem{lee2018deep}
{\color{blue}Lee, Woongsup and Kim, Minhoe and Cho, Dong-Ho}.
\newblock {\color{blue}Deep Learning Based Transmit Power Control in Underlaid
  Device-to-Device Communication}.
\newblock {\em {\color{blue}IEEE Systems Journal}}, {\color{blue}2018}.

\bibitem{liu2018energy}
{\color{blue}Liu, Chi Harold and Chen, Zheyu and Tang, Jian and Xu, Jie and
  Piao, Chengzhe}.
\newblock {\color{blue}Energy-efficient {UAV} control for effective and fair
  communication coverage: A deep reinforcement learning approach}.
\newblock {\em {\color{blue}IEEE Journal on Selected Areas in Communications}},
  {\color{blue}36}({\color{blue}9}):{\color{blue}2059--2070},
  {\color{blue}2018}.

\bibitem{he2017software}
{\color{blue}He, Ying and Yu, F Richard and Zhao, Nan and Leung, Victor CM and
  Yin, Hongxi}.
\newblock {\color{blue}Software-defined networks with mobile edge computing and
  caching for smart cities: A big data deep reinforcement learning approach}.
\newblock {\em {\color{blue}IEEE Communications Magazine}},
  {\color{blue}55}({\color{blue}12}):{\color{blue}31--37}, {\color{blue}2017}.

\bibitem{liu2018anti}
{\color{blue}Liu, Xin and Xu, Yuhua and Jia, Luliang and Wu, Qihui and
  Anpalagan, Alagan}.
\newblock {\color{blue}Anti-jamming Communications Using Spectrum Waterfall: A
  Deep Reinforcement Learning Approach}.
\newblock {\em {\color{blue}IEEE Communications Letters}},
  {\color{blue}22}({\color{blue}5}):{\color{blue}998--1001},
  {\color{blue}2018}.

\bibitem{pham2018deep}
{\color{blue}Pham, Quang Tran Anh and Hadjadj-Aoul, Yassine and Outtagarts,
  Abdelkader}.
\newblock {\color{blue}Deep Reinforcement Learning based {QoS}-aware Routing in
  Knowledge-defined networking}.
\newblock In {\em {\color{blue}Qshine EAI International Conference on
  Heterogeneous Networking for Quality, Reliability, Security and Robustness}},
  pages~{\color{blue}1--13}, {\color{blue}2018}.

\bibitem{ferreira2016multi}
{\color{blue}Ferreira, Paulo and Paffenroth, Randy and Wyglinski, Alexander and
  Hackett, Timothy M and Bil{\'e}n, Sven and Reinhart, Richard and Mortensen,
  Dale}.
\newblock {\color{blue}Multi-Objective Reinforcement Learning for Cognitive
  Radio--Based Satellite Communications}.
\newblock In {\em {\color{blue}34th AIAA International Communications Satellite
  Systems Conference}}, page~{\color{blue}5726}, {\color{blue}2016}.

\bibitem{yousefi2017autoencoder}
Mahmood Yousefi-Azar, Vijay Varadharajan, Len Hamey, and Uday Tupakula.
\newblock Autoencoder-based feature learning for cyber security applications.
\newblock In {\em IEEE International Joint Conference on Neural Networks
  (IJCNN)}, pages 3854--3861, 2017.

\bibitem{aminanto2016detecting}
Muhamad~Erza Aminanto and Kwangjo Kim.
\newblock Detecting impersonation attack in {WiFi} networks using deep learning
  approach.
\newblock In {\em International Workshop on Information Security Applications},
  pages 136--147. Springer, 2016.

\bibitem{feng2016anomaly}
Qingsong Feng, Zheng Dou, Chunmei Li, and Guangzhen Si.
\newblock Anomaly detection of spectrum in wireless communication via deep
  autoencoder.
\newblock In {\em International Conference on Computer Science and its
  Applications}, pages 259--265. Springer, 2016.

\bibitem{khan2016distributed}
Muhammad~Altaf Khan, Shafiullah Khan, Bilal Shams, and Jaime Lloret.
\newblock Distributed flood attack detection mechanism using artificial neural
  network in wireless mesh networks.
\newblock {\em Security and Communication Networks}, 9(15):2715--2729, 2016.

\bibitem{diro2017distributed}
Abebe~Abeshu Diro and Naveen Chilamkurti.
\newblock Distributed attack detection scheme using deep learning approach for
  {Internet of Things}.
\newblock {\em Future Generation Computer Systems}, 2017.

\bibitem{saied2016detection}
Alan Saied, Richard~E Overill, and Tomasz Radzik.
\newblock Detection of known and unknown {DDoS} attacks using artificial neural
  networks.
\newblock {\em Neurocomputing}, 172:385--393, 2016.

\bibitem{lopez2017conditional}
Manuel Lopez-Martin, Belen Carro, Antonio Sanchez-Esguevillas, and Jaime
  Lloret.
\newblock Conditional variational autoencoder for prediction and feature
  recovery applied to intrusion detection in {IoT}.
\newblock {\em Sensors}, 17(9):1967, 2017.

\bibitem{hamedani2018reservoir}
\color{black}{Hamedani, Kian and Liu, Lingjia and Atat, Rachad and Wu, Jinsong
  and Yi, Yang}.
\newblock Reservoir computing meets smart grids: attack detection using delayed
  feedback networks.
\newblock {\em IEEE Transactions on Industrial Informatics}, 14(2):734--743,
  2018\color{black}.

\bibitem{das2018deep}
\color{black}{Das, Rajshekhar and Gadre, Akshay and Zhang, Shanghang and Kumar,
  Swarun and Moura, Jose MF}.
\newblock A deep learning approach to {IoT} authentication.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{jiang2018virtual}
\color{black}{Jiang, Peng and Wu, Hongyi and Wang, Cong and Xin, Chunsheng}.
\newblock Virtual {MAC} spoofing detection through deep learning.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{yuan2014droid}
Zhenlong Yuan, Yongqiang Lu, Zhaoguo Wang, and Yibo Xue.
\newblock {Droid-Sec}: deep learning in {Android} malware detection.
\newblock In {\em ACM SIGCOMM Computer Communication Review}, volume~44, pages
  371--372, 2014.

\bibitem{yuan2016droiddetector}
Zhenlong Yuan, Yongqiang Lu, and Yibo Xue.
\newblock Droiddetector: {Android} malware characterization and detection using
  deep learning.
\newblock {\em Tsinghua Science and Technology}, 21(1):114--123, 2016.

\bibitem{su2016deep}
Xin Su, Dafang Zhang, Wenjia Li, and Kai Zhao.
\newblock A deep learning approach to {Android} malware feature learning and
  detection.
\newblock In {\em IEEE Trustcom/BigDataSE/ISPA}, pages 244--251, 2016.

\bibitem{hou2016deep4maldroid}
Shifu Hou, Aaron Saas, Lifei Chen, and Yanfang Ye.
\newblock {Deep4MalDroid}: A deep learning framework for {Android} malware
  detection based on linux kernel system call graphs.
\newblock In {\em IEEE/WIC/ACM International Conference on Web Intelligence
  Workshops (WIW)}, pages 104--111, 2016.

\bibitem{martinelli2017evaluating}
Fabio Martinelli, Fiammetta Marulli, and Francesco Mercaldo.
\newblock Evaluating convolutional neural network for effective mobile malware
  detection.
\newblock {\em Procedia Computer Science}, 112:2372--2381, 2017.

\bibitem{nguyen2018cyberattack}
{\color{blue}Nguyen, Khoi Khac and Hoang, Dinh Thai and Niyato, Dusit and Wang,
  Ping and Nguyen, Diep and Dutkiewicz, Eryk}.
\newblock {\color{blue}Cyberattack detection in mobile cloud computing: A deep
  learning approach}.
\newblock In {\em {\color{blue}IEEE Wireless Communications and Networking
  Conference (WCNC)}}, pages~{\color{blue}1--6}, {\color{blue}2018}.

\bibitem{mclaughlin2017deep}
Niall McLaughlin, Jesus Martinez~del Rincon, BooJoong Kang, Suleiman Yerima,
  Paul Miller, Sakir Sezer, Yeganeh Safaei, Erik Trickel, Ziming Zhao, Adam
  Doup{\'e}, et~al.
\newblock Deep android malware detection.
\newblock In {\em Proceedings of the Seventh ACM on Conference on Data and
  Application Security and Privacy}, pages 301--308, 2017.

\bibitem{chen2017deep123}
Yuanfang Chen, Yan Zhang, and Sabita Maharjan.
\newblock Deep learning for secure mobile edge computing.
\newblock {\em arXiv preprint arXiv:1709.08025}, 2017.

\bibitem{oulehla2016detection}
Milan Oulehla, Zuzana~Kom{\'\i}nkov{\'a} Oplatkov{\'a}, and David Malanik.
\newblock Detection of mobile botnets using neural networks.
\newblock In {\em IEEE Future Technologies Conference (FTC)}, pages 1324--1326,
  2016.

\bibitem{torres2016analysis}
Pablo Torres, Carlos Catania, Sebastian Garcia, and Carlos~Garcia Garino.
\newblock An analysis of recurrent neural networks for botnet detection
  behavior.
\newblock In {\em IEEE Biennial Congress of Argentina (ARGENCON)}, pages 1--6,
  2016.

\bibitem{eslahi2016mobile}
Meisam Eslahi, Moslem Yousefi, Maryam~Var Naseri, YM~Yussof, NM~Tahir, and
  H~Hashim.
\newblock Mobile botnet detection model based on retrospective pattern
  recognition.
\newblock {\em International Journal of Security and Its Applications},
  10(9):39--+, 2016.

\bibitem{alauthaman2016p2p}
Mohammad Alauthaman, Nauman Aslam, Li~Zhang, Rafe Alasem, and MA~Hossain.
\newblock A p2p botnet detection scheme based on decision tree and adaptive
  multilayer neural networks.
\newblock {\em Neural Computing and Applications}, pages 1--14, 2016.

\bibitem{shokri2015privacy}
Reza Shokri and Vitaly Shmatikov.
\newblock Privacy-preserving deep learning.
\newblock In {\em Proceedings of the 22nd ACM SIGSAC conference on computer and
  communications security}, pages 1310--1321, 2015.

\bibitem{aono2017privacy}
Yoshinori Aono, Takuya Hayashi, Lihua Wang, Shiho Moriai, et~al.
\newblock Privacy-preserving deep learning: Revisited and enhanced.
\newblock In {\em International Conference on Applications and Techniques in
  Information Security}, pages 100--110. Springer, 2017.

\bibitem{ossia2017hybrid}
Seyed~Ali Ossia, Ali~Shahin Shamsabadi, Ali Taheri, Hamid~R Rabiee, Nic Lane,
  and Hamed Haddadi.
\newblock A hybrid deep learning architecture for privacy-preserving mobile
  analytics.
\newblock {\em arXiv preprint arXiv:1703.02952}, 2017.

\bibitem{abadi2016deep}
Mart{\'\i}n Abadi, Andy Chu, Ian Goodfellow, H~Brendan McMahan, Ilya Mironov,
  Kunal Talwar, and Li~Zhang.
\newblock Deep learning with differential privacy.
\newblock In {\em Proceedings of the ACM SIGSAC Conference on Computer and
  Communications Security}, pages 308--318. ACM, 2016.

\bibitem{osia2017privacy}
Seyed~Ali Osia, Ali~Shahin Shamsabadi, Ali Taheri, Kleomenis Katevas, Hamed
  Haddadi, and Hamid~R Rabiee.
\newblock Private and scalable personal data analytics using a hybrid
  edge-cloud deep learning.
\newblock {\em IEEE Computer Magazine Special Issue on Mobile and Embedded Deep
  Learning}, 2018.

\bibitem{servia2017personal}
Sandra Servia-Rodriguez, Liang Wang, Jianxin~R Zhao, Richard Mortier, and Hamed
  Haddadi.
\newblock Personal model training under privacy constraints.
\newblock In {\em Proceedings of the 3rd ACM/IEEE International Conference on
  Internet-of-Things Design and Implementation}, Apr 2018.

\bibitem{hitaj2017deep}
Briland Hitaj, Giuseppe Ateniese, and Fernando Perez-Cruz.
\newblock Deep models under the {GAN}: information leakage from collaborative
  deep learning.
\newblock In {\em Proceedings of the ACM SIGSAC Conference on Computer and
  Communications Security}, pages 603--618, 2017.

\bibitem{greydanus2017learning}
Sam Greydanus.
\newblock Learning the enigma with recurrent neural networks.
\newblock {\em arXiv preprint arXiv:1708.07576}, 2017.

\bibitem{maghrebi2016breaking}
Houssem Maghrebi, Thibault Portigliatti, and Emmanuel Prouff.
\newblock Breaking cryptographic implementations using deep learning
  techniques.
\newblock In {\em International Conference on Security, Privacy, and Applied
  Cryptography Engineering}, pages 3--26. Springer, 2016.

\bibitem{liu2018genpass}
\color{black}{Liu, Yunyu and Xia, Zhiyang and Yi, Ping and Yao, Yao and Xie,
  Tiantian and Wang, Wei and Zhu, Ting}.
\newblock G{ENPass}: A general deep learning model for password guessing with
  {PCFG} rules and adversarial generation.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{ning2018deepmag}
{\color{blue}Ning, Rui and Wang, Cong and Xin, ChunSheng and Li, Jiang and Wu,
  Hongyi}.
\newblock {\color{blue}DeepMag: sniffing mobile apps in magnetic field through
  deep convolutional neural networks}.
\newblock In {\em {\color{blue}IEEE International Conference on Pervasive
  Computing and Communications (PerCom)}}, pages~{\color{blue}1--10},
  {\color{blue}2018}.

\bibitem{o2017deep}
Timothy~J O'Shea, Tugba Erpek, and T~Charles Clancy.
\newblock Deep learning based {MIMO} communications.
\newblock {\em arXiv preprint arXiv:1707.07980}, 2017.

\bibitem{borgerding2017amp}
Mark Borgerding, Philip Schniter, and Sundeep Rangan.
\newblock {AMP}-inspired deep networks for sparse linear inverse problems.
\newblock {\em IEEE Transactions on Signal Processing}, 2017.

\bibitem{fujihashi2018nonlinear}
\color{black}{Fujihashi, Takuya and Koike-Akino, Toshiaki and Watanabe, Takashi
  and Orlik, Philip V}.
\newblock Nonlinear equalization with deep learning for multi-purpose visual
  {MIMO} communications.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{rajendran2017distributed}
Sreeraj Rajendran, Wannes Meert, Domenico Giustiniano, Vincent Lenders, and
  Sofie Pollin.
\newblock Deep learning models for wireless signal classification with
  distributed low-cost spectrum sensors.
\newblock {\em IEEE Transactions on Cognitive Communications and Networking},
  2018.

\bibitem{west2017deep}
Nathan~E West and Tim O'Shea.
\newblock Deep architectures for modulation recognition.
\newblock In {\em IEEE International Symposium on Dynamic Spectrum Access
  Networks (DySPAN)}, pages 1--6, 2017.

\bibitem{o2016radio}
Timothy~J O'Shea, Latha Pemula, Dhruv Batra, and T~Charles Clancy.
\newblock Radio transformer networks: Attention models for learning to
  synchronize in wireless systems.
\newblock In {\em 50th Asilomar Conference on Signals, Systems and Computers},
  pages 662--666, 2016.

\bibitem{gante2018beamformed}
{\color{blue}Gante, Jo{\~a}o and Falc{\~a}o, Gabriel and Sousa, Leonel}.
\newblock {\color{blue}Beamformed Fingerprint Learning for Accurate Millimeter
  Wave Positioning}.
\newblock {\em {\color{blue}arXiv preprint arXiv:1804.04112}},
  {\color{blue}2018}.

\bibitem{alkhateeb2018deep}
{\color{blue}Alkhateeb, Ahmed and Alex, Sam and Varkey, Paul and Li, Ying and
  Qu, Qi and Tujkovic, Djordje}.
\newblock {\color{blue}Deep Learning Coordinated Beamforming for Highly-Mobile
  Millimeter Wave Systems}.
\newblock {\em {\color{blue}IEEE Access}},
  {\color{blue}6}:{\color{blue}37328--37348}, {\color{blue}2018}.

\bibitem{neumann2017deep}
David Neumann, Wolfgang Utschick, and Thomas Wiese.
\newblock Deep channel estimation.
\newblock In {\em Proceedings of 21th International ITG Workshop on Smart
  Antennas}, pages 1--6. VDE, 2017.

\bibitem{samuel2017deep}
Neev Samuel, Tzvi Diskin, and Ami Wiesel.
\newblock Deep {MIMO} detection.
\newblock {\em arXiv preprint arXiv:1706.01151}, 2017.

\bibitem{yan2017signal}
Xin Yan, Fei Long, Jingshuai Wang, Na~Fu, Weihua Ou, and Bin Liu.
\newblock Signal detection of {MIMO-OFDM} system based on auto encoder and
  extreme learning machine.
\newblock In {\em IEEE International Joint Conference on Neural Networks
  (IJCNN)}, pages 1602--1606, 2017.

\bibitem{timothy2017introduction}
Timothy O'Shea and Jakob Hoydis.
\newblock An introduction to deep learning for the physical layer.
\newblock {\em IEEE Transactions on Cognitive Communications and Networking},
  3(4):563--575, 2017.

\bibitem{jagannath2018artificial}
\color{black}{Jagannath, Jithin and Polosky, Nicholas and O'Connor, Daniel and
  Theagarajan, Lakshmi N and Sheaffer, Brendan and Foulke, Svetlana and
  Varshney, Pramod K}.
\newblock Artificial neural network based automatic modulation classification
  over a software defined radio testbed.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{o2016end}
Timothy~J O'Shea, Seth Hitefield, and Johnathan Corgan.
\newblock End-to-end radio traffic sequence recognition with recurrent neural
  networks.
\newblock In {\em IEEE Global Conference on Signal and Information Processing
  (GlobalSIP)}, pages 277--281, 2016.

\bibitem{o2016learning}
Timothy~J O'Shea, Kiran Karra, and T~Charles Clancy.
\newblock Learning to communicate: Channel auto-encoders, domain specific
  regularizers, and attention.
\newblock In {\em IEEE International Symposium on Signal Processing and
  Information Technology (ISSPIT)}, pages 223--228, 2016.

\bibitem{ye2018power}
\color{black}{Ye, Hao and Li, Geoffrey Ye and Juang, Biing-Hwang}.
\newblock Power of deep learning for channel estimation and signal detection in
  {OFDM} systems.
\newblock {\em IEEE Wireless Communications Letters}, 7(1):114--117,
  2018\color{black}.

\bibitem{liang2018exploiting}
\color{black}{Liang, Fei and Shen, Cong and Wu, Feng}.
\newblock Exploiting noise correlation for channel decoding with convolutional
  neural networks.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{lyu2018performance}
\color{black}{Lyu, Wei and Zhang, Zhaoyang and Jiao, Chunxu and Qin, Kangjian
  and Zhang, Huazi}.
\newblock Performance evaluation of channel decoding with deep neural networks.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{dorner2017deep}
Sebastian Dorner, Sebastian Cammerer, Jakob Hoydis, and Stephan ten Brink.
\newblock On deep learning-based communication over the air.
\newblock In {\em 51st IEEE Asilomar Conference on Signals, Systems, and
  Computers}, pages 1791--1795, 2017.

\bibitem{liao2018rayleigh}
{\color{blue}Liao, Run-Fa and Wen, Hong and Wu, Jinsong and Song, Huanhuan and
  Pan, Fei and Dong, Lian}.
\newblock {\color{blue}The Rayleigh Fading Channel Prediction via Deep
  Learning}.
\newblock {\em {\color{blue}Wireless Communications and Mobile Computing}},
  {\color{blue}2018}.

\bibitem{huang2018deep}
{\color{blue}Huang, Hongji and Yang, Jie and Song, Yiwei and Huang, Hao and
  Gui, Guan}.
\newblock {\color{blue}Deep Learning for Super-Resolution Channel Estimation
  and {DOA} Estimation based Massive {MIMO} System}.
\newblock {\em {\color{blue}IEEE Transactions on Vehicular Technology}},
  {\color{blue}2018}.

\bibitem{huang2018fully}
{\color{blue}Huang, Sihao and Lin, Haowen}.
\newblock {\color{blue}{Fully optical spacecraft communications: implementing
  an omnidirectional PV-cell receiver and 8 Mb/s LED visible light downlink
  with deep learning error correction}}.
\newblock {\em {\color{blue}IEEE Aerospace and Electronic Systems Magazine}},
  {\color{blue}33}({\color{blue}4}):{\color{blue}16--22}, {\color{blue}2018}.

\bibitem{qian2018wireless}
{\color{blue}Qian, Yuchen and Xing, Yuan and Dong, Liang}.
\newblock {\color{blue}Wireless transmission design with neural network for
  radio-frequency energy harvesting}.
\newblock In {\em {\color{blue}IEEE Wireless Communications and Networking
  Conference (WCNC)}}, pages~{\color{blue}1--6}, {\color{blue}2018}.

\bibitem{gonzalez2017network}
Roberto Gonzalez, Alberto Garcia-Duran, Filipe Manco, Mathias Niepert, and
  Pelayo Vallina.
\newblock Network data monetization using {Net2Vec}.
\newblock In {\em Proceedings of the ACM SIGCOMM Posters and Demos}, pages
  37--39, 2017.

\bibitem{kaminski2017neural}
Nichoas Kaminski, Irene Macaluso, Emanuele Di~Pascale, Avishek Nag, John Brady,
  Mark Kelly, Keith Nolan, Wael Guibene, and Linda Doyle.
\newblock A neural-network-based realization of in-network computation for the
  {Internet of Things}.
\newblock In {\em 2017 IEEE International Conference on Communications (ICC)},
  pages 1--6.

\bibitem{xiao2017secure}
Liang Xiao, Yanda Li, Guoan Han, Huaiyu Dai, and H~Vincent Poor.
\newblock A secure mobile crowdsensing game with deep reinforcement learning.
\newblock {\em IEEE Transactions on Information Forensics and Security}, 2017.

\bibitem{luong2018optimal}
\color{black}{Luong, Nguyen Cong and Xiong, Zehui and Wang, Ping and Niyato,
  Dusit}.
\newblock Optimal auction for edge computing resource management in mobile
  blockchain networks: A deep learning approach.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{gulati2018deep}
\color{black}{Gulati, Amuleen and Aujla, Gagangeet Singh and Chaudhary, Rajat
  and Kumar, Neeraj and Obaidat, Mohammad S}.
\newblock Deep learning-based content centric data dissemination scheme for
  {Internet of Vehicles}.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{tsai2018caching}
{\color{blue}Tsai, Kuo Chun and Wang, Li Liliane and Han, Zhu}.
\newblock {\color{blue}Caching for Mobile Social Networks with Deep Learning:
  {Twitter} Analysis for 2016 {U.S.} Election}.
\newblock {\em {\color{blue}IEEE Transactions on Network Science and
  Engineering}}, {\color{blue}2018}.

\bibitem{ahmed2018recent}
{\color{blue}Ahmed, Ejaz and Yaqoob, Ibrar and Hashem, Ibrahim Abaker Targio
  and Shuja, Junaid and Imran, Muhammad and Guizani, Nadra and Bakhsh, Sheikh
  Tahir}.
\newblock {\color{blue}Recent Advances and Challenges in Mobile Big Data}.
\newblock {\em {\color{blue}IEEE Communications Magazine}},
  {\color{blue}56}({\color{blue}2}):{\color{blue}102--108}, {\color{blue}2018}.

\bibitem{yazti2014mobile}
Demetrios~Zeinalipour Yazti and Shonali Krishnaswamy.
\newblock Mobile big data analytics: research, practice, and opportunities.
\newblock In {\em 15th IEEE International Conference on Mobile Data Management
  (MDM)}, volume~1, pages 1--2, 2014.

\bibitem{naboulsi2016large}
Diala Naboulsi, Marco Fiore, Stephane Ribot, and Razvan Stanica.
\newblock Large-scale mobile traffic analysis: a survey.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 18(1):124--161, 2016.

\bibitem{ngiam2011multimodal}
Jiquan Ngiam, Aditya Khosla, Mingyu Kim, Juhan Nam, Honglak Lee, and Andrew~Y
  Ng.
\newblock Multimodal deep learning.
\newblock In {\em Proceedings of the 28th international conference on machine
  learning (ICML)}, pages 689--696, 2011.

\bibitem{alawe2018improving}
{\color{blue}Alawe, Imad and Ksentini, Adlen and Hadjadj-Aoul, Yassine and
  Bertin, Philippe}.
\newblock {\color{blue}Improving traffic forecasting for {5G} core network
  scalability: A Machine Learning approach}.
\newblock {\em {\color{blue}IEEE Network}},
  {\color{blue}32}({\color{blue}6}):{\color{blue}42--49}, {\color{blue}2018}.

\bibitem{aceto2018mobile}
\color{black}{Aceto, Giuseppe and Ciuonzo, Domenico and Montieri, Antonio and
  Pescap{\'e}, Antonio}.
\newblock Mobile encrypted traffic classification using deep learning.
\newblock In {\em 2nd IEEE Network Traffic Measurement and Analysis
  Conference}, 2018\color{black}.

\bibitem{al2015internet}
Ala Al-Fuqaha, Mohsen Guizani, Mehdi Mohammadi, Mohammed Aledhari, and Moussa
  Ayyash.
\newblock Internet of things: A survey on enabling technologies, protocols, and
  applications.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 17(4):2347--2376,
  2015.

\bibitem{seneviratne2017survey}
Suranga Seneviratne, Yining Hu, Tham Nguyen, Guohao Lan, Sara Khalifa, Kanchana
  Thilakarathna, Mahbub Hassan, and Aruna Seneviratne.
\newblock A survey of wearable devices and challenges.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 19(4):2573--2620,
  2017.

\bibitem{li2018learning}
He~Li, Kaoru Ota, and Mianxiong Dong.
\newblock Learning {IoT} in edge: Deep learning for the {Internet of Things}
  with edge computing.
\newblock {\em IEEE Network}, 32(1):96--101, 2018.

\bibitem{lane2015early}
Nicholas~D Lane, Sourav Bhattacharya, Petko Georgiev, Claudio Forlivesi, and
  Fahim Kawsar.
\newblock An early resource characterization of deep learning on wearables,
  smartphones and internet-of-things devices.
\newblock In {\em Proceedings of the ACM International Workshop on Internet of
  Things towards Applications}, pages 7--12, 2015.

\bibitem{ravi2017deep}
Daniele Rav{\`\i}, Charence Wong, Fani Deligianni, Melissa Berthelot, Javier
  Andreu-Perez, Benny Lo, and Guang-Zhong Yang.
\newblock Deep learning for health informatics.
\newblock {\em IEEE journal of biomedical and health informatics}, 21(1):4--21,
  2017.

\bibitem{miotto2017deep}
Riccardo Miotto, Fei Wang, Shuang Wang, Xiaoqian Jiang, and Joel~T Dudley.
\newblock Deep learning for healthcare: review, opportunities and challenges.
\newblock {\em Briefings in Bioinformatics}, 2017.

\bibitem{ronao2016human}
Charissa~Ann Ronao and Sung-Bae Cho.
\newblock Human activity recognition with smartphone sensors using deep
  learning neural networks.
\newblock {\em Expert Systems with Applications}, 59:235--244, 2016.

\bibitem{wang2017deep}
Jindong Wang, Yiqiang Chen, Shuji Hao, Xiaohui Peng, and Lisha Hu.
\newblock Deep learning for sensor-based activity recognition: A survey.
\newblock {\em Pattern Recognition Letters}, 2018.

\bibitem{ran2017delivering}
Xukan Ran, Haoliang Chen, Zhenming Liu, and Jiasi Chen.
\newblock Delivering deep learning to mobile devices via offloading.
\newblock In {\em Proceedings of the ACM Workshop on Virtual Reality and
  Augmented Reality Network}, pages 42--47, 2017.

\bibitem{vyas2017survey}
Vishakha~V Vyas, KH~Walse, and RV~Dharaskar.
\newblock A survey on human activity recognition using smartphone.
\newblock {\em International Journal}, 5(3), 2017.

\bibitem{zen2014deep}
Heiga Zen and Andrew Senior.
\newblock Deep mixture density networks for acoustic modeling in statistical
  parametric speech synthesis.
\newblock In {\em IEEE International Conference on Acoustics, Speech and Signal
  Processing (ICASSP)}, pages 3844--3848, 2014.

\bibitem{zhao2016urban}
Kai Zhao, Sasu Tarkoma, Siyuan Liu, and Huy Vo.
\newblock Urban human mobility data mining: An overview.
\newblock In {\em IEEE International Conference on Big Data (Big Data)}, pages
  1911--1920, 2016.

\bibitem{yang2017neural2}
Cheng Yang, Maosong Sun, Wayne~Xin Zhao, Zhiyuan Liu, and Edward~Y Chang.
\newblock A neural network approach to jointly modeling social networks and
  mobile trajectories.
\newblock {\em ACM Transactions on Information Systems (TOIS)}, 35(4):36, 2017.

\bibitem{graves2014neural}
{\color{blue}Graves, Alex and Wayne, Greg and Danihelka, Ivo}.
\newblock {\color{blue}Neural turing machines}.
\newblock {\em {\color{blue}arXiv preprint arXiv:1410.5401}},
  {\color{blue}2014}.

\bibitem{xia2017indoor}
Shixiong Xia, Yi~Liu, Guan Yuan, Mingjun Zhu, and Zhaohui Wang.
\newblock Indoor fingerprint positioning based on {Wi-Fi}: An overview.
\newblock {\em ISPRS International Journal of Geo-Information}, 6(5):135, 2017.

\bibitem{davidson2016survey}
Pavel Davidson and Robert Pich{\'e}.
\newblock A survey of selected indoor positioning methods for smartphones.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 19(2):1347--1370,
  2017.

\bibitem{xiao2012fifs}
Jiang Xiao, Kaishun Wu, Youwen Yi, and Lionel~M Ni.
\newblock {FIFS}: Fine-grained indoor fingerprinting system.
\newblock In {\em 21st International Conference on Computer Communications and
  Networks (ICCCN)}, pages 1--7, 2012.

\bibitem{youssef2005horus}
Moustafa Youssef and Ashok Agrawala.
\newblock The {H}orus {WLAN} location determination system.
\newblock In {\em Proceedings of the 3rd ACM international conference on Mobile
  systems, applications, and services}, pages 205--218, 2005.

\bibitem{brunato2005statistical}
Mauro Brunato and Roberto Battiti.
\newblock Statistical learning theory for location fingerprinting in wireless
  {LANs}.
\newblock {\em Computer Networks}, 47(6):825--845, 2005.

\bibitem{ho2016generative}
Jonathan Ho and Stefano Ermon.
\newblock Generative adversarial imitation learning.
\newblock In {\em Advances in Neural Information Processing Systems}, pages
  4565--4573, 2016.

\bibitem{zorzi2016cobanets}
Michele Zorzi, Andrea Zanella, Alberto Testolin, Michele De~Filippo De~Grazia,
  and Marco Zorzi.
\newblock {COBANETS}: A new paradigm for cognitive communications systems.
\newblock In {\em IEEE International Conference on Computing, Networking and
  Communications (ICNC)}, pages 1--7, 2016.

\bibitem{roopaei2017deep}
Mehdi Roopaei, Paul Rad, and Mo~Jamshidi.
\newblock Deep learning control for complex and large scale cloud systems.
\newblock {\em Intelligent Automation \& Soft Computing}, pages 1--3, 2017.

\bibitem{ferreira2018multi}
{\color{blue}Ferreira, Paulo Victor R and Paffenroth, Randy and Wyglinski,
  Alexander M and Hackett, Timothy M and Bil{\'e}n, Sven G and Reinhart,
  Richard C and Mortensen, Dale J}.
\newblock {\color{blue}Multi-objective Reinforcement Learning for Cognitive
  Satellite Communications using Deep Neural Network Ensembles}.
\newblock {\em {\color{blue}IEEE Journal on Selected Areas in Communications}},
  {\color{blue}2018}.

\bibitem{schaul2015prioritized}
Tom Schaul, John Quan, Ioannis Antonoglou, and David Silver.
\newblock Prioritized experience replay.
\newblock {\em International Conference on Learning Representations (ICLR)},
  2016.

\bibitem{shi2011iteratively}
Qingjiang Shi, Meisam Razaviyayn, Zhi-Quan Luo, and Chen He.
\newblock An iteratively weighted {MMSE} approach to distributed sum-utility
  maximization for a {MIMO} interfering broadcast channel.
\newblock {\em IEEE Transactions on Signal Processing}, 59(9):4331--4340, 2011.

\bibitem{buczak2016survey}
Anna~L Buczak and Erhan Guven.
\newblock A survey of data mining and machine learning methods for cyber
  security intrusion detection.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 18(2):1153--1176,
  2016.

\bibitem{wang2018not}
{\color{blue}Wang, Ji and Zhang, Jianguo and Bao, Weidong and Zhu, Xiaomin and
  Cao, Bokai and Yu, Philip S}.
\newblock {\color{blue}Not just privacy: Improving performance of private deep
  learning in mobile cloud}.
\newblock In {\em {\color{blue}Proceedings of the 24th ACM SIGKDD International
  Conference on Knowledge Discovery \& Data Mining}},
  pages~{\color{blue}2407--2416}, {\color{blue}2018}.

\bibitem{kwon2017survey}
Donghwoon Kwon, Hyunjoo Kim, Jinoh Kim, Sang~C Suh, Ikkyun Kim, and Kuinam~J
  Kim.
\newblock A survey of deep learning-based network anomaly detection.
\newblock {\em Cluster Computing}, pages 1--13, 2017.

\bibitem{tavallaee2009detailed}
Mahbod Tavallaee, Ebrahim Bagheri, Wei Lu, and Ali~A Ghorbani.
\newblock A detailed analysis of the kdd cup 99 data set.
\newblock In {\em Computational Intelligence for Security and Defense
  Applications, 2009. CISDA 2009. IEEE Symposium on}, pages 1--6, 2009.

\bibitem{tam2017evolution}
Kimberly Tam, Ali Feizollah, Nor~Badrul Anuar, Rosli Salleh, and Lorenzo
  Cavallaro.
\newblock The evolution of android malware and {Android} analysis techniques.
\newblock {\em ACM Computing Surveys (CSUR)}, 49(4):76, 2017.

\bibitem{rodriguez2013survey}
Rafael~A Rodr{\'\i}guez-G{\'o}mez, Gabriel Maci{\'a}-Fern{\'a}ndez, and Pedro
  Garc{\'\i}a-Teodoro.
\newblock Survey and taxonomy of botnet research through life-cycle.
\newblock {\em ACM Computing Surveys (CSUR)}, 45(4):45, 2013.

\bibitem{liu2016collaborative}
Menghan Liu, Haotian Jiang, Jia Chen, Alaa Badokhon, Xuetao Wei, and Ming-Chun
  Huang.
\newblock A collaborative privacy-preserving deep learning system in
  distributed mobile environment.
\newblock In {\em IEEE International Conference on Computational Science and
  Computational Intelligence (CSCI)}, pages 192--197, 2016.

\bibitem{chopra2005learning}
Sumit Chopra, Raia Hadsell, and Yann LeCun.
\newblock Learning a similarity metric discriminatively, with application to
  face verification.
\newblock In {\em IEEE Conference on Computer Vision and Pattern Recognition
  (CVPR)}, volume~1, pages 539--546, 2005.

\bibitem{shamsabadi2018}
Ali~Shahin Shamsabadi, Hamed Haddadi, and Andrea Cavallaro.
\newblock Distributed one-class learning.
\newblock In {\em IEEE International Conference on Image Processing (ICIP)},
  2018.

\bibitem{hitaj2017passgan}
Briland Hitaj, Paolo Gasti, Giuseppe Ateniese, and Fernando Perez-Cruz.
\newblock Pass{GAN}: A deep learning approach for password guessing.
\newblock {\em arXiv preprint arXiv:1709.00440}, 2017.

\bibitem{ye2018channel}
{\color{blue}Ye, Hao and Li, Geoffrey Ye and Juang, Biing-Hwang Fred and
  Sivanesan, Kathiravetpillai}.
\newblock {\color{blue}Channel agnostic end-to-end learning based communication
  systems with conditional {GAN}}.
\newblock {\em {\color{blue}arXiv preprint arXiv:1807.00447}},
  {\color{blue}2018}.

\bibitem{gonzalez2017net2vec}
Roberto Gonzalez, Filipe Manco, Alberto Garcia-Duran, Jose Mendes, Felipe
  Huici, Saverio Niccolini, and Mathias Niepert.
\newblock {Net2Vec}: Deep learning for the network.
\newblock In {\em Proceedings of the ACM Workshop on Big Data Analytics and
  Machine Learning for Data Communication Networks}, pages 13--18, 2017.

\bibitem{wolpert1997no}
David~H Wolpert and William~G Macready.
\newblock No free lunch theorems for optimization.
\newblock {\em IEEE transactions on evolutionary computation}, 1(1):67--82,
  1997.

\bibitem{cheng2017survey}
Yu~Cheng, Duo Wang, Pan Zhou, and Tao Zhang.
\newblock Model compression and acceleration for deep neural networks: The
  principles, progress, and challenges.
\newblock {\em IEEE Signal Processing Magazine}, 35(1):126--136, 2018.

\bibitem{lane2017squeezing}
Nicholas~D Lane, Sourav Bhattacharya, Akhil Mathur, Petko Georgiev, Claudio
  Forlivesi, and Fahim Kawsar.
\newblock Squeezing deep learning into mobile and embedded devices.
\newblock {\em IEEE Pervasive Computing}, 16(3):82--88, 2017.

\bibitem{tang2017enabling}
Jie Tang, Dawei Sun, Shaoshan Liu, and Jean-Luc Gaudiot.
\newblock Enabling deep learning on {IoT} devices.
\newblock {\em Computer}, 50(10):92--96, 2017.

\bibitem{wang2018deep}
{\color{blue}Wang, Ji and Cao, Bokai and Yu, Philip and Sun, Lichao and Bao,
  Weidong and Zhu, Xiaomin}.
\newblock {\color{blue}Deep learning towards mobile applications}.
\newblock In {\em {\color{blue}38th IEEE International Conference on
  Distributed Computing Systems (ICDCS)}}, pages~{\color{blue}1385--1393},
  {\color{blue}2018}.

\bibitem{iandola2017squeezenet}
Forrest~N Iandola, Song Han, Matthew~W Moskewicz, Khalid Ashraf, William~J
  Dally, and Kurt Keutzer.
\newblock {SqueezeNet}: {AlexNet}-level accuracy with 50x fewer parameters and<
  0.5 {MB} model size.
\newblock {\em International Conference on Learning Representations (ICLR)},
  2017.

\bibitem{howard2017mobilenets}
Andrew~G Howard, Menglong Zhu, Bo~Chen, Dmitry Kalenichenko, Weijun Wang,
  Tobias Weyand, Marco Andreetto, and Hartwig Adam.
\newblock Mobilenets: Efficient convolutional neural networks for mobile vision
  applications.
\newblock {\em arXiv preprint arXiv:1704.04861}, 2017.

\bibitem{zhang2017shufflenet}
Xiangyu Zhang, Xinyu Zhou, Mengxiao Lin, and Jian Sun.
\newblock {ShuffleNet}: An extremely efficient convolutional neural network for
  mobile devices.
\newblock In {\em The IEEE Conference on Computer Vision and Pattern
  Recognition (CVPR)}, June 2018.

\bibitem{zhang2017tucker}
Qingchen Zhang, Laurence~T Yang, Xingang Liu, Zhikui Chen, and Peng Li.
\newblock A tucker deep computation model for mobile multimedia feature
  learning.
\newblock {\em ACM Transactions on Multimedia Computing, Communications, and
  Applications (TOMM)}, 13(3s):39, 2017.

\bibitem{cao2017mobirnn}
Qingqing Cao, Niranjan Balasubramanian, and Aruna Balasubramanian.
\newblock {MobiRNN}: Efficient recurrent neural network execution on mobile
  {GPU}.
\newblock In {\em Proceedings of the 1st ACM International Workshop on Deep
  Learning for Mobile Systems and Applications}, pages 1--6, 2017.

\bibitem{chen2016deep}
Chun-Fu Chen, Gwo~Giun Lee, Vincent Sritapan, and Ching-Yung Lin.
\newblock Deep convolutional neural network on {iOS} mobile devices.
\newblock In {\em IEEE International Workshop on Signal Processing Systems
  (SiPS)}, pages 130--135, 2016.

\bibitem{rallapalli2016very}
S~Rallapalli, H~Qiu, A~Bency, S~Karthikeyan, R~Govindan, B~Manjunath, and
  R~Urgaonkar.
\newblock Are very deep neural networks feasible on mobile devices.
\newblock {\em IEEE Transactions on Circuits and Systems for Video Technology},
  2016.

\bibitem{lane2016deepx}
Nicholas~D Lane, Sourav Bhattacharya, Petko Georgiev, Claudio Forlivesi, Lei
  Jiao, Lorena Qendro, and Fahim Kawsar.
\newblock {DeepX}: A software accelerator for low-power deep learning inference
  on mobile devices.
\newblock In {\em 15th ACM/IEEE International Conference on Information
  Processing in Sensor Networks (IPSN)}, pages 1--12, 2016.

\bibitem{huynh2017deepmon}
Loc~N Huynh, Rajesh~Krishna Balan, and Youngki Lee.
\newblock {DeepMon}: Building mobile {GPU} deep learning models for continuous
  vision applications.
\newblock In {\em Proceedings of the 15th ACM Annual International Conference
  on Mobile Systems, Applications, and Services}, pages 186--186, 2017.

\bibitem{wu2016quantized}
Jiaxiang Wu, Cong Leng, Yuhang Wang, Qinghao Hu, and Jian Cheng.
\newblock Quantized convolutional neural networks for mobile devices.
\newblock In {\em Proceedings of the IEEE Conference on Computer Vision and
  Pattern Recognition}, pages 4820--4828, 2016.

\bibitem{bhattacharya2016sparsification}
Sourav Bhattacharya and Nicholas~D Lane.
\newblock Sparsification and separation of deep learning layers for constrained
  resource inference on wearables.
\newblock In {\em Proceedings of the 14th ACM Conference on Embedded Network
  Sensor Systems CD-ROM}, pages 176--189, 2016.

\bibitem{cho2017mec}
Minsik Cho and Daniel Brand.
\newblock {MEC}: Memory-efficient convolution for deep neural network.
\newblock In {\em International Conference on Machine Learning (ICML)}, pages
  815--824, 2017.

\bibitem{guo2017pruning}
Jia Guo and Miodrag Potkonjak.
\newblock Pruning filters and classes: Towards on-device customization of
  convolutional neural networks.
\newblock In {\em Proceedings of the 1st ACM International Workshop on Deep
  Learning for Mobile Systems and Applications}, pages 13--17, 2017.

\bibitem{li2017fitcnn}
Shiming Li, Duo Liu, Chaoneng Xiang, Jianfeng Liu, Yingjian Ling, Tianjun Liao,
  and Liang Liang.
\newblock Fitcnn: A cloud-assisted lightweight convolutional neural network
  framework for mobile devices.
\newblock In {\em 23rd IEEE International Conference on Embedded and Real-Time
  Computing Systems and Applications (RTCSA)}, pages 1--6, 2017.

\bibitem{zen2016fast}
Heiga Zen, Yannis Agiomyrgiannakis, Niels Egberts, Fergus Henderson, and
  Przemys{\l}aw Szczepaniak.
\newblock Fast, compact, and high quality {LSTM-RNN} based statistical
  parametric speech synthesizers for mobile devices.
\newblock {\em arXiv preprint arXiv:1606.06061}, 2016.

\bibitem{falcao2017evaluation}
Gabriel Falcao, Lu{\'\i}s~A Alexandre, J~Marques, Xavier Fraz{\~a}o, and Joao
  Maria.
\newblock On the evaluation of energy-efficient deep learning using stacked
  autoencoders on mobile gpus.
\newblock In {\em 25th IEEE Euromicro International Conference on Parallel,
  Distributed and Network-based Processing}, pages 270--273, 2017.

\bibitem{fang2018nestdnn}
{\color{blue}Fang, Biyi and Zeng, Xiao and Zhang, Mi}.
\newblock {\color{blue}{NestDNN}: Resource-Aware Multi-Tenant On-Device Deep
  Learning for Continuous Mobile Vision}.
\newblock In {\em {\color{blue}Proceedings of the 24th ACM Annual International
  Conference on Mobile Computing and Networking}},
  pages~{\color{blue}115--127}, {\color{blue}2018}.

\bibitem{xu2018deepcache}
{\color{blue}Xu, Mengwei and Zhu, Mengze and Liu, Yunxin and Lin, Felix Xiaozhu
  and Liu, Xuanzhe}.
\newblock {\color{blue}{DeepCache}: Principled Cache for Mobile Deep Vision}.
\newblock In {\em {\color{blue}Proceedings of the 24th ACM Annual International
  Conference on Mobile Computing and Networking}},
  pages~{\color{blue}129--144}, {\color{blue}2018}.

\bibitem{liu2018ondemand}
{\color{blue}Liu, Sicong and Lin, Yingyan and Zhou, Zimu and Nan, Kaiming and
  Liu, Hui and Du, Junzhao}.
\newblock {\color{blue}On-Demand Deep Model Compression for Mobile Devices: A
  Usage-Driven Model Selection Framework}.
\newblock In {\em {\color{blue}Proceedings of the 16th ACM Annual International
  Conference on Mobile Systems, Applications, and Services}},
  pages~{\color{blue}389--400}, {\color{blue}2018}.

\bibitem{chen2018tvm}
{\color{blue}Chen, Tianqi and Moreau, Thierry and Jiang, Ziheng and Zheng,
  Lianmin and Yan, Eddie and Shen, Haichen and Cowan, Meghan and Wang, Leyuan
  and Hu, Yuwei and Ceze, Luis and others}.
\newblock {\color{blue}{TVM}: An Automated End-to-End Optimizing Compiler for
  Deep Learning}.
\newblock In {\em {\color{blue}13th USENIX Symposium on Operating Systems
  Design and Implementation (OSDI 18)}}, pages~{\color{blue}578--594},
  {\color{blue}2018}.

\bibitem{yao2018fastdeepiot}
{\color{blue}Yao, Shuochao and Zhao, Yiran and Shao, Huajie and Liu, ShengZhong
  and Liu, Dongxin and Su, Lu and Abdelzaher, Tarek}.
\newblock {\color{blue}{FastDeepIoT}: Towards Understanding and Optimizing
  Neural Network Execution Time on Mobile and Embedded Devices}.
\newblock In {\em {\color{blue}Proceedings of the 16th ACM Conference on
  Embedded Networked Sensor Systems}}, pages~{\color{blue}278--291},
  {\color{blue}2018}.

\bibitem{teerapittayanon2017distributed}
Surat Teerapittayanon, Bradley McDanel, and HT~Kung.
\newblock Distributed deep neural networks over the cloud, the edge and end
  devices.
\newblock In {\em 37th IEEE International Conference on Distributed Computing
  Systems (ICDCS)}, pages 328--339, 2017.

\bibitem{omidshafiei2017deep}
Shayegan Omidshafiei, Jason Pazis, Christopher Amato, Jonathan~P How, and John
  Vian.
\newblock Deep decentralized multi-task multi-agent reinforcement learning
  under partial observability.
\newblock In {\em International Conference on Machine Learning (ICML)}, pages
  2681--2690, 2017.

\bibitem{recht2011hogwild}
Benjamin Recht, Christopher Re, Stephen Wright, and Feng Niu.
\newblock Hogwild: A lock-free approach to parallelizing stochastic gradient
  descent.
\newblock In {\em Advances in neural information processing systems}, pages
  693--701, 2011.

\bibitem{goyal2017accurate}
Priya Goyal, Piotr Doll{\'a}r, Ross Girshick, Pieter Noordhuis, Lukasz
  Wesolowski, Aapo Kyrola, Andrew Tulloch, Yangqing Jia, and Kaiming He.
\newblock Accurate, large {Minibatch SGD}: Training imagenet in 1 hour.
\newblock {\em arXiv preprint arXiv:1706.02677}, 2017.

\bibitem{zhang2016asynchronous}
ShuaiZheng Ruiliang~Zhang and JamesT Kwok.
\newblock Asynchronous distributed semi-stochastic gradient optimization.
\newblock In {\em National Conference on Artificial Intelligence (AAAI)}, 2016.

\bibitem{hardy2017distributed}
Corentin Hardy, Erwan Le~Merrer, and Bruno Sericola.
\newblock Distributed deep learning on edge-devices: feasibility via adaptive
  compression.
\newblock In {\em 16th IEEE International Symposium on Network Computing and
  Applications (NCA)}, pages 1--8, 2017.

\bibitem{pmlr-v54-mcmahan17a}
Brendan McMahan, Eider Moore, Daniel Ramage, Seth Hampson, and Blaise~Aguera
  y~Arcas.
\newblock Communication-efficient learning of deep networks from decentralized
  data.
\newblock In {\em Proceedings of the 20th International Conference on
  Artificial Intelligence and Statistics}, volume~54, pages 1273--1282, Fort
  Lauderdale, FL, USA, 20--22 Apr 2017.

\bibitem{cryptoeprint:2017:281}
Keith Bonawitz, Vladimir Ivanov, Ben Kreuter, Antonio Marcedone, H.~Brendan
  McMahan, Sarvar Patel, Daniel Ramage, Aaron Segal, and Karn Seth.
\newblock Practical secure aggregation for privacy preserving machine learning.
\newblock Cryptology ePrint Archive, Report 2017/281, 2017.
\newblock \url{https://eprint.iacr.org/2017/281}.

\bibitem{gupta2016model}
Suyog Gupta, Wei Zhang, and Fei Wang.
\newblock Model accuracy and runtime tradeoff in distributed deep learning: A
  systematic study.
\newblock In {\em IEEE 16th International Conference on Data Mining (ICDM)},
  pages 171--180, 2016.

\bibitem{mcmahan2017federated}
B~McMahan and Daniel Ramage.
\newblock Federated learning: Collaborative machine learning without
  centralized training data.
\newblock {\em Google Research Blog}, 2017.

\bibitem{furno2017joint}
Angelo Fumo, Marco Fiore, and Razvan Stanica.
\newblock Joint spatial and temporal classification of mobile traffic demands.
\newblock In {\em IEEE Conference on Computer Communications}, pages 1--9,
  2017.

\bibitem{chen2016lifelong}
Zhiyuan Chen and Bing Liu.
\newblock Lifelong machine learning.
\newblock {\em Synthesis Lectures on Artificial Intelligence and Machine
  Learning}, 10(3):1--145, 2016.

\bibitem{lee2016dual}
Sang-Woo Lee, Chung-Yeon Lee, Dong-Hyun Kwak, Jiwon Kim, Jeonghee Kim, and
  Byoung-Tak Zhang.
\newblock Dual-memory deep learning architectures for lifelong learning of
  everyday human behaviors.
\newblock In {\em International Joint Conferences on Artificial Intelligence},
  pages 1669--1675, 2016.

\bibitem{graves2016hybrid}
Alex Graves, Greg Wayne, Malcolm Reynolds, Tim Harley, Ivo Danihelka, Agnieszka
  Grabska-Barwi{\'n}ska, Sergio~G{\'o}mez Colmenarejo, Edward Grefenstette,
  Tiago Ramalho, John Agapiou, et~al.
\newblock Hybrid computing using a neural network with dynamic external memory.
\newblock {\em Nature}, 538(7626):471--476, 2016.

\bibitem{parisi2017lifelong}
German~I Parisi, Jun Tani, Cornelius Weber, and Stefan Wermter.
\newblock Lifelong learning of human actions with deep neural network
  self-organization.
\newblock {\em Neural Networks}, 2017.

\bibitem{tessler2017deep}
Chen Tessler, Shahar Givony, Tom Zahavy, Daniel~J Mankowitz, and Shie Mannor.
\newblock A deep hierarchical approach to lifelong learning in {Minecraft}.
\newblock In {\em National Conference on Artificial Intelligence (AAAI)}, pages
  1553--1561, 2017.

\bibitem{lopez2018deep}
Daniel L{\'o}pez-S{\'a}nchez, Ang{\'e}lica~Gonz{\'a}lez Arrieta, and Juan~M
  Corchado.
\newblock Deep neural networks and transfer learning applied to multimedia web
  mining.
\newblock In {\em 14th International Conference Distributed Computing and
  Artificial Intelligence}, volume 620, page 124. Springer, 2018.

\bibitem{bacstuug2015transfer}
Ejder Ba{\c{s}}tu{\u{g}}, Mehdi Bennis, and M{\'e}rouane Debbah.
\newblock A transfer learning approach for cache-enabled wireless networks.
\newblock In {\em 13th IEEE International Symposium on Modeling and
  Optimization in Mobile, Ad Hoc, and Wireless Networks (WiOpt)}, pages
  161--166, 2015.

\bibitem{fei2006one}
Li~Fei-Fei, Rob Fergus, and Pietro Perona.
\newblock One-shot learning of object categories.
\newblock {\em IEEE transactions on pattern analysis and machine intelligence},
  28(4):594--611, 2006.

\bibitem{palatucci2009zero}
Mark Palatucci, Dean Pomerleau, Geoffrey~E Hinton, and Tom~M Mitchell.
\newblock Zero-shot learning with semantic output codes.
\newblock In {\em Advances in neural information processing systems}, pages
  1410--1418, 2009.

\bibitem{vinyals2016matching}
Oriol Vinyals, Charles Blundell, Tim Lillicrap, Daan Wierstra, et~al.
\newblock Matching networks for one shot learning.
\newblock In {\em Advances in Neural Information Processing Systems}, pages
  3630--3638, 2016.

\bibitem{changpinyo2016synthesized}
Soravit Changpinyo, Wei-Lun Chao, Boqing Gong, and Fei Sha.
\newblock Synthesized classifiers for zero-shot learning.
\newblock In {\em Proceedings of the IEEE Conference on Computer Vision and
  Pattern Recognition}, pages 5327--5336, 2016.

\bibitem{oh2017zero}
Junhyuk Oh, Satinder Singh, Honglak Lee, and Pushmeet Kohli.
\newblock Zero-shot task generalization with multi-task deep reinforcement
  learning.
\newblock In {\em International Conference on Machine Learning (ICML)}, pages
  2661--2670, 2017.

\bibitem{wang2015understanding}
Huandong Wang, Fengli Xu, Yong Li, Pengyu Zhang, and Depeng Jin.
\newblock Understanding mobile traffic patterns of large scale cellular towers
  in urban environment.
\newblock In {\em Proceedings of the ACM Internet Measurement Conference},
  pages 225--238, 2015.

\bibitem{marquez2017apps}
Cristina Marquez, Marco Gramaglia, Marco Fiore, Albert Banchs, Cezary
  Ziemlicki, and Zbigniew Smoreda.
\newblock Not all {Apps} are created equal: Analysis of spatiotemporal
  heterogeneity in nationwide mobile service usage.
\newblock In {\em Proceedings of the 13th ACM Conference on Emerging Networking
  Experiments and Technologies}, 2017.

\bibitem{barlacchi2015multi}
Gianni Barlacchi, Marco De~Nadai, Roberto Larcher, Antonio Casella, Cristiana
  Chitic, Giovanni Torrisi, Fabrizio Antonelli, Alessandro Vespignani, Alex
  Pentland, and Bruno Lepri.
\newblock A multi-source dataset of urban life in the city of {Milan} and the
  province of {Trentino}.
\newblock {\em Scientific data}, 2, 2015.

\bibitem{liu2015urban}
Liang Liu, Wangyang Wei, Dong Zhao, and Huadong Ma.
\newblock Urban resolution: New metric for measuring the quality of urban
  sensing.
\newblock {\em IEEE Transactions on Mobile Computing}, 14(12):2560--2575, 2015.

\bibitem{tikunov2007traffic}
Denis Tikunov and Toshikazu Nishimura.
\newblock Traffic prediction for mobile network using holt-winter's exponential
  smoothing.
\newblock In {\em 15th IEEE International Conference on Software,
  Telecommunications and Computer Networks}, pages 1--5, 2007.

\bibitem{Kim2011}
Hyun-Woo Kim, Jun-Hui Lee, Yong-Hoon Choi, Young-Uk Chung, and Hyukjoon Lee.
\newblock {Dynamic bandwidth provisioning using ARIMA-based traffic forecasting
  for Mobile WiMAX}.
\newblock {\em Computer Communications}, 34(1):99--106, 2011.

\bibitem{charles2017pointnet}
{\color{blue}Charles, R Qi and Su, Hao and Kaichun, Mo and Guibas, Leonidas J}.
\newblock {\color{blue}Pointnet: Deep learning on point sets for {3D}
  classification and segmentation}.
\newblock In {\em {\color{blue}IEEE Conference on Computer Vision and Pattern
  Recognition (CVPR)}}, pages~{\color{blue}77--85}, {\color{blue}2017}.

\bibitem{ioannidou2017deep}
Anastasia Ioannidou, Elisavet Chatzilari, Spiros Nikolopoulos, and Ioannis
  Kompatsiaris.
\newblock Deep learning advances in computer vision with {3D} data: A survey.
\newblock {\em ACM Computing Surveys (CSUR)}, 50(2):20, 2017.

\bibitem{scarselli2009graph}
{\color{blue}Scarselli, Franco and Gori, Marco and Tsoi, Ah Chung and
  Hagenbuchner, Markus and Monfardini, Gabriele}.
\newblock {\color{blue}The graph neural network model}.
\newblock {\em {\color{blue}IEEE Transactions on Neural Networks}},
  {\color{blue}20}({\color{blue}1}):{\color{blue}61--80}, {\color{blue}2009}.

\bibitem{yuan2017temporal}
{\color{blue}Yuan, Yuan and Liang, Xiaodan and Wang, Xiaolong and Yeung,
  Dit-Yan and Gupta, Abhinav}.
\newblock {\color{blue}Temporal Dynamic Graph LSTM for Action-Driven Video
  Object Detection.}
\newblock In {\em {\color{blue}IEEE International Conference on Computer Vision
  (ICCV)}}, pages~{\color{blue}1819--1828}, {\color{blue}2017}.

\bibitem{usama2017unsupervised}
Muhammad Usama, Junaid Qadir, Aunn Raza, Hunain Arif, Kok-Lim~Alvin Yau, Yehia
  Elkhatib, Amir Hussain, and Ala Al-Fuqaha.
\newblock Unsupervised machine learning for networking: Techniques,
  applications and research challenges.
\newblock {\em arXiv preprint arXiv:1709.06599}, 2017.

\bibitem{zhou2017anomaly}
Chong Zhou and Randy~C Paffenroth.
\newblock Anomaly detection with robust deep autoencoders.
\newblock In {\em Proceedings of the 23rd ACM SIGKDD International Conference
  on Knowledge Discovery and Data Mining}, pages 665--674, 2017.

\bibitem{abadi2016learning}
Mart{\'\i}n Abadi and David~G Andersen.
\newblock Learning to protect communications with adversarial neural
  cryptography.
\newblock {\em International Conference on Learning Representations (ICLR)},
  2017.

\bibitem{silver2017mastering}
Silver David, Julian Schrittwieser, Karen Simonyan, Ioannis Antonoglou, Aja
  Huang, Arthur Guez, Thomas Hubert, Lucas Baker, Matthew Lai, Adrian Bolton,
  Yutian Chen, Timothy Lillicrap, Fan Hui, Laurent Sifre, George van~den
  Driessche, Graepel Thore, and Demis Hassabis.
\newblock Mastering the game of {Go} without human knowledge.
\newblock {\em Nature}, 550(7676):354--359, 2017.

\bibitem{Silver1140}
{\color{blue}Silver, David and Hubert, Thomas and Schrittwieser, Julian and
  Antonoglou, Ioannis and Lai, Matthew and Guez, Arthur and Lanctot, Marc and
  Sifre, Laurent and Kumaran, Dharshan and Graepel, Thore and Lillicrap,
  Timothy and Simonyan, Karen and Hassabis, Demis}.
\newblock {\color{blue}A general reinforcement learning algorithm that masters
  chess, shogi, and {Go} through self-play}.
\newblock {\em {\color{blue}Science}},
  {\color{blue}362}({\color{blue}6419}):{\color{blue}1140--1144},
  {\color{blue}2018}.

\end{thebibliography}


==> revision_v2 (2)/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Communications Society subset of the full
IEEEtran package and is intended for use with IEEE Communications Society
publications. The included version of the IEEEtran_HOWTO.pdf has been
specially formatted in IEEE Communications Society (comsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf,
                   bare_jrnl_comsoc.tex.
***************************************************************************


==> revision_v2 (2)/ref.tex <==
\begin{thebibliography}{100}

\bibitem{cisco2017}
{Cisco}.
\newblock {Cisco Visual Networking Index: Forecast and Methodology, 2016-2021},
  June 2017.

\bibitem{wang2015backhauling}
Ning Wang, Ekram Hossain, and Vijay~K Bhargava.
\newblock Backhauling {5G} small cells: A radio resource management
  perspective.
\newblock {\em IEEE Wireless Communications}, 22(5):41--49, 2015.

\bibitem{giust2015distributed}
Fabio Giust, Luca Cominardi, and Carlos~J Bernardos.
\newblock Distributed mobility management for future {5G} networks: overview
  and analysis of existing approaches.
\newblock {\em IEEE Communications Magazine}, 53(1):142--149, 2015.

\bibitem{agiwal2016next}
Mamta Agiwal, Abhishek Roy, and Navrati Saxena.
\newblock Next generation {5G} wireless networks: A comprehensive survey.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 18(3):1617--1655,
  2016.

\bibitem{gupta2015survey}
Akhil Gupta and Rakesh~Kumar Jha.
\newblock A survey of {5G} network: Architecture and emerging technologies.
\newblock {\em IEEE access}, 3:1206--1232, 2015.

\bibitem{zheng2016big}
Kan Zheng, Zhe Yang, Kuan Zhang, Periklis Chatzimisios, Kan Yang, and Wei
  Xiang.
\newblock Big data-driven optimization for mobile networks toward {5G}.
\newblock {\em IEEE network}, 30(1):44--51, 2016.

\bibitem{jiang2017machine}
Chunxiao Jiang, Haijun Zhang, Yong Ren, Zhu Han, Kwang-Cheng Chen, and Lajos
  Hanzo.
\newblock Machine learning paradigms for next-generation wireless networks.
\newblock {\em IEEE Wireless Communications}, 24(2):98--105, 2017.

\bibitem{nguyen2017reinforcement}
Duong~D Nguyen, Hung~X Nguyen, and Langford~B White.
\newblock Reinforcement learning with network-assisted feedback for
  heterogeneous rat selection.
\newblock {\em IEEE Transactions on Wireless Communications}, 2017.

\bibitem{narudin2016evaluation}
Fairuz~Amalina Narudin, Ali Feizollah, Nor~Badrul Anuar, and Abdullah Gani.
\newblock Evaluation of machine learning classifiers for mobile malware
  detection.
\newblock {\em Soft Computing}, 20(1):343--357, 2016.

\bibitem{hsieh2017gaia}
Kevin Hsieh, Aaron Harlap, Nandita Vijaykumar, Dimitris Konomis, Gregory~R
  Ganger, Phillip~B Gibbons, and Onur Mutlu.
\newblock Gaia: Geo-distributed machine learning approaching {LAN} speeds.
\newblock In {\em USENIX Symposium on Networked Systems Design and
  Implementation (NSDI)}, pages 629--647, 2017.

\bibitem{xiao2017tux2}
Wencong Xiao, Jilong Xue, Youshan Miao, Zhen Li, Cheng Chen, Ming Wu, Wei Li,
  and Lidong Zhou.
\newblock Tux2: Distributed graph computation for machine learning.
\newblock In {\em USENIX Symposium on Networked Systems Design and
  Implementation (NSDI)}, pages 669--682, 2017.

\bibitem{anareport}
{Paolini, Monica and Fili, Senza }.
\newblock {Mastering Analytics: How to benefit from big data and network
  complexity: An Analyst Report}.
\newblock {\em RCR Wireless News}, 2017.

\bibitem{zhang2015convolutional}
{\color{black}Zhang, Chaoyun and Zhou, Pan and Li, Chenghua and Liu, Lijun}.
\newblock {\color{black}A convolutional neural network for leaves recognition
  using data augmentation}.
\newblock In {\em {\color{black}IEEE International Conference on Pervasive
  Intelligence and Computing (PICOM)}}, pages~{\color{black}2143--2150},
  {\color{black}2015}.

\bibitem{socher2012deep}
Richard Socher, Yoshua Bengio, and Christopher~D Manning.
\newblock Deep learning for {NLP} (without magic).
\newblock In {\em Tutorial Abstracts of ACL 2012}, pages 5--5. Association for
  Computational Linguistics.

\bibitem{specialissue}
{IEEE Network special issue: Exploring Deep Learning for Efficient and Reliable
  Mobile Sensing}.
\newblock
  \url{http://www.comsoc.org/netmag/cfp/exploring-deep-learning-efficient-and-reliable-mobile-sensing},
  2017.
\newblock [Online; accessed 14-July-2017].

\bibitem{wang2017machine}
Mowei Wang, Yong Cui, Xin Wang, Shihan Xiao, and Junchen Jiang.
\newblock Machine learning for networking: Workflow, advances and
  opportunities.
\newblock {\em IEEE Network}, 32(2):92--99, 2018.

\bibitem{alsheikh2016mobile}
Mohammad~Abu Alsheikh, Dusit Niyato, Shaowei Lin, Hwee-Pink Tan, and Zhu Han.
\newblock Mobile big data analytics using deep learning and {Apache Spark}.
\newblock {\em IEEE network}, 30(3):22--29, 2016.

\bibitem{goodfellow2016deep}
Ian Goodfellow, Yoshua Bengio, and Aaron Courville.
\newblock {\em Deep learning}.
\newblock MIT press, 2016.

\bibitem{mnih2015human}
Volodymyr Mnih, Koray Kavukcuoglu, David Silver, Andrei~A Rusu, Joel Veness,
  Marc~G Bellemare, Alex Graves, Martin Riedmiller, Andreas~K Fidjeland, Georg
  Ostrovski, et~al.
\newblock Human-level control through deep reinforcement learning.
\newblock {\em Nature}, 518(7540):529--533, 2015.

\bibitem{lecun2015deep}
Yann LeCun, Yoshua Bengio, and Geoffrey Hinton.
\newblock Deep learning.
\newblock {\em Nature}, 521(7553):436--444, 2015.

\bibitem{schmidhuber2015deep}
J{\"u}rgen Schmidhuber.
\newblock Deep learning in neural networks: {An} overview.
\newblock {\em Neural networks}, 61:85--117, 2015.

\bibitem{liu2017survey}
Weibo Liu, Zidong Wang, Xiaohui Liu, Nianyin Zeng, Yurong Liu, and Fuad~E
  Alsaadi.
\newblock A survey of deep neural network architectures and their applications.
\newblock {\em Neurocomputing}, 234:11--26, 2017.

\bibitem{deng2014deep}
Li~Deng, Dong Yu, et~al.
\newblock Deep learning: methods and applications.
\newblock {\em Foundations and Trends{\textregistered} in Signal Processing},
  7(3--4):197--387, 2014.

\bibitem{deng2014tutorial}
Li~Deng.
\newblock A tutorial survey of architectures, algorithms, and applications for
  deep learning.
\newblock {\em APSIPA Transactions on Signal and Information Processing}, 3,
  2014.

\bibitem{Pouyanfar:2018:SDL:3271482.3234150}
{\color{blue}Pouyanfar, Samira and Sadiq, Saad and Yan, Yilin and Tian, Haiman
  and Tao, Yudong and Reyes, Maria Presa and Shyu, Mei-Ling and Chen, Shu-Ching
  and Iyengar, S. S.}
\newblock {\color{blue}A Survey on Deep Learning: Algorithms, Techniques, and
  Applications}.
\newblock {\em {\color{blue}ACM Computing Surveys (CSUR)}},
  {\color{blue}51}({\color{blue}5}):{\color{blue}92:1--92:36},
  {\color{blue}2018}.

\bibitem{kai2017brief}
Kai Arulkumaran, Marc~Peter Deisenroth, Miles Brundage, and Anil~Anthony
  Bharath.
\newblock Deep reinforcement learning: A brief survey.
\newblock {\em IEEE Signal Processing Magazine}, 34(6):26--38, 2017.

\bibitem{hussein2017imitation}
\color{black}{Hussein, Ahmed and Gaber, Mohamed Medhat and Elyan, Eyad and
  Jayne, Chrisina}.
\newblock Imitation learning: A survey of learning methods.
\newblock {\em ACM Computing Surveys (CSUR)}, 50(2):21, 2017\color{black}.

\bibitem{chen2014big}
Xue-Wen Chen and Xiaotong Lin.
\newblock Big data deep learning: challenges and perspectives.
\newblock {\em IEEE access}, 2:514--525, 2014.

\bibitem{najafabadi2015deep}
Maryam~M Najafabadi, Flavio Villanustre, Taghi~M Khoshgoftaar, Naeem Seliya,
  Randall Wald, and Edin Muharemagic.
\newblock Deep learning applications and challenges in big data analytics.
\newblock {\em Journal of Big Data}, 2(1):1, 2015.

\bibitem{hordri2017systematic}
NF~Hordri, A~Samar, SS~Yuhaniz, and SM~Shamsuddin.
\newblock A systematic literature review on features of deep learning in big
  data analytics.
\newblock {\em International Journal of Advances in Soft Computing \& Its
  Applications}, 9(1), 2017.

\bibitem{gheisari2017survey}
Mehdi Gheisari, Guojun Wang, and Md~Zakirul~Alam Bhuiyan.
\newblock A survey on deep learning in big data.
\newblock In {\em IEEE International Conference on Computational Science and
  Engineering (CSE) and Embedded and Ubiquitous Computing (EUC)}, volume~2,
  pages 173--180, 2017.

\bibitem{zhang2017deep}
\color{black}{Zhang, Shuai and Yao, Lina and Sun, Aixin}.
\newblock Deep learning based recommender system: A survey and new
  perspectives.
\newblock {\em arXiv preprint arXiv:1707.07435}, 2017\color{black}.

\bibitem{yu2017networking}
Shui Yu, Meng Liu, Wanchun Dou, Xiting Liu, and Sanming Zhou.
\newblock Networking for big data: A survey.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 19(1):531--549, 2017.

\bibitem{alsheikh2014machine}
Mohammad~Abu Alsheikh, Shaowei Lin, Dusit Niyato, and Hwee-Pink Tan.
\newblock Machine learning in wireless sensor networks: Algorithms, strategies,
  and applications.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 16(4):1996--2018,
  2014.

\bibitem{tsai2014data}
Chun-Wei Tsai, Chin-Feng Lai, Ming-Chao Chiang, Laurence~T Yang, et~al.
\newblock Data mining for {Internet} of things: A survey.
\newblock {\em IEEE Communications Surveys and Tutorials}, 16(1):77--97, 2014.

\bibitem{cheng2017exploiting}
Xiang Cheng, Luoyang Fang, Xuemin Hong, and Liuqing Yang.
\newblock Exploiting mobile big data: Sources, features, and applications.
\newblock {\em IEEE Network}, 31(1):72--79, 2017.

\bibitem{bkassiny2013survey}
Mario Bkassiny, Yang Li, and Sudharman~K Jayaweera.
\newblock A survey on machine-learning techniques in cognitive radios.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 15(3):1136--1159,
  2013.

\bibitem{andrews2014will}
Jeffrey~G Andrews, Stefano Buzzi, Wan Choi, Stephen~V Hanly, Angel Lozano,
  Anthony~CK Soong, and Jianzhong~Charlie Zhang.
\newblock What will {5G} be?
\newblock {\em IEEE Journal on selected areas in communications},
  32(6):1065--1082, 2014.

\bibitem{panwar2016survey}
Nisha Panwar, Shantanu Sharma, and Awadhesh~Kumar Singh.
\newblock A survey on {5G}: The next generation of mobile communication.
\newblock {\em Physical Communication}, 18:64--84, 2016.

\bibitem{elijah2016comprehensive}
Olakunle Elijah, Chee~Yen Leow, Tharek~Abdul Rahman, Solomon Nunoo, and
  Solomon~Zakwoi Iliya.
\newblock A comprehensive survey of pilot contamination in massive {MIMO--5G}
  system.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 18(2):905--923, 2016.

\bibitem{buzzi2016survey}
Stefano Buzzi, I~Chih-Lin, Thierry~E Klein, H~Vincent Poor, Chenyang Yang, and
  Alessio Zappone.
\newblock A survey of energy-efficient techniques for {5G} networks and
  challenges ahead.
\newblock {\em IEEE Journal on Selected Areas in Communications},
  34(4):697--709, 2016.

\bibitem{peng2015system}
Mugen Peng, Yong Li, Zhongyuan Zhao, and Chonggang Wang.
\newblock System architecture and key technologies for {5G} heterogeneous cloud
  radio access networks.
\newblock {\em IEEE network}, 29(2):6--14, 2015.

\bibitem{niu2015survey}
Yong Niu, Yong Li, Depeng Jin, Li~Su, and Athanasios~V Vasilakos.
\newblock A survey of millimeter wave communications (mmwave) for {5G}:
  opportunities and challenges.
\newblock {\em Wireless Networks}, 21(8):2657--2676, 2015.

\bibitem{foukas2017network}
Xenofon Foukas, Georgios Patounas, Ahmed Elmokashfi, and Mahesh~K Marina.
\newblock Network slicing in {5G}: Survey and challenges.
\newblock {\em IEEE Communications Magazine}, 55(5):94--100, 2017.

\bibitem{taleb2017multi}
Tarik Taleb, Konstantinos Samdanis, Badr Mada, Hannu Flinck, Sunny Dutta, and
  Dario Sabella.
\newblock On multi-access edge computing: A survey of the emerging {5G} network
  edge architecture \& orchestration.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 2017.

\bibitem{mach2017mobile}
Pavel Mach and Zdenek Becvar.
\newblock Mobile edge computing: A survey on architecture and computation
  offloading.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 2017.

\bibitem{mao2017survey}
Yuyi Mao, Changsheng You, Jun Zhang, Kaibin Huang, and Khaled~B Letaief.
\newblock A survey on mobile edge computing: The communication perspective.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 2017.

\bibitem{wang2017data}
Ying Wang, Peilong Li, Lei Jiao, Zhou Su, Nan Cheng, Xuemin~Sherman Shen, and
  Ping Zhang.
\newblock A data-driven architecture for personalized {QoE} management in {5G}
  wireless networks.
\newblock {\em IEEE Wireless Communications}, 24(1):102--110, 2017.

\bibitem{han2015mobile}
Qilong Han, Shuang Liang, and Hongli Zhang.
\newblock Mobile cloud sensing, big data, and {5G} networks make an intelligent
  and smart world.
\newblock {\em IEEE Network}, 29(2):40--45, 2015.

\bibitem{singh2017survey}
Sukhdeep Singh, Navrati Saxena, Abhishek Roy, and HanSeok Kim.
\newblock A survey on {5G} network technologies from social perspective.
\newblock {\em IETE Technical Review}, 34(1):30--39, 2017.

\bibitem{chen20175g}
Min Chen, Jun Yang, Yixue Hao, Shiwen Mao, and Kai Hwang.
\newblock A {5G} cognitive system for healthcare.
\newblock {\em Big Data and Cognitive Computing}, 1(1):2, 2017.

\bibitem{chen2015energy}
\color{black}{Chen, Xianfu and Wu, Jinsong and Cai, Yueming and Zhang, Honggang
  and Chen, Tao}.
\newblock {Energy-efficiency oriented traffic offloading in wireless networks:
  A brief survey and a learning approach for heterogeneous cellular networks}.
\newblock {\em IEEE Journal on Selected Areas in Communications},
  33(4):627--640, {2015}\color{black}.

\bibitem{wu2016big}
\color{black}{Wu, Jinsong and Guo, Song and Li, Jie and Zeng, Deze}.
\newblock Big data meet green challenges: big data toward green applications.
\newblock {\em IEEE Systems Journal}, 10(3):888--900, 2016\color{black}.

\bibitem{buda2016can}
Teodora~Sandra Buda, Haytham Assem, Lei Xu, Danny Raz, Udi Margolin, Elisha
  Rosensweig, Diego~R Lopez, Marius-Iulian Corici, Mikhail Smirnov, Robert
  Mullins, et~al.
\newblock Can machine learning aid in delivering new use cases and scenarios in
  {5G}?
\newblock In {\em IEEE/IFIP Network Operations and Management Symposium
  (NOMS)}, pages 1279--1284, 2016.

\bibitem{imran2014challenges}
Ali Imran, Ahmed Zoha, and Adnan Abu-Dayya.
\newblock {Challenges in 5G: how to empower SON with big data for enabling 5G}.
\newblock {\em IEEE Network}, 28(6):27--33, 2014.

\bibitem{keshavamurthy2016conceptual}
Bharath Keshavamurthy and Mohammad Ashraf.
\newblock Conceptual design of proactive {SONs} based on the big data framework
  for {5G} cellular networks: A novel machine learning perspective facilitating
  a shift in the son paradigm.
\newblock In {\em IEEE International Conference on System Modeling \&
  Advancement in Research Trends (SMART)}, pages 298--304, 2016.

\bibitem{valente2017survey}
Paulo Valente~Klaine, Muhammad~Ali Imran, Oluwakayode Onireti, and Richard~Demo
  Souza.
\newblock A survey of machine learning techniques applied to self organizing
  cellular networks.
\newblock {\em IEEE Communications Surveys and Tutorials}, 2017.

\bibitem{li2017intelligent}
Rongpeng Li, Zhifeng Zhao, Xuan Zhou, Guoru Ding, Yan Chen, Zhongyao Wang, and
  Honggang Zhang.
\newblock Intelligent {5G}: When cellular networks meet artificial
  intelligence.
\newblock {\em IEEE Wireless communications}, 24(5):175--183, 2017.

\bibitem{bui2017survey}
Nicola Bui, Matteo Cesana, S~Amir Hosseini, Qi~Liao, Ilaria Malanchini, and
  Joerg Widmer.
\newblock A survey of anticipatory mobile networking: Context-based
  classification, prediction methodologies, and optimization techniques.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 19(3):1790--1821,
  2017.

\bibitem{kasnesis2017changing}
Panagiotis Kasnesis, Charalampos Patrikakis, and Iakovos Venieris.
\newblock Changing the game of mobile data analysis with deep learning.
\newblock {\em IT Professional}, 2017.

\bibitem{cheng2017mobile}
Xiang Cheng, Luoyang Fang, Liuqing Yang, and Shuguang Cui.
\newblock Mobile big data: the fuel for data-driven wireless.
\newblock {\em IEEE Internet of Things Journal}, 4(5):1489--1516, 2017.

\bibitem{wang2017big}
Lidong Wang and Randy Jones.
\newblock Big data analytics for network intrusion detection: A survey.
\newblock {\em International Journal of Networks and Communications},
  7(1):24--31, 2017.

\bibitem{kato2017deep}
Nei Kato, Zubair~Md Fadlullah, Bomin Mao, Fengxiao Tang, Osamu Akashi, Takeru
  Inoue, and Kimihiro Mizutani.
\newblock The deep learning vision for heterogeneous network traffic control:
  proposal, challenges, and future perspective.
\newblock {\em IEEE Wireless Communications}, 24(3):146--153, 2017.

\bibitem{zorzi2015cognition}
Michele Zorzi, Andrea Zanella, Alberto Testolin, Michele De~Filippo De~Grazia,
  and Marco Zorzi.
\newblock Cognition-based networks: A new perspective on network optimization
  using learning and distributed intelligence.
\newblock {\em IEEE Access}, 3:1512--1530, 2015.

\bibitem{fadlullah2017state}
Zubair Fadlullah, Fengxiao Tang, Bomin Mao, Nei Kato, Osamu Akashi, Takeru
  Inoue, and Kimihiro Mizutani.
\newblock State-of-the-art deep learning: Evolving machine intelligence toward
  tomorrow's intelligent network traffic control systems.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 19(4):2432--2455,
  2017.

\bibitem{mohammadi2018deep}
\color{black}{Mohammadi, Mehdi and Al-Fuqaha, Ala and Sorour, Sameh and
  Guizani, Mohsen}.
\newblock {Deep Learning for IoT Big Data and Streaming Analytics: A Survey}.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 2018\color{black}.

\bibitem{ahad2016neural}
Nauman Ahad, Junaid Qadir, and Nasir Ahsan.
\newblock Neural networks in wireless networks: Techniques, applications and
  guidelines.
\newblock {\em Journal of Network and Computer Applications}, 68:1--27, 2016.

\bibitem{mao2018deep}
\color{black}{Mao, Qian and Hu, Fei and Hao, Qi}.
\newblock Deep learning for intelligent wireless networks: A comprehensive
  survey.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 2018\color{black}.

\bibitem{luong2018applications}
{\color{blue}Luong, Nguyen Cong and Hoang, Dinh Thai and Gong, Shimin and
  Niyato, Dusit and Wang, Ping and Liang, Ying-Chang and Kim, Dong In}.
\newblock {\color{blue}Applications of Deep Reinforcement Learning in
  Communications and Networking: A Survey}.
\newblock {\em {\color{blue}arXiv preprint arXiv:1810.07862}},
  {\color{blue}2018}.

\bibitem{zhou2017intelligent2}
\color{black}{Zhou, Xiangwei and Sun, Mingxuan and Li, Ye Geoffrey and Juang,
  Biing-Hwang}.
\newblock {Intelligent Wireless Communications Enabled by Cognitive Radio and
  Machine Learning}.
\newblock {\em arXiv preprint arXiv:1710.11240}, 2017\color{black}.

\bibitem{chen2017machine2}
\color{black}{Chen, Mingzhe and Challita, Ursula and Saad, Walid and Yin,
  Changchuan and Debbah, M{\'e}rouane}.
\newblock Machine learning for wireless networks with artificial intelligence:
  A tutorial on neural networks.
\newblock {\em arXiv preprint arXiv:1710.02913}, 2017\color{black}.

\bibitem{gharaibeh2017smart}
Ammar Gharaibeh, Mohammad~A Salahuddin, Sayed~Jahed Hussini, Abdallah
  Khreishah, Issa Khalil, Mohsen Guizani, and Ala Al-Fuqaha.
\newblock Smart cities: A survey on data management, security, and enabling
  technologies.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 19(4):2456--2501,
  2017.

\bibitem{lane2015can}
Nicholas~D Lane and Petko Georgiev.
\newblock Can deep learning revolutionize mobile sensing?
\newblock In {\em Proceedings of the 16th ACM International Workshop on Mobile
  Computing Systems and Applications}, pages 117--122, 2015.

\bibitem{ota2017deep}
Kaoru Ota, Minh~Son Dao, Vasileios Mezaris, and Francesco~GB De~Natale.
\newblock Deep learning for mobile multimedia: A survey.
\newblock {\em ACM Transactions on Multimedia Computing, Communications, and
  Applications (TOMM)}, 13(3s):34, 2017.

\bibitem{mishra2018detailed}
\color{black}{Mishra, Preeti and Varadharajan, Vijay and Tupakula, Uday and
  Pilli, Emmanuel S}.
\newblock A detailed investigation and analysis of using machine learning
  techniques for intrusion detection.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 2018\color{black}.

\bibitem{li2017deeprl}
Yuxi Li.
\newblock Deep reinforcement learning: An overview.
\newblock {\em arXiv preprint arXiv:1701.07274}, 2017.

\bibitem{chen2018deep0}
Longbiao Chen, Dingqi Yang, Daqing Zhang, Cheng Wang, Jonathan Li, et~al.
\newblock Deep mobile traffic forecast and complementary base station
  clustering for {C-RAN} optimization.
\newblock {\em Journal of Network and Computer Applications}, 121:59--69, 2018.

\bibitem{mnih2016asynchronous}
Volodymyr Mnih, Adria~Puigdomenech Badia, Mehdi Mirza, Alex Graves, Timothy
  Lillicrap, Tim Harley, David Silver, and Koray Kavukcuoglu.
\newblock Asynchronous methods for deep reinforcement learning.
\newblock In {\em International Conference on Machine Learning (ICML)}, pages
  1928--1937, 2016.

\bibitem{arjovsky2017wasserstein}
Martin Arjovsky, Soumith Chintala, and L{\'e}on Bottou.
\newblock Wasserstein generative adversarial networks.
\newblock In {\em International Conference on Machine Learning}, pages
  214--223, 2017.

\bibitem{damianou2013deep2}
\color{black}{Damianou, Andreas and Lawrence, Neil}.
\newblock Deep {Gaussian} processes.
\newblock In {\em Artificial Intelligence and Statistics}, pages 207--215,
  2013\color{black}.

\bibitem{garnelo2018neural}
\color{black}{Garnelo, Marta and Schwarz, Jonathan and Rosenbaum, Dan and
  Viola, Fabio and Rezende, Danilo J and Eslami, SM and Teh, Yee Whye}.
\newblock Neural processes.
\newblock {\em arXiv preprint arXiv:1807.01622}, 2018\color{black}.

\bibitem{zhou2017deep2}
\color{black}{Zhou, Zhi-Hua and Feng, Ji}.
\newblock Deep forest: towards an alternative to deep neural networks.
\newblock In {\em Proceedings of the 26th International Joint Conference on
  Artificial Intelligence}, pages 3553--3559. AAAI Press, 2017\color{black}.

\bibitem{mcculloch:1943}
W.~McCulloch and W.~Pitts.
\newblock A logical calculus of the ideas immanent in nervous activity.
\newblock {\em Bulletin of Mathematical Biophysics}, (5).

\bibitem{williams1986learning}
David~E Rumelhart, Geoffrey~E Hinton, and Ronald~J Williams.
\newblock Learning representations by back-propagating errors.
\newblock {\em Nature}, 323(6088):533, 1986.

\bibitem{lecun1995convolutional}
Yann LeCun, Yoshua Bengio, et~al.
\newblock Convolutional networks for images, speech, and time series.
\newblock {\em The handbook of brain theory and neural networks},
  3361(10):1995, 1995.

\bibitem{krizhevsky2012imagenet}
Alex Krizhevsky, Ilya Sutskever, and Geoffrey~E Hinton.
\newblock Imagenet classification with deep convolutional neural networks.
\newblock In {\em Advances in neural information processing systems}, pages
  1097--1105, 2012.

\bibitem{Domingos:2012}
Pedro Domingos.
\newblock A few useful things to know about machine learning.
\newblock {\em Communications of the ACM}, 55(10):78--87, 2012.

\bibitem{tsang2005core}
Ivor~W Tsang, James~T Kwok, and Pak-Ming Cheung.
\newblock {Core vector machines: Fast {SVM} training on very large data sets}.
\newblock {\em Journal of Machine Learning Research}, 6:363--392, 2005.

\bibitem{rasmussen2006gaussian}
Carl~Edward Rasmussen and Christopher~KI Williams.
\newblock {\em Gaussian processes for machine learning}, volume~1.
\newblock MIT press Cambridge, 2006.

\bibitem{le2008representational}
Nicolas Le~Roux and Yoshua Bengio.
\newblock Representational power of restricted boltzmann machines and deep
  belief networks.
\newblock {\em Neural computation}, 20(6):1631--1649, 2008.

\bibitem{goodfellow2014generative}
Ian Goodfellow, Jean Pouget-Abadie, Mehdi Mirza, Bing Xu, David Warde-Farley,
  Sherjil Ozair, Aaron Courville, and Yoshua Bengio.
\newblock Generative adversarial nets.
\newblock In {\em Advances in neural information processing systems}, pages
  2672--2680, 2014.

\bibitem{schroff2015facenet}
Florian Schroff, Dmitry Kalenichenko, and James Philbin.
\newblock Facenet: A unified embedding for face recognition and clustering.
\newblock In {\em Proceedings of the IEEE Conference on Computer Vision and
  Pattern Recognition}, pages 815--823, 2015.

\bibitem{kingma2014semi}
Diederik~P Kingma, Shakir Mohamed, Danilo~Jimenez Rezende, and Max Welling.
\newblock Semi-supervised learning with deep generative models.
\newblock In {\em Advances in Neural Information Processing Systems}, pages
  3581--3589, 2014.

\bibitem{stewart2017label}
Russell Stewart and Stefano Ermon.
\newblock Label-free supervision of neural networks with physics and domain
  knowledge.
\newblock In {\em National Conference on Artificial Intelligence (AAAI)}, pages
  2576--2582, 2017.

\bibitem{rezende2016one}
Danilo Rezende, Ivo Danihelka, Karol Gregor, Daan Wierstra, et~al.
\newblock One-shot generalization in deep generative models.
\newblock In {\em International Conference on Machine Learning (ICML)}, pages
  1521--1529, 2016.

\bibitem{socher2013zero}
Richard Socher, Milind Ganjoo, Christopher~D Manning, and Andrew Ng.
\newblock Zero-shot learning through cross-modal transfer.
\newblock In {\em Advances in neural information processing systems}, pages
  935--943, 2013.

\bibitem{georgiev2017low}
Petko Georgiev, Sourav Bhattacharya, Nicholas~D Lane, and Cecilia Mascolo.
\newblock Low-resource multi-task audio sensing for mobile and embedded devices
  via shared deep neural network representations.
\newblock {\em Proceedings of the ACM on Interactive, Mobile, Wearable and
  Ubiquitous Technologies}, 1(3):50, 2017.

\bibitem{monti2017geometric}
{\color{blue}Monti, Federico and Boscaini, Davide and Masci, Jonathan and
  Rodola, Emanuele and Svoboda, Jan and Bronstein, Michael M}.
\newblock {\color{blue}Geometric deep learning on graphs and manifolds using
  mixture model {CNNs}}.
\newblock In {\em {\color{blue}IEEE Conference on Computer Vision and Pattern
  Recognition (CVPR)}}, volume~{\color{blue}1}, page~{\color{blue}3},
  {\color{blue}2017}.

\bibitem{le2004geometric}
{\color{blue}Le Roux, Brigitte and Rouanet, Henry}.
\newblock {\em {\color{blue}Geometric data analysis: from correspondence
  analysis to structured data analysis}}.
\newblock {\color{blue}Springer Science \& Business Media}, {\color{blue}2004}.

\bibitem{qi2017pointnet}
{\color{blue}Qi, Charles Ruizhongtai and Yi, Li and Su, Hao and Guibas,
  Leonidas J}.
\newblock {\color{blue}Pointnet++: Deep hierarchical feature learning on point
  sets in a metric space}.
\newblock In {\em {\color{blue}Advances in Neural Information Processing
  Systems}}, pages~{\color{blue}5099--5108}, {\color{blue}2017}.

\bibitem{kipf2016semi}
{\color{blue}Kipf, Thomas N and Welling, Max}.
\newblock {\color{blue}Semi-supervised classification with graph convolutional
  networks}.
\newblock {\em {\color{blue}International Conference on Learning
  Representations (ICLR)}}, {\color{blue}2017}.

\bibitem{wang2018spatio}
{\color{blue}Wang, Xu and Zhou, Zimu and Xiao, Fu and Xing, Kai and Yang, Zheng
  and Liu, Yunhao and Peng, Chunyi}.
\newblock {\color{blue}Spatio-temporal analysis and prediction of cellular
  traffic in metropolis}.
\newblock {\em {\color{blue}IEEE Transactions on Mobile Computing}},
  {\color{blue}2018}.

\bibitem{nguyen2015deep}
{\color{blue}Nguyen, Anh and Yosinski, Jason and Clune, Jeff}.
\newblock {\color{blue}Deep neural networks are easily fooled: High confidence
  predictions for unrecognizable images}.
\newblock In {\em {\color{blue}Proceedings of the IEEE Conference on Computer
  Vision and Pattern Recognition}}, pages~{\color{blue}427--436},
  {\color{blue}2015}.

\bibitem{behzadan2017vulnerability}
{\color{blue}Behzadan, Vahid and Munir, Arslan}.
\newblock {\color{blue}Vulnerability of deep reinforcement learning to policy
  induction attacks}.
\newblock In {\em {\color{blue}International Conference on Machine Learning and
  Data Mining in Pattern Recognition}}, pages~{\color{blue}262--275}.
  {\color{blue}Springer}, {\color{blue}2017}.

\bibitem{madani2018robustness}
{\color{blue}Madani, Pooria and Vlajic, Natalija}.
\newblock {\color{blue}Robustness of deep autoencoder in intrusion detection
  under adversarial contamination}.
\newblock In {\em {\color{blue}Proceedings of the 5th ACM Annual Symposium and
  Bootcamp on Hot Topics in the Science of Security}}, page~{\color{blue}1},
  {\color{blue}2018}.

\bibitem{bau2017network}
{\color{blue}Bau, David and Zhou, Bolei and Khosla, Aditya and Oliva, Aude and
  Torralba, Antonio}.
\newblock {\color{blue}Network Dissection: Quantifying Interpretability of Deep
  Visual Representations}.
\newblock In {\em {\color{blue}IEEE Conference on Computer Vision and Pattern
  Recognition (CVPR)}}, pages~{\color{blue}3319--3327}, {\color{blue}2017}.

\bibitem{wu2017beyond}
{\color{blue}Wu, Mike and Hughes, Michael C and Parbhoo, Sonali and Zazzi,
  Maurizio and Roth, Volker and Doshi-Velez, Finale}.
\newblock {\color{blue}Beyond sparsity: Tree regularization of deep models for
  interpretability}.
\newblock {\color{blue}2018}.

\bibitem{chakraborty2017interpretability}
{\color{blue}Chakraborty, Supriyo and Tomsett, Richard and Raghavendra, Ramya
  and Harborne, Daniel and Alzantot, Moustafa and Cerutti, Federico and
  Srivastava, Mani and Preece, Alun and Julier, Simon and Rao, Raghuveer M and
  others}.
\newblock {\color{blue}Interpretability of deep learning models: a survey of
  results}.
\newblock In {\em {\color{blue}IEEE Smart World Congress 2017 Workshop: DAIS}},
  {\color{blue}2017}.

\bibitem{perez2017effectiveness}
{\color{blue}Perez, Luis and Wang, Jason}.
\newblock {\color{blue}The effectiveness of data augmentation in image
  classification using deep learning}.
\newblock {\em {\color{blue}arXiv preprint arXiv:1712.04621}},
  {\color{blue}2017}.

\bibitem{liu2017progressive}
\color{black}{Liu, Chenxi and Zoph, Barret and Shlens, Jonathon and Hua, Wei
  and Li, Li-Jia and Fei-Fei, Li and Yuille, Alan and Huang, Jonathan and
  Murphy, Kevin}.
\newblock Progressive neural architecture search.
\newblock {\em arXiv preprint arXiv:1712.00559}, 2017\color{black}.

\bibitem{zhang2016deep3}
Wei Zhang, Kan Liu, Weidong Zhang, Youmei Zhang, and Jason Gu.
\newblock Deep neural networks for wireless localization in indoor and outdoor
  environments.
\newblock {\em Neurocomputing}, 194:279--287, 2016.

\bibitem{ordonez2016deep}
Francisco~Javier Ord{\'o}{\~n}ez and Daniel Roggen.
\newblock Deep convolutional and {LSTM} recurrent neural networks for
  multimodal wearable activity recognition.
\newblock {\em Sensors}, 16(1):115, 2016.

\bibitem{de2016distributed}
Elias De~Coninck, Tim Verbelen, Bert Vankeirsbilck, Steven Bohez, Pieter
  Simoens, Piet Demeester, and Bart Dhoedt.
\newblock Distributed neural networks for {Internet of Things}: the big-little
  approach.
\newblock In {\em Internet of Things. IoT Infrastructures: Second International
  Summit, IoT 360$^{\circ}$ 2015, Rome, Italy, October 27-29, Revised Selected
  Papers, Part II}, pages 484--492. Springer, 2016.

\bibitem{jouppi2017datacenter}
Norman~P Jouppi, Cliff Young, Nishant Patil, David Patterson, Gaurav Agrawal,
  Raminder Bajwa, Sarah Bates, Suresh Bhatia, Nan Boden, Al~Borchers, et~al.
\newblock In-datacenter performance analysis of a tensor processing unit.
\newblock In {\em ACM/IEEE 44th Annual International Symposium on Computer
  Architecture (ISCA)}, pages 1--12, 2017.

\bibitem{nickolls2008scalable}
John Nickolls, Ian Buck, Michael Garland, and Kevin Skadron.
\newblock Scalable parallel programming with {CUDA}.
\newblock {\em Queue}, 6(2):40--53, 2008.

\bibitem{chetlur2014cudnn}
Sharan Chetlur, Cliff Woolley, Philippe Vandermersch, Jonathan Cohen, John
  Tran, Bryan Catanzaro, and Evan Shelhamer.
\newblock {cuDNN}: Efficient primitives for deep learning.
\newblock {\em arXiv preprint arXiv:1410.0759}, 2014.

\bibitem{tensorflow2015-whitepaper}
Mart{\'\i}n Abadi, Paul Barham, Jianmin Chen, Zhifeng Chen, Andy Davis, Jeffrey
  Dean, Matthieu Devin, Sanjay Ghemawat, Geoffrey Irving, Michael Isard, et~al.
\newblock {TensorFlow}: A system for large-scale machine learning.
\newblock In {\em USENIX Symposium on Operating Systems Design and
  Implementation (OSDI)}, volume~16, pages 265--283, 2016.

\bibitem{2016arXiv160502688short}
{Theano Development Team}.
\newblock {Theano: A {Python} framework for fast computation of mathematical
  expressions}.
\newblock {\em arXiv e-prints}, abs/1605.02688, May 2016.

\bibitem{jia2014caffe}
Yangqing Jia, Evan Shelhamer, Jeff Donahue, Sergey Karayev, Jonathan Long, Ross
  Girshick, Sergio Guadarrama, and Trevor Darrell.
\newblock Caffe: Convolutional architecture for fast feature embedding.
\newblock {\em arXiv preprint arXiv:1408.5093}, 2014.

\bibitem{torch}
R.~Collobert, K.~Kavukcuoglu, and C.~Farabet.
\newblock Torch7: A {Matlab}-like environment for machine learning.
\newblock In {\em BigLearn, NIPS Workshop}, 2011.

\bibitem{gokhale2014240}
Vinayak Gokhale, Jonghoon Jin, Aysegul Dundar, Berin Martini, and Eugenio
  Culurciello.
\newblock A 240 {G}-ops/s mobile coprocessor for deep neural networks.
\newblock In {\em Proceedings of the IEEE Conference on Computer Vision and
  Pattern Recognition Workshops}, pages 682--687, 2014.

\bibitem{ncnn}
{ncnn is a high-performance neural network inference framework optimized for
  the mobile platform }.
\newblock \url{https://github.com/Tencent/ncnn}, 2017.
\newblock [Online; accessed 25-July-2017].

\bibitem{huawei2017kirin}
{Huawei announces the {Kirin} 970- new flagship {SoC} with {AI} capabilities}.
\newblock
  \url{http://www.androidauthority.com/huawei-announces-kirin-970-797788/},
  2017.
\newblock [Online; accessed 01-Sep-2017].

\bibitem{coreml}
{Core ML: Integrate machine learning models into your app.}
\newblock \url{https://developer.apple.com/documentation/coreml}, 2017.
\newblock [Online; accessed 25-July-2017].

\bibitem{sutskever2013importance}
Ilya Sutskever, James Martens, George~E Dahl, and Geoffrey~E Hinton.
\newblock On the importance of initialization and momentum in deep learning.
\newblock {\em Proceedings of the international conference on machine learning
  (ICML)}, 28:1139--1147, 2013.

\bibitem{dean2012large}
Jeffrey Dean, Greg Corrado, Rajat Monga, Kai Chen, Matthieu Devin, Mark Mao,
  Andrew Senior, Paul Tucker, Ke~Yang, Quoc~V Le, et~al.
\newblock Large scale distributed deep networks.
\newblock In {\em Advances in neural information processing systems}, pages
  1223--1231, 2012.

\bibitem{kingma2015adam}
Diederik Kingma and Jimmy Ba.
\newblock {Adam: A method for stochastic optimization}.
\newblock {\em International Conference on Learning Representations (ICLR)},
  2015.

\bibitem{kraska2013mlbase}
Tim Kraska, Ameet Talwalkar, John~C Duchi, Rean Griffith, Michael~J Franklin,
  and Michael~I Jordan.
\newblock {MLbase}: A distributed machine-learning system.
\newblock In {\em CIDR}, volume~1, pages 2--1, 2013.

\bibitem{chilimbi2014project}
Trishul~M Chilimbi, Yutaka Suzue, Johnson Apacible, and Karthik Kalyanaraman.
\newblock Project adam: Building an efficient and scalable deep learning
  training system.
\newblock In {\em USENIX Symposium on Operating Systems Design and
  Implementation (OSDI)}, volume~14, pages 571--582, 2014.

\bibitem{cui2016geeps}
Henggang Cui, Hao Zhang, Gregory~R Ganger, Phillip~B Gibbons, and Eric~P Xing.
\newblock Geeps: Scalable deep learning on distributed {GPUs} with a
  {GPU}-specialized parameter server.
\newblock In {\em Proceedings of the Eleventh ACM European Conference on
  Computer Systems}, page~4, 2016.

\bibitem{Lineaat8084}
\color{black}{Lin, Xing and Rivenson, Yair and Yardimci, Nezih T. and Veli,
  Muhammed and Luo, Yi and Jarrahi, Mona and Ozcan, Aydogan}.
\newblock All-optical machine learning using diffractive deep neural networks.
\newblock {\em Science}, 2018\color{black}.

\bibitem{spring2017scalable}
Ryan Spring and Anshumali Shrivastava.
\newblock Scalable and sustainable deep learning via randomized hashing.
\newblock {\em ACM SIGKDD Conference on Knowledge Discovery and Data Mining},
  2017.

\bibitem{mirhoseini2017device}
Azalia Mirhoseini, Hieu Pham, Quoc~V Le, Benoit Steiner, Rasmus Larsen, Yuefeng
  Zhou, Naveen Kumar, Mohammad Norouzi, Samy Bengio, and Jeff Dean.
\newblock Device placement optimization with reinforcement learning.
\newblock {\em International Conference on Machine Learning}, 2017.

\bibitem{xing2015petuum}
Eric~P Xing, Qirong Ho, Wei Dai, Jin~Kyu Kim, Jinliang Wei, Seunghak Lee, Xun
  Zheng, Pengtao Xie, Abhimanu Kumar, and Yaoliang Yu.
\newblock Petuum: A new platform for distributed machine learning on big data.
\newblock {\em IEEE Transactions on Big Data}, 1(2):49--67, 2015.

\bibitem{moritz2018ray}
{\color{blue}Moritz, Philipp and Nishihara, Robert and Wang, Stephanie and
  Tumanov, Alexey and Liaw, Richard and Liang, Eric and Elibol, Melih and Yang,
  Zongheng and Paul, William and Jordan, Michael I and others}.
\newblock {\color{blue}Ray: A Distributed Framework for Emerging {AI}
  Applications}.
\newblock In {\em {\color{blue}13th USENIX Symposium on Operating Systems
  Design and Implementation (OSDI 18)}}, pages~{\color{blue}561--577},
  {\color{blue}2018}.

\bibitem{alzantot2017rstensorflow}
Moustafa Alzantot, Yingnan Wang, Zhengshuang Ren, and Mani~B Srivastava.
\newblock {RSTensorFlow}: {GPU} enabled tensorflow for deep learning on
  commodity {Android} devices.
\newblock In {\em Proceedings of the 1st ACM International Workshop on Deep
  Learning for Mobile Systems and Applications}, pages 7--12, 2017.

\bibitem{tensorlayer}
Hao Dong, Akara Supratak, Luo Mai, Fangde Liu, Axel Oehmichen, Simiao Yu, and
  Yike Guo.
\newblock {TensorLayer}: A versatile library for efficient deep learning
  development.
\newblock In {\em Proceedings of the ACM on Multimedia Conference}, MM '17,
  pages 1201--1204, 2017.

\bibitem{paszke2017automatic}
Adam Paszke, Sam Gross, Soumith Chintala, Gregory Chanan, Edward Yang, Zachary
  DeVito, Zeming Lin, Alban Desmaison, Luca Antiga, and Adam Lerer.
\newblock Automatic differentiation in {PyTorch}.
\newblock 2017.

\bibitem{chen2015mxnet}
Tianqi Chen, Mu~Li, Yutian Li, Min Lin, Naiyan Wang, Minjie Wang, Tianjun Xiao,
  Bing Xu, Chiyuan Zhang, and Zheng Zhang.
\newblock Mxnet: A flexible and efficient machine learning library for
  heterogeneous distributed systems.
\newblock {\em arXiv preprint arXiv:1512.01274}, 2015.

\bibitem{ruder2016overview}
Sebastian Ruder.
\newblock An overview of gradient descent optimization algorithms.
\newblock {\em arXiv preprint arXiv:1609.04747}, 2016.

\bibitem{zeiler2012adadelta}
\color{black}{Zeiler, Matthew D}.
\newblock {ADADELTA}: an adaptive learning rate method.
\newblock {\em arXiv preprint arXiv:1212.5701}, 2012\color{black}.

\bibitem{dozat2016incorporating}
\color{black}{Dozat, Timothy}.
\newblock Incorporating {Nesterov} momentum into {Adam}.
\newblock 2016\color{black}.

\bibitem{andrychowicz2016learning}
Marcin Andrychowicz, Misha Denil, Sergio Gomez, Matthew~W Hoffman, David Pfau,
  Tom Schaul, and Nando de~Freitas.
\newblock Learning to learn by gradient descent by gradient descent.
\newblock In {\em Advances in Neural Information Processing Systems}, pages
  3981--3989, 2016.

\bibitem{szegedy2015going}
Christian Szegedy, Wei Liu, Yangqing Jia, Pierre Sermanet, Scott Reed, Dragomir
  Anguelov, Dumitru Erhan, Vincent Vanhoucke, and Andrew Rabinovich.
\newblock Going deeper with convolutions.
\newblock In {\em Proceedings of the IEEE conference on computer vision and
  pattern recognition}, pages 1--9, 2015.

\bibitem{stable2018zhou}
\color{black} {Zhou, Yingxue and Chen, Sheng and Banerjee, Arindam}.
\newblock Stable gradient descent.
\newblock In {\em Conference on Uncertainty in Artificial Intelligence},
  2018\color{black}.

\bibitem{wen2017terngrad}
Wei Wen, Cong Xu, Feng Yan, Chunpeng Wu, Yandan Wang, Yiran Chen, and Hai Li.
\newblock {TernGrad}: Ternary gradients to reduce communication in distributed
  deep learning.
\newblock In {\em Advances in neural information processing systems}, 2017.

\bibitem{bonomi2014fog}
Flavio Bonomi, Rodolfo Milito, Preethi Natarajan, and Jiang Zhu.
\newblock Fog computing: A platform for internet of things and analytics.
\newblock In {\em Big Data and Internet of Things: A Roadmap for Smart
  Environments}, pages 169--186. Springer, 2014.

\bibitem{mao2017modnn}
Jiachen Mao, Xiang Chen, Kent~W Nixon, Christopher Krieger, and Yiran Chen.
\newblock {MoDNN}: Local distributed mobile computing system for deep neural
  network.
\newblock In {\em IEEE Design, Automation \& Test in Europe Conference \&
  Exhibition (DATE)}, pages 1396--1401, 2017.

\bibitem{mukherjee2018survey}
\color{black}{Mukherjee, Mithun and Shu, Lei and Wang, Di}.
\newblock Survey of fog computing: Fundamental, network applications, and
  research challenges.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 2018\color{black}.

\bibitem{vaquero2014finding}
\color{black}{Vaquero, Luis M and Rodero-Merino, Luis}.
\newblock Finding your way in the fog: Towards a comprehensive definition of
  fog computing.
\newblock {\em ACM SIGCOMM Computer Communication Review}, 44(5):27--32,
  2014\color{black}.

\bibitem{aazam2018offloading}
{\color{blue}Aazam, Mohammad and Zeadally, Sherali and Harras, Khaled A}.
\newblock {\color{blue}Offloading in fog computing for {IoT}: Review, enabling
  technologies, and research opportunities}.
\newblock {\em {\color{blue}Future Generation Computer Systems}},
  {\color{blue}87}:{\color{blue}278--289}, {\color{blue}2018}.

\bibitem{Buyya2018Manifesto}
{\color{blue}Buyya, Rajkumar and Srirama, Satish Narayana and Casale, Giuliano
  and Calheiros, Rodrigo and Simmhan, Yogesh and Varghese, Blesson and Gelenbe,
  Erol and Javadi, Bahman and Vaquero, Luis Miguel and Netto, Marco A. S. and
  Toosi, Adel Nadjaran and Rodriguez, Maria Alejandra and Llorente, Ignacio M.
  and Vimercati, Sabrina De Capitani Di and Samarati, Pierangela and Milojicic,
  Dejan and Varela, Carlos and Bahsoon, Rami and Assuncao, Marcos Dias De and
  Rana, Omer and Zhou, Wanlei and Jin, Hai and Gentzsch, Wolfgang and Zomaya,
  Albert Y. and Shen, Haiying}.
\newblock {\color{blue}A Manifesto for Future Generation Cloud Computing:
  Research Directions for the Next Decade}.
\newblock {\em {\color{blue}ACM Computing Survey}},
  {\color{blue}51}({\color{blue}5}):{\color{blue}105:1--105:38}.

\bibitem{sze2017efficient}
{\color{blue}Sze, Vivienne and Chen, Yu-Hsin and Yang, Tien-Ju and Emer, Joel
  S}.
\newblock {\color{blue}Efficient processing of deep neural networks: A tutorial
  and survey}.
\newblock {\em {\color{blue}Proceedings of the IEEE}},
  {\color{blue}105}({\color{blue}12}):{\color{blue}2295--2329},
  {\color{blue}2017}.

\bibitem{bang201714}
Suyoung Bang, Jingcheng Wang, Ziyun Li, Cao Gao, Yejoong Kim, Qing Dong, Yen-Po
  Chen, Laura Fick, Xun Sun, Ron Dreslinski, et~al.
\newblock 14.7 a 288$\mu$w programmable deep-learning processor with 270kb
  on-chip weight storage using non-uniform memory hierarchy for mobile
  intelligence.
\newblock In {\em IEEE International Conference on Solid-State Circuits
  (ISSCC)}, pages 250--251, 2017.

\bibitem{akopyan2016design}
Filipp Akopyan.
\newblock Design and tool flow of {IBM}'s truenorth: an ultra-low power
  programmable neurosynaptic chip with 1 million neurons.
\newblock In {\em Proceedings of the International Symposium on Physical
  Design}, pages 59--60. ACM, 2016.

\bibitem{latifi2016cnndroid}
Seyyed~Salar Latifi~Oskouei, Hossein Golestani, Matin Hashemi, and Soheil
  Ghiasi.
\newblock Cnndroid: {GPU}-accelerated execution of trained deep convolutional
  neural networks on {A}ndroid.
\newblock In {\em Proceedings of the ACM on Multimedia Conference}, pages
  1201--1205, 2016.

\bibitem{cortes2017adanet}
Corinna Cortes, Xavi Gonzalvo, Vitaly Kuznetsov, Mehryar Mohri, and Scott Yang.
\newblock Adanet: Adaptive structural learning of artificial neural networks.
\newblock {\em International Conference on Machine Learning (ICML)}, 2017.

\bibitem{hinton2006fast}
Geoffrey~E Hinton, Simon Osindero, and Yee-Whye Teh.
\newblock A fast learning algorithm for deep belief nets.
\newblock {\em Neural computation}, 18(7):1527--1554, 2006.

\bibitem{lee2009convolutional}
Honglak Lee, Roger Grosse, Rajesh Ranganath, and Andrew~Y Ng.
\newblock Convolutional deep belief networks for scalable unsupervised learning
  of hierarchical representations.
\newblock In {\em Proceedings of the 26th ACM annual international conference
  on machine learning}, pages 609--616, 2009.

\bibitem{vincent2010stacked}
Pascal Vincent, Hugo Larochelle, Isabelle Lajoie, Yoshua Bengio, and
  Pierre-Antoine Manzagol.
\newblock Stacked denoising autoencoders: Learning useful representations in a
  deep network with a local denoising criterion.
\newblock {\em Journal of Machine Learning Research}, 11(Dec):3371--3408, 2010.

\bibitem{kingma2014auto}
Diederik~P Kingma and Max Welling.
\newblock {Auto-encoding variational bayes}.
\newblock {\em International Conference on Learning Representations (ICLR)},
  2014.

\bibitem{he2016deep}
Kaiming He, Xiangyu Zhang, Shaoqing Ren, and Jian Sun.
\newblock Deep residual learning for image recognition.
\newblock In {\em Proceedings of the IEEE conference on computer vision and
  pattern recognition}, pages 770--778, 2016.

\bibitem{ji20133d}
Shuiwang Ji, Wei Xu, Ming Yang, and Kai Yu.
\newblock {3D} convolutional neural networks for human action recognition.
\newblock {\em IEEE transactions on pattern analysis and machine intelligence},
  35(1):221--231, 2013.

\bibitem{huang2017densely}
Gao Huang, Zhuang Liu, Kilian~Q Weinberger, and Laurens van~der Maaten.
\newblock Densely connected convolutional networks.
\newblock {\em IEEE Conference on Computer Vision and Pattern Recognition},
  2017.

\bibitem{gers1999learning}
Felix~A Gers, J{\"u}rgen Schmidhuber, and Fred Cummins.
\newblock Learning to forget: Continual prediction with {LSTM}.
\newblock 1999.

\bibitem{sutskever2014sequence}
Ilya Sutskever, Oriol Vinyals, and Quoc~V Le.
\newblock Sequence to sequence learning with neural networks.
\newblock In {\em Advances in neural information processing systems}, pages
  3104--3112, 2014.

\bibitem{xingjian2015convolutional}
Shi Xingjian, Zhourong Chen, Hao Wang, Dit-Yan Yeung, Wai-Kin Wong, and
  Wang-chun Woo.
\newblock Convolutional {LSTM} network: A machine learning approach for
  precipitation nowcasting.
\newblock In {\em Advances in neural information processing systems}, pages
  802--810, 2015.

\bibitem{qi2017loss}
Guo-Jun Qi.
\newblock Loss-sensitive generative adversarial networks on {Lipschitz}
  densities.
\newblock {\em arXiv preprint arXiv:1701.06264}, 2017.

\bibitem{brock2018large}
{\color{blue}Brock, Andrew and Donahue, Jeff and Simonyan, Karen}.
\newblock {\color{blue}Large scale {GAN} training for high fidelity natural
  image synthesis}.
\newblock {\em {\color{blue}arXiv preprint arXiv:1809.11096}},
  {\color{blue}2018}.

\bibitem{silver2016mastering}
David Silver, Aja Huang, Chris~J Maddison, Arthur Guez, Laurent Sifre, George
  Van Den~Driessche, Julian Schrittwieser, Ioannis Antonoglou, Veda
  Panneershelvam, Marc Lanctot, et~al.
\newblock Mastering the game of {Go} with deep neural networks and tree search.
\newblock {\em Nature}, 529(7587):484--489, 2016.

\bibitem{hessel2017rainbow}
\color{black}{Hessel, Matteo and Modayil, Joseph and Van Hasselt, Hado and
  Schaul, Tom and Ostrovski, Georg and Dabney, Will and Horgan, Dan and Piot,
  Bilal and Azar, Mohammad and Silver, David}.
\newblock Rainbow: Combining improvements in deep reinforcement learning.
\newblock 2017\color{black}.

\bibitem{schulman2017proximal}
\color{black}{Schulman, John and Wolski, Filip and Dhariwal, Prafulla and
  Radford, Alec and Klimov, Oleg}.
\newblock Proximal policy optimization algorithms.
\newblock {\em arXiv preprint arXiv:1707.06347}, 2017\color{black}.

\bibitem{collobert2004links}
Ronan Collobert and Samy Bengio.
\newblock Links between perceptrons, {MLP}s and {SVM}s.
\newblock In {\em Proceedings of the twenty-first ACM international conference
  on Machine learning}, page~23, 2004.

\bibitem{glorot2011deep}
booktitle={Proceedings of the fourteenth international conference on artificial
  intelligence and statistics} \color{black}{Glorot, Xavier and Bordes, Antoine
  and Bengio, Yoshua}.
\newblock Deep sparse rectifier neural networks.
\newblock pages 315--323, 2011\color{black}.

\bibitem{klambauer2017self}
\color{black}{Klambauer, G{\"u}nter and Unterthiner, Thomas and Mayr, Andreas
  and Hochreiter, Sepp}.
\newblock Self-normalizing neural networks.
\newblock In {\em Advances in Neural Information Processing Systems}, pages
  971--980, 2017\color{black}.

\bibitem{ioffe2015batch}
{\color{blue}Ioffe, Sergey and Szegedy, Christian}.
\newblock {\color{blue}Batch Normalization: Accelerating Deep Network Training
  by Reducing Internal Covariate Shift}.
\newblock In {\em {\color{blue}Proceedings of the International Conference on
  Machine Learning}}, pages~{\color{blue}448--456}, {\color{blue}2015}.

\bibitem{hinton2002training}
Geoffrey~E Hinton.
\newblock Training products of experts by minimizing contrastive divergence.
\newblock {\em Neural computation}, 14(8):1771--1800, 2002.

\bibitem{casella1992explaining}
George Casella and Edward~I George.
\newblock Explaining the {Gibbs} sampler.
\newblock {\em The American Statistician}, 46(3):167--174, 1992.

\bibitem{kuremoto2014forecast}
Takashi Kuremoto, Masanao Obayashi, Kunikazu Kobayashi, Takaomi Hirata, and
  Shingo Mabu.
\newblock Forecast chaotic time series data by {DBNs}.
\newblock In {\em 7th IEEE International Congress on Image and Signal
  Processing (CISP)}, pages 1130--1135, 2014.

\bibitem{dauphin2013stochastic}
Yann Dauphin and Yoshua Bengio.
\newblock Stochastic ratio matching of {RBMs} for sparse high-dimensional
  inputs.
\newblock In {\em Advances in Neural Information Processing Systems}, pages
  1340--1348, 2013.

\bibitem{sainath2011making}
Tara~N Sainath, Brian Kingsbury, Bhuvana Ramabhadran, Petr Fousek, Petr Novak,
  and Abdel-rahman Mohamed.
\newblock Making deep belief networks effective for large vocabulary continuous
  speech recognition.
\newblock In {\em IEEE Workshop on Automatic Speech Recognition and
  Understanding (ASRU)}, pages 30--35, 2011.

\bibitem{bengio2009learning}
Yoshua Bengio et~al.
\newblock Learning deep architectures for {AI}.
\newblock {\em Foundations and trends{\textregistered} in Machine Learning},
  2(1):1--127, 2009.

\bibitem{sakurada2014anomaly}
Mayu Sakurada and Takehisa Yairi.
\newblock Anomaly detection using autoencoders with nonlinear dimensionality
  reduction.
\newblock In {\em Proceedings Workshop on Machine Learning for Sensory Data
  Analysis (MLSDA)}, page~4. ACM, 2014.

\bibitem{nicolau2016hybrid}
Miguel Nicolau, James McDermott, et~al.
\newblock A hybrid autoencoder and density estimation model for anomaly
  detection.
\newblock In {\em International Conference on Parallel Problem Solving from
  Nature}, pages 717--726. Springer, 2016.

\bibitem{thing2017ieee}
Vrizlynn~LL Thing.
\newblock {IEEE} 802.11 network anomaly detection and attack classification: A
  deep learning approach.
\newblock In {\em IEEE Wireless Communications and Networking Conference
  (WCNC)}, pages 1--6, 2017.

\bibitem{mao2017routing}
Bomin Mao, Zubair~Md Fadlullah, Fengxiao Tang, Nei Kato, Osamu Akashi, Takeru
  Inoue, and Kimihiro Mizutani.
\newblock Routing or computing? the paradigm shift towards intelligent computer
  network packet transmission based on deep learning.
\newblock {\em IEEE Transactions on Computers}, 66(11):1946--1960, 2017.

\bibitem{radu2016towards}
Valentin Radu, Nicholas~D Lane, Sourav Bhattacharya, Cecilia Mascolo, Mahesh~K
  Marina, and Fahim Kawsar.
\newblock Towards multimodal deep learning for activity recognition on mobile
  devices.
\newblock In {\em Proceedings of ACM International Joint Conference on
  Pervasive and Ubiquitous Computing: Adjunct}, pages 185--188, 2016.

\bibitem{radu2018multimodal}
Valentin Radu, Catherine Tong, Sourav Bhattacharya, Nicholas~D Lane, Cecilia
  Mascolo, Mahesh~K Marina, and Fahim Kawsar.
\newblock Multimodal deep learning for activity and context recognition.
\newblock {\em Proceedings of the ACM on Interactive, Mobile, Wearable and
  Ubiquitous Technologies}, 1(4):157, 2018.

\bibitem{raghavendra2016learning}
Ramachandra Raghavendra and Christoph Busch.
\newblock Learning deeply coupled autoencoders for smartphone based robust
  periocular verification.
\newblock In {\em IEEE International Conference on Image Processing (ICIP)},
  pages 325--329, 2016.

\bibitem{li2016wavelet}
Jing Li, Jingyuan Wang, and Zhang Xiong.
\newblock Wavelet-based stacked denoising autoencoders for cell phone base
  station user number prediction.
\newblock In {\em IEEE International Conference on Internet of Things (iThings)
  and IEEE Green Computing and Communications (GreenCom) and IEEE Cyber,
  Physical and Social Computing (CPSCom) and IEEE Smart Data (SmartData)},
  pages 833--838, 2016.

\bibitem{ILSVRC15}
Olga Russakovsky, Jia Deng, Hao Su, Jonathan Krause, Sanjeev Satheesh, Sean Ma,
  Zhiheng Huang, Andrej Karpathy, Aditya Khosla, Michael Bernstein,
  Alexander~C. Berg, and Li~Fei-Fei.
\newblock {ImageNet Large Scale Visual Recognition Challenge}.
\newblock {\em International Journal of Computer Vision (IJCV)},
  115(3):211--252, 2015.

\bibitem{active2017yunho}
Junmo~Kim Yunho~Jeon.
\newblock Active convolution: Learning the shape of convolution for image
  classification.
\newblock In {\em Proceedings of the IEEE Conference on Computer Vision and
  Pattern Recognition}, 2017.

\bibitem{dai2017deformable}
Jifeng Dai, Haozhi Qi, Yuwen Xiong, Yi~Li, Guodong Zhang, Han Hu, and Yichen
  Wei.
\newblock Deformable convolutional networks.
\newblock In {\em Proceedings of the IEEE International Conference on Computer
  Vision}, pages 764--773, 2017.

\bibitem{Zhu2018morel}
{\color{blue}Zhu, Xizhou and Hu, Han and Lin, Stephen and Dai, Jifeng}.
\newblock {\color{blue}Deformable ConvNets v2: More Deformable, Better
  Results}.
\newblock {\em {\color{blue}arXiv preprint arXiv:1811.11168}},
  {\color{blue}2018}.

\bibitem{bengio1994learning}
Yoshua Bengio, Patrice Simard, and Paolo Frasconi.
\newblock Learning long-term dependencies with gradient descent is difficult.
\newblock {\em IEEE transactions on neural networks}, 5(2):157--166, 1994.

\bibitem{graves2013hybrid}
Alex Graves, Navdeep Jaitly, and Abdel-rahman Mohamed.
\newblock Hybrid speech recognition with deep bidirectional {LSTM}.
\newblock In {\em IEEE Workshop on Automatic Speech Recognition and
  Understanding (ASRU)}, pages 273--278, 2013.

\bibitem{johnson2016supervised}
Rie Johnson and Tong Zhang.
\newblock Supervised and semi-supervised text categorization using {LSTM} for
  region embeddings.
\newblock In {\em International Conference on Machine Learning (ICML)}, pages
  526--534, 2016.

\bibitem{goodfellow2016nips}
{\color{blue}Goodfellow, Ian}.
\newblock {\color{blue}{NIPS} 2016 tutorial: Generative adversarial networks}.
\newblock {\em {\color{blue}arXiv preprint arXiv:1701.00160}},
  {\color{blue}2016}.

\bibitem{ledig2017photo}
Christian Ledig, Lucas Theis, Ferenc Husz{\'a}r, Jose Caballero, Andrew
  Cunningham, Alejandro Acosta, Andrew Aitken, Alykhan Tejani, Johannes Totz,
  Zehan Wang, et~al.
\newblock Photo-realistic single image super-resolution using a generative
  adversarial network.
\newblock In {\em IEEE Conference on Computer Vision and Pattern Recognition},
  2017.

\bibitem{li2017perceptual}
Jianan Li, Xiaodan Liang, Yunchao Wei, Tingfa Xu, Jiashi Feng, and Shuicheng
  Yan.
\newblock Perceptual generative adversarial networks for small object
  detection.
\newblock In {\em IEEE Conference on Computer Vision and Pattern Recognition},
  2017.

\bibitem{li2017generative}
Yijun Li, Sifei Liu, Jimei Yang, and Ming-Hsuan Yang.
\newblock Generative face completion.
\newblock In {\em IEEE Conference on Computer Vision and Pattern Recognition},
  2017.

\bibitem{gawlowicz2018ns3}
{\color{blue}Gaw{\l}owicz, Piotr and Zubow, Anatolij}.
\newblock {\color{blue}{NS3-Gym}: Extending {OpenAI Gym} for Networking
  Research}.
\newblock {\em {\color{blue}arXiv preprint arXiv:1810.03943}},
  {\color{blue}2018}.

\bibitem{gu2016continuous}
Shixiang Gu, Timothy Lillicrap, Ilya Sutskever, and Sergey Levine.
\newblock Continuous deep {Q}-learning with model-based acceleration.
\newblock In {\em International Conference on Machine Learning}, pages
  2829--2838, 2016.

\bibitem{moravvcik2017deepstack}
Matej Morav{\v{c}}{\'\i}k, Martin Schmid, Neil Burch, Viliam Lis{\`y}, Dustin
  Morrill, Nolan Bard, Trevor Davis, Kevin Waugh, Michael Johanson, and Michael
  Bowling.
\newblock Deepstack: Expert-level artificial intelligence in heads-up no-limit
  poker.
\newblock {\em Science}, 356(6337):508--513, 2017.

\bibitem{levine2016learning}
Sergey Levine, Peter Pastor, Alex Krizhevsky, Julian Ibarz, and Deirdre
  Quillen.
\newblock Learning hand-eye coordination for robotic grasping with deep
  learning and large-scale data collection.
\newblock {\em The International Journal of Robotics Research},
  37(4-5):421--436, 2018.

\bibitem{sallab2017deep}
Ahmad~EL Sallab, Mohammed Abdou, Etienne Perot, and Senthil Yogamani.
\newblock Deep reinforcement learning framework for autonomous driving.
\newblock {\em Electronic Imaging}, (19):70--76, 2017.

\bibitem{li2014tact}
Rongpeng Li, Zhifeng Zhao, Xianfu Chen, Jacques Palicot, and Honggang Zhang.
\newblock Tact: A transfer actor-critic learning framework for energy saving in
  cellular radio access networks.
\newblock {\em IEEE Transactions on Wireless Communications}, 13(4):2000--2011,
  2014.

\bibitem{al2015application}
Hasan~AA Al-Rawi, Ming~Ann Ng, and Kok-Lim~Alvin Yau.
\newblock Application of reinforcement learning to routing in distributed
  wireless networks: a review.
\newblock {\em Artificial Intelligence Review}, 43(3):381--416, 2015.

\bibitem{liu2015reinforcement}
Yan-Jun Liu, Li~Tang, Shaocheng Tong, CL~Philip Chen, and Dong-Juan Li.
\newblock Reinforcement learning design-based adaptive tracking control with
  less learning parameters for nonlinear discrete-time {MIMO} systems.
\newblock {\em IEEE Transactions on Neural Networks and Learning Systems},
  26(1):165--176, 2015.

\bibitem{pierucci2016neural}
Laura Pierucci and Davide Micheli.
\newblock A neural network for quality of experience estimation in mobile
  communications.
\newblock {\em IEEE MultiMedia}, 23(4):42--49, 2016.

\bibitem{gwon2014inferring}
Youngjune~L Gwon and HT~Kung.
\newblock Inferring origin flow patterns in wi-fi with deep learning.
\newblock In {\em 11th IEEE International Conference on Autonomic Computing
  (ICAC))}, pages 73--83, 2014.

\bibitem{nie2017network}
Laisen Nie, Dingde Jiang, Shui Yu, and Houbing Song.
\newblock Network traffic prediction based on deep belief network in wireless
  mesh backbone networks.
\newblock In {\em Wireless Communications and Networking Conference (WCNC),
  IEEE}, pages 1--5, 2017.

\bibitem{moyo2015generalization}
Vusumuzi Moyo et~al.
\newblock The generalization ability of artificial neural networks in
  forecasting {TCP/IP} traffic trends: How much does the size of learning rate
  matter?
\newblock {\em International Journal of Computer Science and Application},
  2015.

\bibitem{wangspatiotemporal}
Jing Wang, Jian Tang, Zhiyuan Xu, Yanzhi Wang, Guoliang Xue, Xing Zhang, and
  Dejun Yang.
\newblock Spatiotemporal modeling and prediction in cellular networks: A big
  data enabled deep learning approach.
\newblock In {\em 36th Annual IEEE International Conference on Computer
  Communications (INFOCOM)}, 2017.

\bibitem{zhang2017long}
Chaoyun Zhang and Paul Patras.
\newblock Long-term mobile traffic forecasting using deep spatio-temporal
  neural networks.
\newblock In {\em Proceedings of the Eighteenth ACM International Symposium on
  Mobile Ad Hoc Networking and Computing}, pages 231--240, 2018.

\bibitem{chaoyun2017zipnet}
Chaoyun Zhang, Xi~Ouyang, and Paul Patras.
\newblock {ZipNet-GAN}: Inferring fine-grained mobile traffic patterns via a
  generative adversarial neural network.
\newblock In {\em Proceedings of the 13th ACM Conference on Emerging Networking
  Experiments and Technologies}, 2017.

\bibitem{huang2017study}
\color{black}{Huang, Chih-Wei and Chiang, Chiu-Ti and Li, Qiuhui}.
\newblock A study of deep learning networks on mobile traffic forecasting.
\newblock In {\em 28th IEEE Annual International Symposium on Personal, Indoor,
  and Mobile Radio Communications (PIMRC)}, pages 1--6, 2017\color{black}.

\bibitem{zhang2018citywide}
\color{black}{Zhang, Chuanting and Zhang, Haixia and Yuan, Dongfeng and Zhang,
  Minggao}.
\newblock Citywide cellular traffic prediction based on densely connected
  convolutional neural networks.
\newblock {\em IEEE Communications Letters}, 2018\color{black}.

\bibitem{navabi2018predicting}
\color{black}{Navabi, Shiva and Wang, Chenwei and Bursalioglu, Ozgun Y and
  Papadopoulos, Haralabos}.
\newblock Predicting wireless channel features using neural networks.
\newblock {\em arXiv preprint arXiv:1802.00107}, 2018\color{black}.

\bibitem{wang2015applications}
Zhanyi Wang.
\newblock The applications of deep learning on traffic identification.
\newblock {\em BlackHat USA}, 2015.

\bibitem{wang2017end}
Wei Wang, Ming Zhu, Jinlin Wang, Xuewen Zeng, and Zhongzhen Yang.
\newblock End-to-end encrypted traffic classification with one-dimensional
  convolution neural networks.
\newblock In {\em IEEE International Conference on Intelligence and Security
  Informatics (ISI)}, pages 43--48, 2017.

\bibitem{lotfollahi2017deep}
Mohammad Lotfollahi, Ramin Shirali, Mahdi~Jafari Siavoshani, and Mohammdsadegh
  Saberian.
\newblock Deep packet: A novel approach for encrypted traffic classification
  using deep learning.
\newblock {\em arXiv preprint arXiv:1709.02656}, 2017.

\bibitem{wang2017malware}
Wei Wang, Ming Zhu, Xuewen Zeng, Xiaozhou Ye, and Yiqiang Sheng.
\newblock Malware traffic classification using convolutional neural network for
  representation learning.
\newblock In {\em IEEE International Conference on Information Networking
  (ICOIN)}, pages 712--717, 2017.

\bibitem{liang2016mercury}
Victor~C Liang, Richard~TB Ma, Wee~Siong Ng, Li~Wang, Marianne Winslett, Huayu
  Wu, Shanshan Ying, and Zhenjie Zhang.
\newblock Mercury: Metro density prediction with recurrent neural network on
  streaming {CDR} data.
\newblock In {\em IEEE 32nd International Conference on Data Engineering
  (ICDE)}, pages 1374--1377, 2016.

\bibitem{felbo2016using}
Bjarke Felbo, P{\aa}l Sunds{\o}y, Alex'Sandy' Pentland, Sune Lehmann, and
  Yves-Alexandre de~Montjoye.
\newblock Using deep learning to predict demographics from mobile phone
  metadata.
\newblock {\em workshop track of the International Conference on Learning
  Representations (ICLR)}, 2016.

\bibitem{chen2017comprehensive}
Nai~Chun Chen, Wanqin Xie, Roy~E Welsch, Kent Larson, and Jenny Xie.
\newblock Comprehensive predictions of tourists' next visit location based on
  call detail records using machine learning and deep learning methods.
\newblock In {\em IEEE International Congress on Big Data (BigData Congress)},
  pages 1--6, 2017.

\bibitem{lin2017deep}
Ziheng Lin, Mogeng Yin, Sidney Feygin, Madeleine Sheehan, Jean-Francois
  Paiement, and Alexei Pozdnoukhov.
\newblock Deep generative models of urban mobility.
\newblock {\em IEEE Transactions on Intelligent Transportation Systems}, 2017.

\bibitem{xu2017large}
Chang Xu, Kuiyu Chang, Khee-Chin Chua, Meishan Hu, and Zhenxiang Gao.
\newblock Large-scale {Wi-Fi} hotspot classification via deep learning.
\newblock In {\em Proceedings of the 26th International Conference on World
  Wide Web Companion}, pages 857--858. International World Wide Web Conferences
  Steering Committee, 2017.

\bibitem{meng2018qoe}
Qianyu Meng, Kun Wang, Bo~Liu, Toshiaki Miyazaki, and Xiaoming He.
\newblock {QoE}-based big data analysis with deep learning in pervasive edge
  environment.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018.

\bibitem{fang2018mobile}
{\color{blue}Fang, Luoyang and Cheng, Xiang and Wang, Haonan and Yang,
  Liuqing}.
\newblock {\color{blue}Mobile Demand Forecasting via Deep Graph-Sequence
  Spatiotemporal Modeling in Cellular Networks}.
\newblock {\em {\color{blue}IEEE Internet of Things Journal}},
  {\color{blue}2018}.

\bibitem{luo2018channel}
{\color{blue}Luo, Changqing and Ji, Jinlong and Wang, Qianlong and Chen, Xuhui
  and Li, Pan}.
\newblock {\color{blue}Channel state information prediction for {5G} wireless
  communications: A deep learning approach}.
\newblock {\em {\color{blue}IEEE Transactions on Network Science and
  Engineering}}, {\color{blue}2018}.

\bibitem{8553650}
{\color{blue}Li, Peng and Chen, Zhikui and Yang, Laurence T. and Gao, Jing and
  Zhang, Qingchen and Deen, M. Jamal }.
\newblock {\color{blue}An Improved Stacked Auto-Encoder for Network Traffic
  Flow Classification}.
\newblock {\em {\color{blue}IEEE Network}},
  {\color{blue}32}({\color{blue}6}):{\color{blue}22--27}, {\color{blue}2018}.

\bibitem{feng2018deeptp}
{\color{blue}Feng, Jie and Chen, Xinlei and Gao, Rundong and Zeng, Ming and Li,
  Yong}.
\newblock {\color{blue}{DeepTP}: An End-to-End Neural Network for Mobile
  Cellular Traffic Prediction}.
\newblock {\em {\color{blue}IEEE Network}},
  {\color{blue}32}({\color{blue}6}):{\color{blue}108--115}, {\color{blue}2018}.

\bibitem{zhu2018deep}
{\color{blue}Zhu, Hao and Cao, Yang and Wang, Wei and Jiang, Tao and Jin, Shi}.
\newblock {\color{blue}Deep Reinforcement Learning for Mobile Edge Caching:
  Review, New Features, and Open Issues}.
\newblock {\em {\color{blue}IEEE Network}},
  {\color{blue}32}({\color{blue}6}):{\color{blue}50--57}, {\color{blue}2018}.

\bibitem{liu2016poster}
Sicong Liu and Junzhao Du.
\newblock Poster: Mobiear-building an environment-independent acoustic sensing
  platform for the deaf using deep learning.
\newblock In {\em Proceedings of the 14th ACM Annual International Conference
  on Mobile Systems, Applications, and Services Companion}, pages 50--50, 2016.

\bibitem{sicong2017ubiear}
Liu Sicong, Zhou Zimu, Du~Junzhao, Shangguan Longfei, Jun Han, and Xin Wang.
\newblock Ubiear: Bringing location-independent sound awareness to the
  hard-of-hearing people with smartphones.
\newblock {\em Proceedings of the ACM on Interactive, Mobile, Wearable and
  Ubiquitous Technologies}, 1(2):17, 2017.

\bibitem{jindal2016integrating}
Vasu Jindal.
\newblock Integrating mobile and cloud for {PPG} signal selection to monitor
  heart rate during intensive physical exercise.
\newblock In {\em Proceedings of the ACM International Workshop on Mobile
  Software Engineering and Systems}, pages 36--37, 2016.

\bibitem{kim2016deep}
Edward Kim, Miguel Corte-Real, and Zubair Baloch.
\newblock A deep semantic mobile application for thyroid cytopathology.
\newblock In {\em Medical Imaging 2016: PACS and Imaging Informatics: Next
  Generation and Innovations}, volume 9789, page 97890A. International Society
  for Optics and Photonics, 2016.

\bibitem{sathyanarayana2016sleep}
Aarti Sathyanarayana, Shafiq Joty, Luis Fernandez-Luque, Ferda Ofli, Jaideep
  Srivastava, Ahmed Elmagarmid, Teresa Arora, and Shahrad Taheri.
\newblock Sleep quality prediction from wearable data using deep learning.
\newblock {\em JMIR mHealth and uHealth}, 4(4), 2016.

\bibitem{li2017personal}
Honggui Li and Maria Trocan.
\newblock Personal health indicators by deep learning of smart phone sensor
  data.
\newblock In {\em 3rd IEEE International Conference on Cybernetics (CYBCONF)},
  pages 1--5, 2017.

\bibitem{hosseini2017deep}
Mohammad-Parsa Hosseini, Tuyen~X Tran, Dario Pompili, Kost Elisevich, and Hamid
  Soltanian-Zadeh.
\newblock Deep learning with edge computing for localization of
  epileptogenicity using multimodal rs-{fMRI} and {EEG} big data.
\newblock In {\em IEEE International Conference on Autonomic Computing (ICAC)},
  pages 83--92, 2017.

\bibitem{stamate2017deep}
Cosmin Stamate, George~D Magoulas, Stefan K{\"u}ppers, Effrosyni Nomikou,
  Ioannis Daskalopoulos, Marco~U Luchini, Theano Moussouri, and George Roussos.
\newblock Deep learning parkinson's from smartphone data.
\newblock In {\em IEEE International Conference on Pervasive Computing and
  Communications (PerCom)}, pages 31--40, 2017.

\bibitem{quisel2017collecting}
Tom Quisel, Luca Foschini, Alessio Signorini, and David~C Kale.
\newblock Collecting and analyzing millions of mhealth data streams.
\newblock In {\em Proceedings of the 23rd ACM SIGKDD International Conference
  on Knowledge Discovery and Data Mining}, pages 1971--1980, 2017.

\bibitem{khan2017deep}
Usman~Mahmood Khan, Zain Kabir, Syed~Ali Hassan, and Syed~Hassan Ahmed.
\newblock A deep learning framework using passive {WiFi} sensing for
  respiration monitoring.
\newblock In {\em Global Communications Conference (GLOBECOM)}, pages 1--6.
  IEEE, 2017.

\bibitem{li2016deepcham}
Dawei Li, Theodoros Salonidis, Nirmit~V Desai, and Mooi~Choo Chuah.
\newblock Deepcham: Collaborative edge-mediated adaptive deep learning for
  mobile object recognition.
\newblock In {\em IEEE/ACM Symposium on Edge Computing (SEC)}, pages 64--76,
  2016.

\bibitem{tobias2016convolutional}
Luis Tob{\'\i}as, Aur{\'e}lien Ducournau, Fran{\c{c}}ois Rousseau, Gr{\'e}goire
  Mercier, and Ronan Fablet.
\newblock Convolutional neural networks for object recognition on mobile
  devices: A case study.
\newblock In {\em 23rd IEEE International Conference on Pattern Recognition
  (ICPR)}, pages 3530--3535, 2016.

\bibitem{pouladzadeh2017mobile}
Parisa Pouladzadeh and Shervin Shirmohammadi.
\newblock Mobile multi-food recognition using deep learning.
\newblock {\em ACM Transactions on Multimedia Computing, Communications, and
  Applications (TOMM)}, 13(3s):36, 2017.

\bibitem{tanno2016deepfoodcam}
Ryosuke Tanno, Koichi Okamoto, and Keiji Yanai.
\newblock {DeepFoodCam}: A {DCNN}-based real-time mobile food recognition
  system.
\newblock In {\em Proceedings of the 2nd ACM International Workshop on
  Multimedia Assisted Dietary Management}, pages 89--89, 2016.

\bibitem{kuhad2015using}
Pallavi Kuhad, Abdulsalam Yassine, and Shervin Shimohammadi.
\newblock Using distance estimation and deep learning to simplify calibration
  in food calorie measurement.
\newblock In {\em IEEE International Conference on Computational Intelligence
  and Virtual Environments for Measurement Systems and Applications (CIVEMSA)},
  pages 1--6, 2015.

\bibitem{teng2016facial}
Teng Teng and Xubo Yang.
\newblock Facial expressions recognition based on convolutional neural networks
  for mobile virtual reality.
\newblock In {\em Proceedings of the 15th ACM SIGGRAPH Conference on
  Virtual-Reality Continuum and Its Applications in Industry-Volume 1}, pages
  475--478, 2016.

\bibitem{rao2017mobile}
Jinmeng Rao, Yanjun Qiao, Fu~Ren, Junxing Wang, and Qingyun Du.
\newblock A mobile outdoor augmented reality method combining deep learning
  object detection and spatial relationships for geovisualization.
\newblock {\em Sensors}, 17(9):1951, 2017.

\bibitem{zeng2014convolutional}
Ming Zeng, Le~T Nguyen, Bo~Yu, Ole~J Mengshoel, Jiang Zhu, Pang Wu, and Joy
  Zhang.
\newblock Convolutional neural networks for human activity recognition using
  mobile sensors.
\newblock In {\em 6th IEEE International Conference on Mobile Computing,
  Applications and Services (MobiCASE)}, pages 197--205, 2014.

\bibitem{almaslukh2017effective}
Bandar Almaslukh, Jalal AlMuhtadi, and Abdelmonim Artoli.
\newblock An effective deep autoencoder approach for online smartphone-based
  human activity recognition.
\newblock {\em International Journal of Computer Science and Network Security
  (IJCSNS)}, 17(4):160, 2017.

\bibitem{li2016deep22}
Xinyu Li, Yanyi Zhang, Ivan Marsic, Aleksandra Sarcevic, and Randall~S Burd.
\newblock Deep learning for {RFID}-based activity recognition.
\newblock In {\em Proceedings of the 14th ACM Conference on Embedded Network
  Sensor Systems CD-ROM}, pages 164--175, 2016.

\bibitem{bhattacharya2016smart}
Sourav Bhattacharya and Nicholas~D Lane.
\newblock From smart to deep: Robust activity recognition on smartwatches using
  deep learning.
\newblock In {\em IEEE International Conference on Pervasive Computing and
  Communication Workshops (PerCom Workshops)}, pages 1--6, 2016.

\bibitem{antoniou2016general}
Antreas Antoniou and Plamen Angelov.
\newblock A general purpose intelligent surveillance system for mobile devices
  using deep learning.
\newblock In {\em IEEE International Joint Conference on Neural Networks
  (IJCNN)}, pages 2879--2886, 2016.

\bibitem{wang2016interacting}
Saiwen Wang, Jie Song, Jaime Lien, Ivan Poupyrev, and Otmar Hilliges.
\newblock Interacting with {Soli}: Exploring fine-grained dynamic gesture
  recognition in the radio-frequency spectrum.
\newblock In {\em Proceedings of the 29th ACM Annual Symposium on User
  Interface Software and Technology}, pages 851--860, 2016.

\bibitem{gao2016ihear}
Yang Gao, Ning Zhang, Honghao Wang, Xiang Ding, Xu~Ye, Guanling Chen, and
  Yu~Cao.
\newblock ihear food: Eating detection using commodity bluetooth headsets.
\newblock In {\em IEEE First International Conference on Connected Health:
  Applications, Systems and Engineering Technologies (CHASE)}, pages 163--172,
  2016.

\bibitem{zhu2015using}
Jindan Zhu, Amit Pande, Prasant Mohapatra, and Jay~J Han.
\newblock Using deep learning for energy expenditure estimation with wearable
  sensors.
\newblock In {\em 17th IEEE International Conference on E-health Networking,
  Application \& Services (HealthCom)}, pages 501--506, 2015.

\bibitem{sundsoy2016deep}
P{\aa}l Sunds{\o}y, Johannes Bjelland, B~Reme, A~Iqbal, and Eaman Jahani.
\newblock Deep learning applied to mobile phone data for individual income
  classification.
\newblock {\em ICAITA doi}, 10, 2016.

\bibitem{chen2015deep}
Yuqing Chen and Yang Xue.
\newblock A deep learning approach to human activity recognition based on
  single accelerometer.
\newblock In {\em IEEE International Conference on Systems, Man, and
  Cybernetics (SMC)}, pages 1488--1492, 2015.

\bibitem{ha2016convolutional}
Sojeong Ha and Seungjin Choi.
\newblock Convolutional neural networks for human activity recognition using
  multiple accelerometer and gyroscope sensors.
\newblock In {\em IEEE International Joint Conference on Neural Networks
  (IJCNN)}, pages 381--388, 2016.

\bibitem{edel2016binarized}
Marcus Edel and Enrico K{\"o}ppe.
\newblock Binarized-{BLSTM-RNN} based human activity recognition.
\newblock In {\em IEEE International Conference on Indoor Positioning and
  Indoor Navigation (IPIN)}, pages 1--7, 2016.

\bibitem{xue2018appdna}
{\color{blue}Xue, Shuangshuang and Zhang, Lan and Li, Anran and Li, Xiang-Yang
  and Ruan, Chaoyi and Huang, Wenchao}.
\newblock {\color{blue}{AppDNA}: App behavior profiling via graph-based deep
  learning}.
\newblock In {\em {\color{blue}IEEE Conference on Computer Communications}},
  pages~{\color{blue}1475--1483}, {\color{blue}2018}.

\bibitem{liu2018finding}
{\color{blue}Liu, Huiqi and Li, Xiang-Yang and Zhang, Lan and Xie, Yaochen and
  Wu, Zhenan and Dai, Qian and Chen, Ge and Wan, Chunxiao}.
\newblock {\color{blue}Finding the stars in the fireworks: Deep understanding
  of motion sensor fingerprint}.
\newblock In {\em {\color{blue}IEEE Conference on Computer Communications}},
  pages~{\color{blue}126--134}, {\color{blue}2018}.

\bibitem{okita2017recognition}
Tsuyoshi Okita and Sozo Inoue.
\newblock Recognition of multiple overlapping activities using compositional
  cnn-lstm model.
\newblock In {\em Proceedings of the ACM International Joint Conference on
  Pervasive and Ubiquitous Computing and Proceedings of the ACM International
  Symposium on Wearable Computers}, pages 165--168. ACM, 2017.

\bibitem{mittal2016spotgarbage}
Gaurav Mittal, Kaushal~B Yagnik, Mohit Garg, and Narayanan~C Krishnan.
\newblock Spotgarbage: smartphone app to detect garbage using deep learning.
\newblock In {\em Proceedings of the ACM International Joint Conference on
  Pervasive and Ubiquitous Computing}, pages 940--945, 2016.

\bibitem{seidenari2017deep}
Lorenzo Seidenari, Claudio Baecchi, Tiberio Uricchio, Andrea Ferracani, Marco
  Bertini, and Alberto~Del Bimbo.
\newblock Deep artwork detection and retrieval for automatic context-aware
  audio guides.
\newblock {\em ACM Transactions on Multimedia Computing, Communications, and
  Applications (TOMM)}, 13(3s):35, 2017.

\bibitem{zeng2017mobiledeeppill}
Xiao Zeng, Kai Cao, and Mi~Zhang.
\newblock Mobiledeeppill: A small-footprint mobile deep learning system for
  recognizing unconstrained pill images.
\newblock In {\em Proceedings of the 15th ACM Annual International Conference
  on Mobile Systems, Applications, and Services}, pages 56--67, 2017.

\bibitem{zoudeepsense}
\color{black}{Zou, Han and Zhou, Yuxun and Yang, Jianfei and Jiang, Hao and
  Xie, Lihua and Spanos, Costas J}.
\newblock Deepsense: Device-free human activity recognition via autoencoder
  long-term recurrent convolutional network.
\newblock 2018\color{black}.

\bibitem{zeng2017mobile}
Xiao Zeng.
\newblock Mobile sensing through deep learning.
\newblock In {\em Proceedings of the Workshop on MobiSys Ph. D. Forum}, pages
  5--6. ACM, 2017.

\bibitem{wang2015phasefi}
Xuyu Wang, Lingjun Gao, and Shiwen Mao.
\newblock {PhaseFi}: Phase fingerprinting for indoor localization with a deep
  learning approach.
\newblock In {\em IEEE Global Communications Conference (GLOBECOM)}, pages
  1--6, 2015.

\bibitem{wang2016csi}
Xuyu Wang, Lingjun Gao, and Shiwen Mao.
\newblock {CSI} phase fingerprinting for indoor localization with a deep
  learning approach.
\newblock {\em IEEE Internet of Things Journal}, 3(6):1113--1123, 2016.

\bibitem{feng2018evaluation}
\color{black}{Feng, Chunhai and Arshad, Sheheryar and Yu, Ruiyun and Liu,
  Yonghe}.
\newblock Evaluation and improvement of activity detection systems with
  recurrent neural network.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{cao2017deepmood}
Bokai Cao, Lei Zheng, Chenwei Zhang, Philip~S Yu, Andrea Piscitello, John
  Zulueta, Olu Ajilore, Kelly Ryan, and Alex~D Leow.
\newblock Deepmood: Modeling mobile phone typing dynamics for mood detection.
\newblock In {\em Proceedings of the 23rd ACM SIGKDD International Conference
  on Knowledge Discovery and Data Mining}, pages 747--755, 2017.

\bibitem{ran2018deepdecision}
\color{black}{Ran, Xukan and Chen, Haoliang and Zhu, Xiaodan and Liu, Zhenming
  and Chen, Jiasi}.
\newblock Deepdecision: A mobile deep learning framework for edge video
  analytics.
\newblock In {\em IEEE International Conference on Computer Communications},
  2018\color{black}.

\bibitem{siri}
Siri Team.
\newblock {Deep Learning for Siri's Voice: On-device Deep Mixture Density
  Networks for Hybrid Unit Selection Synthesis}.
\newblock \url{https://machinelearning.apple.com/2017/08/06/siri-voices.html},
  2017.
\newblock [Online; accessed 16-Sep-2017].

\bibitem{mcgraw2016personalized}
Ian McGraw, Rohit Prabhavalkar, Raziel Alvarez, Montse~Gonzalez Arenas,
  Kanishka Rao, David Rybach, Ouais Alsharif, Ha{\c{s}}im Sak, Alexander
  Gruenstein, Fran{\c{c}}oise Beaufays, et~al.
\newblock Personalized speech recognition on mobile devices.
\newblock In {\em IEEE International Conference on Acoustics, Speech and Signal
  Processing (ICASSP)}, pages 5955--5959, 2016.

\bibitem{prabhavalkar2016compression}
Rohit Prabhavalkar, Ouais Alsharif, Antoine Bruguier, and Lan McGraw.
\newblock On the compression of recurrent neural networks with an application
  to {LVCSR} acoustic modeling for embedded speech recognition.
\newblock In {\em IEEE International Conference on Acoustics, Speech and Signal
  Processing (ICASSP)}, pages 5970--5974, 2016.

\bibitem{yoshioka2015ntt}
Takuya Yoshioka, Nobutaka Ito, Marc Delcroix, Atsunori Ogawa, Keisuke
  Kinoshita, Masakiyo Fujimoto, Chengzhu Yu, Wojciech~J Fabian, Miquel Espi,
  Takuya Higuchi, et~al.
\newblock The {NTT CHiME}-3 system: Advances in speech enhancement and
  recognition for mobile multi-microphone devices.
\newblock In {\em IEEE Workshop on Automatic Speech Recognition and
  Understanding (ASRU)}, pages 436--443, 2015.

\bibitem{ruan2016speech}
Sherry Ruan, Jacob~O Wobbrock, Kenny Liou, Andrew Ng, and James Landay.
\newblock Speech is 3x faster than typing for english and mandarin text entry
  on mobile devices.
\newblock {\em arXiv preprint arXiv:1608.07323}, 2016.

\bibitem{ignatov2017dslr}
Andrey Ignatov, Nikolay Kobyshev, Radu Timofte, Kenneth Vanhoey, and Luc
  Van~Gool.
\newblock {DSLR}-quality photos on mobile devices with deep convolutional
  networks.
\newblock In {\em IEEE International Conference on Computer Vision (ICCV)},
  2017.

\bibitem{lu2017demo}
Zongqing Lu, Noor Felemban, Kevin Chan, and Thomas La~Porta.
\newblock Demo abstract: On-demand information retrieval from videos using deep
  learning in wireless networks.
\newblock In {\em IEEE/ACM Second International Conference on
  Internet-of-Things Design and Implementation (IoTDI)}, pages 279--280, 2017.

\bibitem{lee2016reducing}
Jemin Lee, Jinse Kwon, and Hyungshin Kim.
\newblock Reducing distraction of smartwatch users with deep learning.
\newblock In {\em Proceedings of the 18th ACM International Conference on
  Human-Computer Interaction with Mobile Devices and Services Adjunct}, pages
  948--953, 2016.

\bibitem{vu2016transportation}
Toan~H Vu, Le~Dung, and Jia-Ching Wang.
\newblock Transportation mode detection on mobile devices using recurrent nets.
\newblock In {\em Proceedings of the ACM on Multimedia Conference}, pages
  392--396, 2016.

\bibitem{fang2017learning}
Shih-Hau Fang, Yu-Xaing Fei, Zhezhuang Xu, and Yu~Tsao.
\newblock Learning transportation modes from smartphone sensors based on deep
  neural network.
\newblock {\em IEEE Sensors Journal}, 17(18):6111--6118, 2017.

\bibitem{zhao2018rf}
\color{black}{Zhao, Mingmin and Tian, Yonglong and Zhao, Hang and Alsheikh,
  Mohammad Abu and Li, Tianhong and Hristov, Rumen and Kabelac, Zachary and
  Katabi, Dina and Torralba, Antonio}.
\newblock {RF}-based {3D} skeletons.
\newblock In {\em Proceedings of the ACM Conference of the ACM Special Interest
  Group on Data Communication (SIGCOMM)}, pages 267--281, 2018\color{black}.

\bibitem{katevas2017practical}
Kleomenis Katevas, Ilias Leontiadis, Martin Pielot, and Joan Serr{\`a}.
\newblock Practical processing of mobile sensor data for continual deep
  learning predictions.
\newblock In {\em Proceedings of the 1st ACM International Workshop on Deep
  Learning for Mobile Systems and Applications}, 2017.

\bibitem{yao2017deepsense}
Shuochao Yao, Shaohan Hu, Yiran Zhao, Aston Zhang, and Tarek Abdelzaher.
\newblock Deepsense: A unified deep learning framework for time-series mobile
  sensing data processing.
\newblock In {\em Proceedings of the 26th International Conference on World
  Wide Web}, pages 351--360. International World Wide Web Conferences Steering
  Committee, 2017.

\bibitem{ohara2017detecting}
Kazuya Ohara, Takuya Maekawa, and Yasuyuki Matsushita.
\newblock Detecting state changes of indoor everyday objects using {Wi-Fi}
  channel state information.
\newblock {\em Proceedings of the ACM on Interactive, Mobile, Wearable and
  Ubiquitous Technologies}, 1(3):88, 2017.

\bibitem{liu2017deep}
Wu~Liu, Huadong Ma, Heng Qi, Dong Zhao, and Zhineng Chen.
\newblock Deep learning hashing for mobile visual search.
\newblock {\em EURASIP Journal on Image and Video Processing}, (1):17, 2017.

\bibitem{ouyang2016deepspace}
Xi~Ouyang, Chaoyun Zhang, Pan Zhou, and Hao Jiang.
\newblock {DeepSpace}: An online deep learning framework for mobile big data to
  understand human mobility patterns.
\newblock {\em arXiv preprint arXiv:1610.07009}, 2016.

\bibitem{yang2017neural}
Hua Yang, Zhimei Li, and Zhiyong Liu.
\newblock Neural networks for {MANET AODV}: an optimization approach.
\newblock {\em Cluster Computing}, pages 1--9, 2017.

\bibitem{song2016deeptransport}
Xuan Song, Hiroshi Kanasugi, and Ryosuke Shibasaki.
\newblock {DeepTransport}: Prediction and simulation of human mobility and
  transportation mode at a citywide level.
\newblock In {\em International Joint Conference on Artificial Intelligence},
  pages 2618--2624, 2016.

\bibitem{zhang2017deep123}
Junbo Zhang, Yu~Zheng, and Dekang Qi.
\newblock Deep spatio-temporal residual networks for citywide crowd flows
  prediction.
\newblock In {\em Thirty-First Association for the Advancement of Artificial
  Intelligence (AAAI) Conference on Artificial Intelligence}, 2017.

\bibitem{subramanian2014implementation}
J~Venkata Subramanian and M~Abdul~Karim Sadiq.
\newblock Implementation of artificial neural network for mobile movement
  prediction.
\newblock {\em Indian Journal of science and Technology}, 7(6):858--863, 2014.

\bibitem{ezema2017artificial}
Longinus~S Ezema and Cosmas~I Ani.
\newblock Artificial neural network approach to mobile location estimation in
  {GSM} network.
\newblock {\em International Journal of Electronics and Telecommunications},
  63(1):39--44, 2017.

\bibitem{shao2018depedo}
\color{black}{Shao, Wenhua and Luo, Haiyong and Zhao, Fang and Wang, Cong and
  Crivello, Antonino and Tunio, Muhammad Zahid}.
\newblock {DePedo}: Anti periodic negative-step movement pedometer with deep
  convolutional neural networks.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{yayeh2018mobility}
{\color{blue}Yayeh, Yirga and Lin, Hsin-piao and Berie, Getaneh and Adege,
  Abebe Belay and Yen, Lei and Jeng, Shiann-Shiun}.
\newblock {\color{blue}Mobility prediction in mobile {Ad-hoc} network using
  deep learning}.
\newblock In {\em {\color{blue}IEEE International Conference on Applied System
  Invention (ICASI)}}, pages~{\color{blue}1203--1206}, {\color{blue}2018}.

\bibitem{chen2016learning2}
{\color{blue}Chen, Quanjun and Song, Xuan and Yamada, Harutoshi and Shibasaki,
  Ryosuke}.
\newblock {\color{blue}Learning Deep Representation from Big and Heterogeneous
  Data for Traffic Accident Inference}.
\newblock In {\em {\color{blue}National Conference on Artificial Intelligence
  (AAAI)}}, pages~{\color{blue}338--344}, {\color{blue}2016}.

\bibitem{song2017deepmob}
{\color{blue}Song, Xuan and Shibasaki, Ryosuke and Yuan, Nicholos Jing and Xie,
  Xing and Li, Tao and Adachi, Ryutaro}.
\newblock {\color{blue}{DeepMob}: learning deep knowledge of human emergency
  behavior and mobility from big and heterogeneous data}.
\newblock {\em {\color{blue}ACM Transactions on Information Systems (TOIS)}},
  {\color{blue}35}({\color{blue}4}):{\color{blue}41}, {\color{blue}2017}.

\bibitem{yao2017trajectory}
{\color{blue}Yao, Di and Zhang, Chao and Zhu, Zhihua and Huang, Jianhui and Bi,
  Jingping}.
\newblock {\color{blue}Trajectory clustering via deep representation learning}.
\newblock In {\em {\color{blue}IEEE International Joint Conference on Neural
  Networks (IJCNN)}}, pages~{\color{blue}3880--3887}, {\color{blue}2017}.

\bibitem{liu2018urban}
{\color{blue}Liu, Zhidan and Li, Zhenjiang and Wu, Kaishun and Li, Mo}.
\newblock {\color{blue}Urban Traffic Prediction from Mobility Data Using Deep
  Learning}.
\newblock {\em {\color{blue}IEEE Network}},
  {\color{blue}32}({\color{blue}4}):{\color{blue}40--46}, {\color{blue}2018}.

\bibitem{wickramasuriya2017base}
Dilranjan~S Wickramasuriya, Calvin~A Perumalla, Kemal Davaslioglu, and
  Richard~D Gitlin.
\newblock Base station prediction and proactive mobility management in virtual
  cells using recurrent neural networks.
\newblock In {\em IEEE Wireless and Microwave Technology Conference (WAMICON)},
  pages 1--6.

\bibitem{tkavcik2016neural}
{\color{blue}Tka{\v{c}}{\'\i}k, Jan and Kord{\'\i}k, Pavel}.
\newblock {\color{blue}Neural turing machine for sequential learning of human
  mobility patterns}.
\newblock In {\em {\color{blue}IEEE International Joint Conference on Neural
  Networks (IJCNN)}}, pages~{\color{blue}2790--2797}, {\color{blue}2016}.

\bibitem{kim2018method}
{\color{blue}Kim, Dong Yup and Song, Ha Yoon}.
\newblock {\color{blue}Method of predicting human mobility patterns using deep
  learning}.
\newblock {\em {\color{blue}Neurocomputing}},
  {\color{blue}280}:{\color{blue}56--64}, {\color{blue}2018}.

\bibitem{jiang2018deepurbanmomentum}
{\color{blue}Jiang, Renhe and Song, Xuan and Fan, Zipei and Xia, Tianqi and
  Chen, Quanjun and Miyazawa, Satoshi and Shibasaki, Ryosuke}.
\newblock {\color{blue}{DeepUrbanMomentum}: An Online Deep-Learning System for
  Short-Term Urban Mobility Prediction}.
\newblock In {\em {\color{blue}National Conference on Artificial Intelligence
  (AAAI)}}, {\color{blue}2018}.

\bibitem{wang2018deep1231}
{\color{blue}Wang, Chujie and Zhao, Zhifeng and Sun, Qi and Zhang, Honggang}.
\newblock {\color{blue}Deep Learning-based Intelligent Dual Connectivity for
  Mobility Management in Dense Network}.
\newblock {\em {\color{blue}arXiv preprint arXiv:1806.04584}},
  {\color{blue}2018}.

\bibitem{jiang2018deep}
{\color{blue}Jiang, Renhe and Song, Xuan and Fan, Zipei and Xia, Tianqi and
  Chen, Quanjun and Chen, Qi and Shibasaki, Ryosuke}.
\newblock {\color{blue}Deep {ROI}-Based Modeling for Urban Human Mobility
  Prediction}.
\newblock {\em {\color{blue}Proceedings of the ACM on Interactive, Mobile,
  Wearable and Ubiquitous Technologies}},
  {\color{blue}2}({\color{blue}1}):{\color{blue}14}, {\color{blue}2018}.

\bibitem{feng2018deepmove}
{\color{blue}Feng, Jie and Li, Yong and Zhang, Chao and Sun, Funing and Meng,
  Fanchao and Guo, Ang and Jin, Depeng}.
\newblock {\color{blue}{DeepMove}: Predicting Human Mobility with Attentional
  Recurrent Networks}.
\newblock In {\em {\color{blue}Proceedings of the 2018 World Wide Web
  Conference on World Wide Web}}, pages~{\color{blue}1459--1468}.
  {\color{blue}International World Wide Web Conferences Steering Committee},
  {\color{blue}2018}.

\bibitem{wang2015deepfi}
Xuyu Wang, Lingjun Gao, Shiwen Mao, and Santosh Pandey.
\newblock {DeepFi}: Deep learning for indoor fingerprinting using channel state
  information.
\newblock In {\em IEEE Wireless Communications and Networking Conference
  (WCNC)}, pages 1666--1671, 2015.

\bibitem{wang2017cifi}
Xuyu Wang, Xiangyu Wang, and Shiwen Mao.
\newblock {CiFi}: Deep convolutional neural networks for indoor localization
  with 5 {GHz} {Wi-Fi}.
\newblock In {\em 2017 IEEE International Conference on Communications (ICC)},
  pages 1--6.

\bibitem{wang2017biloc}
Xuyu Wang, Lingjun Gao, and Shiwen Mao.
\newblock {BiLoc}: Bi-modal deep learning for indoor localization with
  commodity {5GHz WiFi}.
\newblock {\em IEEE Access}, 5:4209--4220, 2017.

\bibitem{nowicki2017low}
Micha{\l} Nowicki and Jan Wietrzykowski.
\newblock Low-effort place recognition with {WiFi} fingerprints using deep
  learning.
\newblock In {\em International Conference Automation}, pages 575--584.
  Springer, 2017.

\bibitem{zhang2016device}
Xiao Zhang, Jie Wang, Qinghua Gao, Xiaorui Ma, and Hongyu Wang.
\newblock Device-free wireless localization and activity recognition with deep
  learning.
\newblock In {\em IEEE International Conference on Pervasive Computing and
  Communication Workshops (PerCom Workshops)}, pages 1--5, 2016.

\bibitem{wang2017device}
Jie Wang, Xiao Zhang, Qinhua Gao, Hao Yue, and Hongyu Wang.
\newblock Device-free wireless localization and activity recognition: A deep
  learning approach.
\newblock {\em IEEE Transactions on Vehicular Technology}, 66(7):6258--6267,
  2017.

\bibitem{mohammadi2017semi}
Mehdi Mohammadi, Ala Al-Fuqaha, Mohsen Guizani, and Jun-Seok Oh.
\newblock Semi-supervised deep reinforcement learning in support of {IoT} and
  smart city services.
\newblock {\em IEEE Internet of Things Journal}, 2017.

\bibitem{anzum2018zone}
\color{black}{Anzum, Nafisa and Afroze, Syeda Farzia and Rahman, Ashikur}.
\newblock Zone-based indoor localization using neural networks: A view from a
  real testbed.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--7, 2018\color{black}.

\bibitem{wang2018deepml}
\color{black}{Wang, Xuyu and Yu, Zhitao and Mao, Shiwen}.
\newblock {DeepML}: Deep {LSTM} for indoor localization with smartphone
  magnetic and light sensors.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{kumar2016indoor}
Anil Kumar Tirumala~Ravi Kumar, Bernd Sch{\"a}ufele, Daniel Becker, Oliver
  Sawade, and Ilja Radusch.
\newblock Indoor localization of vehicles using deep learning.
\newblock In {\em 17th IEEE International Symposium on World of Wireless,
  Mobile and Multimedia Networks (WoWMoM)}, pages 1--6.

\bibitem{zhengj2016mobile}
Zejia Zhengj and Juyang Weng.
\newblock Mobile device based outdoor navigation with on-line learning neural
  network: A comparison with convolutional neural network.
\newblock In {\em Proceedings of the IEEE Conference on Computer Vision and
  Pattern Recognition Workshops}, pages 11--18, 2016.

\bibitem{vieira2017deep}
Joao Vieira, Erik Leitinger, Muris Sarajlic, Xuhong Li, and Fredrik Tufvesson.
\newblock Deep convolutional neural networks for massive {MIMO}
  fingerprint-based positioning.
\newblock In {\em 28th IEEE Annual International Symposium on Personal, Indoor
  and Mobile Radio Communications}, 2017.

\bibitem{wang2017csi}
{\color{blue}Wang, Xuyu and Gao, Lingjun and Mao, Shiwen and Pandey, Santosh}.
\newblock {\color{blue}{CSI}-based fingerprinting for indoor localization: A
  deep learning approach}.
\newblock {\em {\color{blue}IEEE Transactions on Vehicular Technology}},
  {\color{blue}66}({\color{blue}1}):{\color{blue}763--776}, {\color{blue}2017}.

\bibitem{chen2017confi}
{\color{blue}Chen, Hao and Zhang, Yifan and Li, Wei and Tao, Xiaofeng and
  Zhang, Ping}.
\newblock {\color{blue}{ConFi}: Convolutional neural networks based indoor
  {wi-fi} localization using channel state information}.
\newblock {\em {\color{blue}IEEE Access}},
  {\color{blue}5}:{\color{blue}18066--18074}, {\color{blue}2017}.

\bibitem{shokry2018deeploc}
{\color{blue}Shokry, Ahmed and Torki, Marwan and Youssef, Moustafa}.
\newblock {\color{blue}{DeepLoc}: A ubiquitous accurate and low-overhead
  outdoor cellular localization system}.
\newblock In {\em {\color{blue}Proceedings of the 26th ACM SIGSPATIAL
  International Conference on Advances in Geographic Information Systems}},
  pages~{\color{blue}339--348}, {\color{blue}2018}.

\bibitem{zhou2018device}
{\color{blue}Zhou, Rui and Hao, Meng and Lu, Xiang and Tang, Mingjie and Fu,
  Yang}.
\newblock {\color{blue}Device-Free Localization Based on {CSI} Fingerprints and
  Deep Neural Networks}.
\newblock In {\em {\color{blue}15th Annual IEEE International Conference on
  Sensing, Communication, and Networking (SECON)}}, pages~{\color{blue}1--9},
  {\color{blue}2018}.

\bibitem{zhang2017deeppositioning}
{\color{blue}Zhang, Wei and Sengupta, Rahul and Fodero, John and Li, Xiaolin}.
\newblock {\color{blue}{DeepPositioning}: Intelligent Fusion of Pervasive
  Magnetic Field and {WiFi} Fingerprinting for Smartphone Indoor Localization
  via Deep Learning}.
\newblock In {\em {\color{blue}16th IEEE International Conference on Machine
  Learning and Applications (ICMLA)}}, pages~{\color{blue}7--13},
  {\color{blue}2017}.

\bibitem{adege2018applying}
{\color{blue}Adege, Abebe and Lin, Hsin-Piao and Tarekegn, Getaneh and Jeng,
  Shiann-Shiun}.
\newblock {\color{blue}Applying Deep Neural Network {(DNN)} for Robust Indoor
  Localization in Multi-Building Environment}.
\newblock {\em {\color{blue}Applied Sciences}},
  {\color{blue}8}({\color{blue}7}):{\color{blue}1062}, {\color{blue}2018}.

\bibitem{ibrahim2018cnn}
{\color{blue}Ibrahim, Mai and Torki, Marwan and ElNainay, Mustafa}.
\newblock {\color{blue}{CNN} based Indoor Localization using {RSS}
  Time-Series}.
\newblock In {\em {\color{blue}IEEE Symposium on Computers and Communications
  (ISCC)}}, pages~{\color{blue}1044--1049}, {\color{blue}2018}.

\bibitem{niitsoo2018convolutional}
{\color{blue}Niitsoo, Arne and Edelh{\"a}u$\beta$er, Thorsten and Mutschler,
  Christopher}.
\newblock {\color{blue}Convolutional neural networks for position estimation in
  {TDoA}-based locating systems}.
\newblock In {\em {\color{blue}IEEE International Conference on Indoor
  Positioning and Indoor Navigation (IPIN)}}, pages~{\color{blue}1--8},
  {\color{blue}2018}.

\bibitem{wang2018deep6}
{\color{blue}Wang, Xuyu and Wang, Xiangyu and Mao, Shiwen}.
\newblock {\color{blue}Deep convolutional neural networks for indoor
  localization with {CSI} images}.
\newblock {\em {\color{blue}IEEE Transactions on Network Science and
  Engineering}}, {\color{blue}2018}.

\bibitem{xiao20173}
{\color{blue}Xiao, Chao and Yang, Daiqin and Chen, Zhenzhong and Tan, Guang}.
\newblock {\color{blue}{3-D BLE} indoor localization based on denoising
  autoencoder}.
\newblock {\em {\color{blue}IEEE Access}},
  {\color{blue}5}:{\color{blue}12751--12760}, {\color{blue}2017}.

\bibitem{Hsu:2017:ZIS:3139486.3130924}
{\color{blue}Hsu, Chen-Yu and Ahuja, Aayush and Yue, Shichao and Hristov, Rumen
  and Kabelac, Zachary and Katabi, Dina}.
\newblock {\color{blue}Zero-Effort In-Home Sleep and Insomnia Monitoring Using
  Radio Signals}.
\newblock {\em {\color{blue}Proceedings of ACM Interactive, Mobile, Wearable
  and Ubiquitous Technologies (IMWUT)}}, {\color{blue}1}({\color{blue}3}),
  September {\color{blue}2017}.

\bibitem{guan2017high}
{\color{blue}Guan, Weipeng and Wu, Yuxiang and Xie, Canyu and Chen, Hao and
  Cai, Ye and Chen, Yingcong}.
\newblock {\color{blue}High-precision approach to localization scheme of
  visible light communication based on artificial neural networks and modified
  genetic algorithms}.
\newblock {\em {\color{blue}Optical Engineering}},
  {\color{blue}56}({\color{blue}10}):{\color{blue}106103}, {\color{blue}2017}.

\bibitem{chuang2014effective}
Po-Jen Chuang and Yi-Jun Jiang.
\newblock Effective neural network-based node localisation scheme for wireless
  sensor networks.
\newblock {\em IET Wireless Sensor Systems}, 4(2):97--103, 2014.

\bibitem{bernas2015fully}
Marcin Bernas and Bart{\l}omiej P{\l}aczek.
\newblock Fully connected neural networks ensemble with signal strength
  clustering for indoor localization in wireless sensor networks.
\newblock {\em International Journal of Distributed Sensor Networks},
  11(12):403242, 2015.

\bibitem{payal2015analysis}
Ashish Payal, Chandra~Shekhar Rai, and BV~Ramana Reddy.
\newblock Analysis of some feedforward artificial neural network training
  algorithms for developing localization framework in wireless sensor networks.
\newblock {\em Wireless Personal Communications}, 82(4):2519--2536, 2015.

\bibitem{dong2017range}
Yuhan Dong, Zheng Li, Rui Wang, and Kai Zhang.
\newblock Range-based localization in underwater wireless sensor networks using
  deep neural network.
\newblock In {\em IPSN}, pages 321--322, 2017.

\bibitem{yan2016real}
Xiaofei Yan, Hong Cheng, Yandong Zhao, Wenhua Yu, Huan Huang, and Xiaoliang
  Zheng.
\newblock Real-time identification of smoldering and flaming combustion phases
  in forest using a wireless sensor network-based multi-sensor system and
  artificial neural network.
\newblock {\em Sensors}, 16(8):1228, 2016.

\bibitem{wang2017temperature}
Baowei Wang, Xiaodu Gu, Li~Ma, and Shuangshuang Yan.
\newblock Temperature error correction based on {BP} neural network in
  meteorological wireless sensor network.
\newblock {\em International Journal of Sensor Networks}, 23(4):265--278, 2017.

\bibitem{lee2017deep222}
Ki-Seong Lee, Sun-Ro Lee, Youngmin Kim, and Chan-Gun Lee.
\newblock Deep learning--based real-time query processing for wireless sensor
  network.
\newblock {\em International Journal of Distributed Sensor Networks}, 13(5),
  2017.

\bibitem{li2016adaptive}
Jiakai Li and Gursel Serpen.
\newblock Adaptive and intelligent wireless sensor networks through neural
  networks: an illustration for infrastructure adaptation through hopfield
  network.
\newblock {\em Applied Intelligence}, 45(2):343--362, 2016.

\bibitem{khorasani2017energy}
Fereshteh Khorasani and Hamid~Reza Naji.
\newblock Energy efficient data aggregation in wireless sensor networks using
  neural networks.
\newblock {\em International Journal of Sensor Networks}, 24(1):26--42, 2017.

\bibitem{li2015distributed}
Chunlin Li, Xiaofu Xie, Yuejiang Huang, Hong Wang, and Changxi Niu.
\newblock Distributed data mining based on deep neural network for wireless
  sensor network.
\newblock {\em International Journal of Distributed Sensor Networks},
  11(7):157453, 2015.

\bibitem{luo2018distributed}
\color{black}{Luo, Tie and Nagarajany, Sai G}.
\newblock Distributed anomaly detection using autoencoder neural networks in
  {WSN for IoT}.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{kumar2019machine}
{\color{blue}Kumar, D Praveen and Amgoth, Tarachand and Annavarapu, Chandra
  Sekhara Rao}.
\newblock {\color{blue}Machine learning algorithms for wireless sensor
  networks: A survey}.
\newblock {\em {\color{blue}Information Fusion}},
  {\color{blue}49}:{\color{blue}1--25}, {\color{blue}2019}.

\bibitem{heydari2017reduce}
{\color{blue}Heydari, Nasim and Minaei-Bidgoli, Behrouz}.
\newblock {\color{blue}Reduce energy consumption and send secure data wireless
  multimedia sensor networks using a combination of techniques for multi-layer
  watermark and deep learning}.
\newblock {\em {\color{blue}International Journal of Computer Science and
  Network Security (IJCSNS)}},
  {\color{blue}17}({\color{blue}2}):{\color{blue}98--105}, {\color{blue}2017}.

\bibitem{phoemphon2018hybrid}
{\color{blue}Phoemphon, Songyut and So-In, Chakchai and Niyato, Dusit Tao}.
\newblock {\color{blue}A hybrid model using fuzzy logic and an extreme learning
  machine with vector particle swarm optimization for wireless sensor network
  localization}.
\newblock {\em {\color{blue}Applied Soft Computing}},
  {\color{blue}65}:{\color{blue}101--120}, {\color{blue}2018}.

\bibitem{banihashemian2018new}
{\color{blue}Banihashemian, Seyed Saber and Adibnia, Fazlollah and Sarram,
  Mehdi A}.
\newblock {\color{blue}A new range-free and storage-efficient localization
  algorithm using neural networks in wireless sensor networks}.
\newblock {\em {\color{blue}Wireless Personal Communications}},
  {\color{blue}98}({\color{blue}1}):{\color{blue}1547--1568},
  {\color{blue}2018}.

\bibitem{sun2017wnn}
{\color{blue}Sun, Wei and Lu, Wei and Li, Qiyue and Chen, Liangfeng and Mu,
  Daoming and Yuan, Xiaojing}.
\newblock {\color{blue}{WNN-LQE}: Wavelet-Neural-Network-Based Link Quality
  Estimation for Smart Grid {WSNs}}.
\newblock {\em {\color{blue}IEEE Access}},
  {\color{blue}5}:{\color{blue}12788--12797}, {\color{blue}2017}.

\bibitem{kang2018novel}
{\color{blue}Kang, Jiheon and Park, Youn-Jong and Lee, Jaeho and Wang, Soo-Hyun
  and Eom, Doo-Seop}.
\newblock {\color{blue}Novel Leakage Detection by Ensemble {CNN-SVM} and
  Graph-based Localization in Water Distribution Systems}.
\newblock {\em {\color{blue}IEEE Transactions on Industrial Electronics}},
  {\color{blue}65}({\color{blue}5}):{\color{blue}4279--4289},
  {\color{blue}2018}.

\bibitem{mehmood2017eldc}
{\color{blue}Mehmood, Amjad and Lv, Zhihan and Lloret, Jaime and Umar, Muhammad
  Muneer}.
\newblock {\color{blue}{ELDC}: An artificial neural network based
  energy-efficient and robust routing scheme for pollution monitoring in WSNs}.
\newblock {\em {\color{blue}IEEE Transactions on Emerging Topics in
  Computing}}, {\color{blue}2017}.

\bibitem{alsheikh2016rate}
{\color{blue}Alsheikh, Mohammad Abu and Lin, Shaowei and Niyato, Dusit and Tan,
  Hwee-Pink}.
\newblock {\color{blue}Rate-distortion balanced data compression for wireless
  sensor networks}.
\newblock {\em {\color{blue}IEEE Sensors Journal}},
  {\color{blue}16}({\color{blue}12}):{\color{blue}5072--5083},
  {\color{blue}2016}.

\bibitem{el2016robust}
{\color{blue}El Assaf, Ahmad and Zaidi, Slim and Affes, Sofi{\`e}ne and Kandil,
  Nahi}.
\newblock {\color{blue}Robust {ANNs-Based WSN} Localization in the Presence of
  Anisotropic Signal Attenuation}.
\newblock {\em {\color{blue}IEEE Wireless Communications Letters}},
  {\color{blue}5}({\color{blue}5}):{\color{blue}504--507}, {\color{blue}2016}.

\bibitem{wang2017deep3}
{\color{blue}Wang, Yuzhi and Yang, Anqi and Chen, Xiaoming and Wang, Pengjun
  and Wang, Yu and Yang, Huazhong}.
\newblock {\color{blue}A deep learning approach for blind drift calibration of
  sensor networks}.
\newblock {\em {\color{blue}IEEE Sensors Journal}},
  {\color{blue}17}({\color{blue}13}):{\color{blue}4158--4171},
  {\color{blue}2017}.

\bibitem{jia2018continuous}
{\color{blue}Jia, Zhenhua and Lyu, Xinmeng and Zhang, Wuyang and Martin,
  Richard P and Howard, Richard E and Zhang, Yanyong}.
\newblock {\color{blue}Continuous Low-Power Ammonia Monitoring Using Long
  Short-Term Memory Neural Networks}.
\newblock In {\em {\color{blue}Proceedings of the 16th ACM Conference on
  Embedded Networked Sensor Systems}}, pages~{\color{blue}224--236},
  {\color{blue}2018}.

\bibitem{liu2017deep222}
Lu~Liu, Yu~Cheng, Lin Cai, Sheng Zhou, and Zhisheng Niu.
\newblock Deep learning based optimization in wireless network.
\newblock In {\em 2017 IEEE International Conference on Communications (ICC)},
  pages 1--6.

\bibitem{subramanian2016poster}
Shivashankar Subramanian and Arindam Banerjee.
\newblock Poster: Deep learning enabled {M2M} gateway for network optimization.
\newblock In {\em Proceedings of the 14th ACM Annual International Conference
  on Mobile Systems, Applications, and Services Companion}, pages 144--144,
  2016.

\bibitem{he2017optimization}
Ying He, Chengchao Liang, F~Richard Yu, Nan Zhao, and Hongxi Yin.
\newblock Optimization of cache-enabled opportunistic interference alignment
  wireless networks: A big data deep reinforcement learning approach.
\newblock In {\em 2017 IEEE International Conference on Communications (ICC)},
  pages 1--6.

\bibitem{he2017deep3}
Ying He, Zheng Zhang, F~Richard Yu, Nan Zhao, Hongxi Yin, Victor~CM Leung, and
  Yanhua Zhang.
\newblock Deep reinforcement learning-based optimization for cache-enabled
  opportunistic interference alignment wireless networks.
\newblock {\em IEEE Transactions on Vehicular Technology}, 2017.

\bibitem{mismar2017deep}
Faris~B Mismar and Brian~L Evans.
\newblock Deep reinforcement learning for improving downlink mmwave
  communication performance.
\newblock {\em arXiv preprint arXiv:1707.02329}, 2017.

\bibitem{wang2018handover}
\color{black}{Wang, Zhi and Li, Lihua and Xu, Yue and Tian, Hui and Cui,
  Shuguang}.
\newblock Handover optimization via asynchronous multi-user deep reinforcement
  learning.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{chen2018heterogeneous}
\color{black}{Chen, Ziqi and Smith, David B}.
\newblock Heterogeneous machine-type communications in cellular networks:
  Random access optimization by deep reinforcement learning.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{chen2018auto}
\color{black}{Chen, Li and Lingys, Justinas and Chen, Kai and Liu, Feng}.
\newblock {AuTO}: scaling deep reinforcement learning for datacenter-scale
  automatic traffic optimization.
\newblock In {\em Proceedings of the ACM Conference of the ACM Special Interest
  Group on Data Communication (SIGCOMM)}, pages 191--205, 2018\color{black}.

\bibitem{lee2017classification}
YangMin Lee.
\newblock Classification of node degree based on deep learning and routing
  method applied for virtual route assignment.
\newblock {\em Ad Hoc Networks}, 58:70--85, 2017.

\bibitem{tang2017removing}
Fengxiao Tang, Bomin Mao, Zubair~Md Fadlullah, Nei Kato, Osamu Akashi, Takeru
  Inoue, and Kimihiro Mizutani.
\newblock On removing routing protocol from future wireless networks: A
  real-time deep learning approach for intelligent traffic control.
\newblock {\em IEEE Wireless Communications}, 2017.

\bibitem{zhang2017energy}
Qingchen Zhang, Man Lin, Laurence~T Yang, Zhikui Chen, and Peng Li.
\newblock Energy-efficient scheduling for real-time systems based on deep
  {Q}-learning model.
\newblock {\em IEEE Transactions on Sustainable Computing}, 2017.

\bibitem{atallah2017deep}
Ribal Atallah, Chadi Assi, and Maurice Khabbaz.
\newblock Deep reinforcement learning-based scheduling for roadside
  communication networks.
\newblock In {\em 15th IEEE International Symposium on Modeling and
  Optimization in Mobile, Ad Hoc, and Wireless Networks (WiOpt)}, pages 1--8,
  2017.

\bibitem{chinchali2018}
Sandeep Chinchali, Pan Hu, Tianshu Chu, Manu Sharma, Manu Bansal, Rakesh Misra,
  Marco Pavone, and Katti Sachin.
\newblock Cellular network traffic scheduling with deep reinforcement learning.
\newblock In {\em National Conference on Artificial Intelligence (AAAI)}, 2018.

\bibitem{wei2018joint}
\color{black}{Wei, Yifei and Zhang, Zhiqiang and Yu, F Richard and Han, Zhu}.
\newblock Joint user scheduling and content caching strategy for mobile edge
  networks using deep reinforcement learning.
\newblock In {\em IEEE International Conference on Communications Workshops
  (ICC Workshops)}, 2018\color{black}.

\bibitem{sun2017learning}
Haoran Sun, Xiangyi Chen, Qingjiang Shi, Mingyi Hong, Xiao Fu, and Nikos~D
  Sidiropoulos.
\newblock Learning to optimize: Training deep neural networks for wireless
  resource management.
\newblock In {\em 18th IEEE International Workshop on Signal Processing
  Advances in Wireless Communications (SPAWC)}, pages 1--6, 2017.

\bibitem{xu2017deep3}
Zhiyuan Xu, Yanzhi Wang, Jian Tang, Jing Wang, and Mustafa~Cenk Gursoy.
\newblock A deep reinforcement learning based framework for power-efficient
  resource allocation in cloud {RANs}.
\newblock In {\em 2017 IEEE International Conference on Communications (ICC)},
  pages 1--6.

\bibitem{ferreira2017multi}
Paulo Victor~R Ferreira, Randy Paffenroth, Alexander~M Wyglinski, Timothy~M
  Hackett, Sven~G Bil{\'e}n, Richard~C Reinhart, and Dale~J Mortensen.
\newblock Multi-objective reinforcement learning-based deep neural networks for
  cognitive space communications.
\newblock In {\em Cognitive Communications for Aerospace Applications Workshop
  (CCAA)}, pages 1--8. IEEE, 2017.

\bibitem{ye2018deep12}
\color{black}{Ye, Hao and Li, Geoffrey Ye}.
\newblock Deep reinforcement learning for resource allocation in {V2V}
  communications.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{challita2018proactive}
\color{black}{Challita, Ursula and Dong, Li and Saad, Walid}.
\newblock Proactive resource management for {LTE} in unlicensed spectrum: A
  deep learning perspective.
\newblock {\em IEEE Transactions on Wireless Communications},
  2018\color{black}.

\bibitem{naparstek2017deep}
Oshri Naparstek and Kobi Cohen.
\newblock Deep multi-user reinforcement learning for dynamic spectrum access in
  multichannel wireless networks.
\newblock In {\em IEEE Global Communications Conference}, pages 1--7, 2017.

\bibitem{o2016deep}
Timothy~J O'Shea and T~Charles Clancy.
\newblock Deep reinforcement learning radio control and signal detection with
  {KeRLym}, a gym {RL} agent.
\newblock {\em arXiv preprint arXiv:1605.09221}, 2016.

\bibitem{wijaya2015intercell}
Michael~Andri Wijaya, Kazuhiko Fukawa, and Hiroshi Suzuki.
\newblock Intercell-interference cancellation and neural network transmit power
  optimization for {MIMO} channels.
\newblock In {\em IEEE 82nd Vehicular Technology Conference (VTC Fall)}, pages
  1--5, 2015.

\bibitem{rutagemwa2018dynamic}
\color{black}{Rutagemwa, Humphrey and Ghasemi, Amir and Liu, Shuo}.
\newblock Dynamic spectrum assignment for land mobile radio with deep recurrent
  neural networks.
\newblock In {\em IEEE International Conference on Communications Workshops
  (ICC Workshops)}, 2018\color{black}.

\bibitem{wijaya2016neural}
Michael~Andri Wijaya, Kazuhiko Fukawa, and Hiroshi Suzuki.
\newblock Neural network based transmit power control and interference
  cancellation for {MIMO} small cell networks.
\newblock {\em IEICE Transactions on Communications}, 99(5):1157--1169, 2016.

\bibitem{mao2017neural}
Hongzi Mao, Ravi Netravali, and Mohammad Alizadeh.
\newblock Neural adaptive video streaming with pensieve.
\newblock In {\em Proceedings of the Conference of the ACM Special Interest
  Group on Data Communication (SIGCOMM)}, pages 197--210. ACM, 2017.

\bibitem{oda2017design}
Tetsuya Oda, Ryoichiro Obukata, Makoto Ikeda, Leonard Barolli, and Makoto
  Takizawa.
\newblock Design and implementation of a simulation system based on deep
  {Q}-network for mobile actor node control in wireless sensor and actor
  networks.
\newblock In {\em 31st IEEE International Conference on Advanced Information
  Networking and Applications Workshops (WAINA)}, pages 195--200, 2017.

\bibitem{oda2017performance}
Tetsuya Oda, Donald Elmazi, Miralda Cuka, Elis Kulla, Makoto Ikeda, and Leonard
  Barolli.
\newblock Performance evaluation of a deep {Q}-network based simulation system
  for actor node mobility control in wireless sensor and actor networks
  considering three-dimensional environment.
\newblock In {\em International Conference on Intelligent Networking and
  Collaborative Systems}, pages 41--52. Springer, 2017.

\bibitem{kim2017load}
Hye-Young Kim and Jong-Min Kim.
\newblock A load balancing scheme based on deep-learning in {IoT}.
\newblock {\em Cluster Computing}, 20(1):873--878, 2017.

\bibitem{challita2018deep}
\color{black}{Challita, Ursula and Saad, Walid and Bettstetter, Christian}.
\newblock Deep reinforcement learning for interference-aware path planning of
  cellular connected {UAVs}.
\newblock In {\em IEEE International Conference on Communications (ICC)},
  2018\color{black}.

\bibitem{luo2018online}
\color{black}{Luo, Changqing and Ji, Jinlong and Wang, Qianlong and Yu, Lixing
  and Li, Pan}.
\newblock Online power control for {5G} wireless communications: A deep
  {Q}-network approach.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{yu2018deep2}
\color{black}{Yu, Yiding and Wang, Taotao and Liew, Soung Chang}.
\newblock Deep-reinforcement learning multiple access for heterogeneous
  wireless networks.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--7, 2018\color{black}.

\bibitem{xu2018experience}
\color{black}{Xu, Zhiyuan and Tang, Jian and Meng, Jingsong and Zhang, Weiyi
  and Wang, Yanzhi and Liu, Chi Harold and Yang, Dejun}.
\newblock Experience-driven networking: A deep reinforcement learning based
  approach.
\newblock In {\em IEEE International Conference on Computer Communications},
  2018\color{black}.

\bibitem{liu2018deepnap}
\color{black}{Liu, Jingchu and Krishnamachari, Bhaskar and Zhou, Sheng and Niu,
  Zhisheng}.
\newblock {DeepNap}: Data-driven base station sleeping operations through deep
  reinforcement learning.
\newblock {\em IEEE Internet of Things Journal}, 2018\color{black}.

\bibitem{zhao2018deep}
{\color{blue}Zhao, Zhifeng and Li, Rongpeng and Sun, Qi and Yang, Yangchen and
  Chen, Xianfu and Zhao, Minjian and Zhang, Honggang and others}.
\newblock {\color{blue}Deep Reinforcement Learning for Network Slicing}.
\newblock {\em {\color{blue}arXiv preprint arXiv:1805.06591}},
  {\color{blue}2018}.

\bibitem{li2018deep}
{\color{blue}Li, Ji and Gao, Hui and Lv, Tiejun and Lu, Yueming}.
\newblock {\color{blue}Deep reinforcement learning based computation offloading
  and resource allocation for {MEC}}.
\newblock In {\em {\color{blue}IEEE Wireless Communications and Networking
  Conference (WCNC)}}, pages~{\color{blue}1--6}, {\color{blue}2018}.

\bibitem{mennes2018neural}
Steven {\color{blue}Mennes, Ruben and Camelo, Miguel and Claeys, Maxim and
  Latr{\'e}}.
\newblock {\color{blue}A neural-network-based {MF-TDMA MAC} scheduler for
  collaborative wireless networks}.

\bibitem{8553651}
{\color{blue}Zhou, Yibo and Fadlullah, Zubair Md. and Mao, Bomin and Kato,
  Nei}.
\newblock {\color{blue}A Deep-Learning-Based Radio Resource Assignment
  Technique for {5G} Ultra Dense Networks}.
\newblock {\em {\color{blue}IEEE Network}},
  {\color{blue}32}({\color{blue}6}):{\color{blue}28--34}, {\color{blue}2018}.

\bibitem{mao2017tensor}
{\color{blue}Mao, Bomin and Fadlullah, Zubair Md and Tang, Fengxiao and Kato,
  Nei and Akashi, Osamu and Inoue, Takeru and Mizutani, Kimihiro}.
\newblock {\color{blue}A Tensor Based Deep Learning Technique for Intelligent
  Packet Routing}.
\newblock In {\em {\color{blue}IEEE Global Communications Conference}},
  pages~{\color{blue}1--6}. {\color{blue}IEEE}, {\color{blue}2017}.

\bibitem{geyer2018learning}
{\color{blue}Geyer, Fabien and Carle, Georg}.
\newblock {\color{blue}Learning and Generating Distributed Routing Protocols
  Using Graph-Based Deep Learning}.
\newblock In {\em {\color{blue}Proceedings of the ACM Workshop on Big Data
  Analytics and Machine Learning for Data Communication Networks}},
  pages~{\color{blue}40--45}, {\color{blue}2018}.

\bibitem{luong2018joint}
{\color{blue}Luong, Nguyen Cong and Anh, Tran The and Binh, Huynh Thi Thanh and
  Niyato, Dusit and Kim, Dong In and Liang, Ying-Chang}.
\newblock {\color{blue}Joint Transaction Transmission and Channel Selection in
  Cognitive Radio Based Blockchain Networks: A Deep Reinforcement Learning
  Approach}.
\newblock {\em {\color{blue}arXiv preprint arXiv:1810.10139}},
  {\color{blue}2018}.

\bibitem{li2017intelligent2}
{\color{blue}Li, Xingjian and Fang, Jun and Cheng, Wen and Duan, Huiping and
  Chen, Zhi and Li, Hongbin}.
\newblock {\color{blue}Intelligent Power Control for Spectrum Sharing in
  Cognitive Radios: A Deep Reinforcement Learning Approach}.
\newblock {\em {\color{blue}IEEE access}}, {\color{blue}2018}.

\bibitem{lee2018deep}
{\color{blue}Lee, Woongsup and Kim, Minhoe and Cho, Dong-Ho}.
\newblock {\color{blue}Deep Learning Based Transmit Power Control in Underlaid
  Device-to-Device Communication}.
\newblock {\em {\color{blue}IEEE Systems Journal}}, {\color{blue}2018}.

\bibitem{liu2018energy}
{\color{blue}Liu, Chi Harold and Chen, Zheyu and Tang, Jian and Xu, Jie and
  Piao, Chengzhe}.
\newblock {\color{blue}Energy-efficient {UAV} control for effective and fair
  communication coverage: A deep reinforcement learning approach}.
\newblock {\em {\color{blue}IEEE Journal on Selected Areas in Communications}},
  {\color{blue}36}({\color{blue}9}):{\color{blue}2059--2070},
  {\color{blue}2018}.

\bibitem{he2017software}
{\color{blue}He, Ying and Yu, F Richard and Zhao, Nan and Leung, Victor CM and
  Yin, Hongxi}.
\newblock {\color{blue}Software-defined networks with mobile edge computing and
  caching for smart cities: A big data deep reinforcement learning approach}.
\newblock {\em {\color{blue}IEEE Communications Magazine}},
  {\color{blue}55}({\color{blue}12}):{\color{blue}31--37}, {\color{blue}2017}.

\bibitem{liu2018anti}
{\color{blue}Liu, Xin and Xu, Yuhua and Jia, Luliang and Wu, Qihui and
  Anpalagan, Alagan}.
\newblock {\color{blue}Anti-jamming Communications Using Spectrum Waterfall: A
  Deep Reinforcement Learning Approach}.
\newblock {\em {\color{blue}IEEE Communications Letters}},
  {\color{blue}22}({\color{blue}5}):{\color{blue}998--1001},
  {\color{blue}2018}.

\bibitem{pham2018deep}
{\color{blue}Pham, Quang Tran Anh and Hadjadj-Aoul, Yassine and Outtagarts,
  Abdelkader}.
\newblock {\color{blue}Deep Reinforcement Learning based {QoS}-aware Routing in
  Knowledge-defined networking}.
\newblock In {\em {\color{blue}Qshine EAI International Conference on
  Heterogeneous Networking for Quality, Reliability, Security and Robustness}},
  pages~{\color{blue}1--13}, {\color{blue}2018}.

\bibitem{ferreira2016multi}
{\color{blue}Ferreira, Paulo and Paffenroth, Randy and Wyglinski, Alexander and
  Hackett, Timothy M and Bil{\'e}n, Sven and Reinhart, Richard and Mortensen,
  Dale}.
\newblock {\color{blue}Multi-Objective Reinforcement Learning for Cognitive
  Radio--Based Satellite Communications}.
\newblock In {\em {\color{blue}34th AIAA International Communications Satellite
  Systems Conference}}, page~{\color{blue}5726}, {\color{blue}2016}.

\bibitem{yousefi2017autoencoder}
Mahmood Yousefi-Azar, Vijay Varadharajan, Len Hamey, and Uday Tupakula.
\newblock Autoencoder-based feature learning for cyber security applications.
\newblock In {\em IEEE International Joint Conference on Neural Networks
  (IJCNN)}, pages 3854--3861, 2017.

\bibitem{aminanto2016detecting}
Muhamad~Erza Aminanto and Kwangjo Kim.
\newblock Detecting impersonation attack in {WiFi} networks using deep learning
  approach.
\newblock In {\em International Workshop on Information Security Applications},
  pages 136--147. Springer, 2016.

\bibitem{feng2016anomaly}
Qingsong Feng, Zheng Dou, Chunmei Li, and Guangzhen Si.
\newblock Anomaly detection of spectrum in wireless communication via deep
  autoencoder.
\newblock In {\em International Conference on Computer Science and its
  Applications}, pages 259--265. Springer, 2016.

\bibitem{khan2016distributed}
Muhammad~Altaf Khan, Shafiullah Khan, Bilal Shams, and Jaime Lloret.
\newblock Distributed flood attack detection mechanism using artificial neural
  network in wireless mesh networks.
\newblock {\em Security and Communication Networks}, 9(15):2715--2729, 2016.

\bibitem{diro2017distributed}
Abebe~Abeshu Diro and Naveen Chilamkurti.
\newblock Distributed attack detection scheme using deep learning approach for
  {Internet of Things}.
\newblock {\em Future Generation Computer Systems}, 2017.

\bibitem{saied2016detection}
Alan Saied, Richard~E Overill, and Tomasz Radzik.
\newblock Detection of known and unknown {DDoS} attacks using artificial neural
  networks.
\newblock {\em Neurocomputing}, 172:385--393, 2016.

\bibitem{lopez2017conditional}
Manuel Lopez-Martin, Belen Carro, Antonio Sanchez-Esguevillas, and Jaime
  Lloret.
\newblock Conditional variational autoencoder for prediction and feature
  recovery applied to intrusion detection in {IoT}.
\newblock {\em Sensors}, 17(9):1967, 2017.

\bibitem{hamedani2018reservoir}
\color{black}{Hamedani, Kian and Liu, Lingjia and Atat, Rachad and Wu, Jinsong
  and Yi, Yang}.
\newblock Reservoir computing meets smart grids: attack detection using delayed
  feedback networks.
\newblock {\em IEEE Transactions on Industrial Informatics}, 14(2):734--743,
  2018\color{black}.

\bibitem{das2018deep}
\color{black}{Das, Rajshekhar and Gadre, Akshay and Zhang, Shanghang and Kumar,
  Swarun and Moura, Jose MF}.
\newblock A deep learning approach to {IoT} authentication.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{jiang2018virtual}
\color{black}{Jiang, Peng and Wu, Hongyi and Wang, Cong and Xin, Chunsheng}.
\newblock Virtual {MAC} spoofing detection through deep learning.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{yuan2014droid}
Zhenlong Yuan, Yongqiang Lu, Zhaoguo Wang, and Yibo Xue.
\newblock {Droid-Sec}: deep learning in {Android} malware detection.
\newblock In {\em ACM SIGCOMM Computer Communication Review}, volume~44, pages
  371--372, 2014.

\bibitem{yuan2016droiddetector}
Zhenlong Yuan, Yongqiang Lu, and Yibo Xue.
\newblock Droiddetector: {Android} malware characterization and detection using
  deep learning.
\newblock {\em Tsinghua Science and Technology}, 21(1):114--123, 2016.

\bibitem{su2016deep}
Xin Su, Dafang Zhang, Wenjia Li, and Kai Zhao.
\newblock A deep learning approach to {Android} malware feature learning and
  detection.
\newblock In {\em IEEE Trustcom/BigDataSE/ISPA}, pages 244--251, 2016.

\bibitem{hou2016deep4maldroid}
Shifu Hou, Aaron Saas, Lifei Chen, and Yanfang Ye.
\newblock {Deep4MalDroid}: A deep learning framework for {Android} malware
  detection based on linux kernel system call graphs.
\newblock In {\em IEEE/WIC/ACM International Conference on Web Intelligence
  Workshops (WIW)}, pages 104--111, 2016.

\bibitem{martinelli2017evaluating}
Fabio Martinelli, Fiammetta Marulli, and Francesco Mercaldo.
\newblock Evaluating convolutional neural network for effective mobile malware
  detection.
\newblock {\em Procedia Computer Science}, 112:2372--2381, 2017.

\bibitem{nguyen2018cyberattack}
{\color{blue}Nguyen, Khoi Khac and Hoang, Dinh Thai and Niyato, Dusit and Wang,
  Ping and Nguyen, Diep and Dutkiewicz, Eryk}.
\newblock {\color{blue}Cyberattack detection in mobile cloud computing: A deep
  learning approach}.
\newblock In {\em {\color{blue}IEEE Wireless Communications and Networking
  Conference (WCNC)}}, pages~{\color{blue}1--6}, {\color{blue}2018}.

\bibitem{mclaughlin2017deep}
Niall McLaughlin, Jesus Martinez~del Rincon, BooJoong Kang, Suleiman Yerima,
  Paul Miller, Sakir Sezer, Yeganeh Safaei, Erik Trickel, Ziming Zhao, Adam
  Doup{\'e}, et~al.
\newblock Deep android malware detection.
\newblock In {\em Proceedings of the Seventh ACM on Conference on Data and
  Application Security and Privacy}, pages 301--308, 2017.

\bibitem{chen2017deep123}
Yuanfang Chen, Yan Zhang, and Sabita Maharjan.
\newblock Deep learning for secure mobile edge computing.
\newblock {\em arXiv preprint arXiv:1709.08025}, 2017.

\bibitem{oulehla2016detection}
Milan Oulehla, Zuzana~Kom{\'\i}nkov{\'a} Oplatkov{\'a}, and David Malanik.
\newblock Detection of mobile botnets using neural networks.
\newblock In {\em IEEE Future Technologies Conference (FTC)}, pages 1324--1326,
  2016.

\bibitem{torres2016analysis}
Pablo Torres, Carlos Catania, Sebastian Garcia, and Carlos~Garcia Garino.
\newblock An analysis of recurrent neural networks for botnet detection
  behavior.
\newblock In {\em IEEE Biennial Congress of Argentina (ARGENCON)}, pages 1--6,
  2016.

\bibitem{eslahi2016mobile}
Meisam Eslahi, Moslem Yousefi, Maryam~Var Naseri, YM~Yussof, NM~Tahir, and
  H~Hashim.
\newblock Mobile botnet detection model based on retrospective pattern
  recognition.
\newblock {\em International Journal of Security and Its Applications},
  10(9):39--+, 2016.

\bibitem{alauthaman2016p2p}
Mohammad Alauthaman, Nauman Aslam, Li~Zhang, Rafe Alasem, and MA~Hossain.
\newblock A p2p botnet detection scheme based on decision tree and adaptive
  multilayer neural networks.
\newblock {\em Neural Computing and Applications}, pages 1--14, 2016.

\bibitem{shokri2015privacy}
Reza Shokri and Vitaly Shmatikov.
\newblock Privacy-preserving deep learning.
\newblock In {\em Proceedings of the 22nd ACM SIGSAC conference on computer and
  communications security}, pages 1310--1321, 2015.

\bibitem{aono2017privacy}
Yoshinori Aono, Takuya Hayashi, Lihua Wang, Shiho Moriai, et~al.
\newblock Privacy-preserving deep learning: Revisited and enhanced.
\newblock In {\em International Conference on Applications and Techniques in
  Information Security}, pages 100--110. Springer, 2017.

\bibitem{ossia2017hybrid}
Seyed~Ali Ossia, Ali~Shahin Shamsabadi, Ali Taheri, Hamid~R Rabiee, Nic Lane,
  and Hamed Haddadi.
\newblock A hybrid deep learning architecture for privacy-preserving mobile
  analytics.
\newblock {\em arXiv preprint arXiv:1703.02952}, 2017.

\bibitem{abadi2016deep}
Mart{\'\i}n Abadi, Andy Chu, Ian Goodfellow, H~Brendan McMahan, Ilya Mironov,
  Kunal Talwar, and Li~Zhang.
\newblock Deep learning with differential privacy.
\newblock In {\em Proceedings of the ACM SIGSAC Conference on Computer and
  Communications Security}, pages 308--318. ACM, 2016.

\bibitem{osia2017privacy}
Seyed~Ali Osia, Ali~Shahin Shamsabadi, Ali Taheri, Kleomenis Katevas, Hamed
  Haddadi, and Hamid~R Rabiee.
\newblock Private and scalable personal data analytics using a hybrid
  edge-cloud deep learning.
\newblock {\em IEEE Computer Magazine Special Issue on Mobile and Embedded Deep
  Learning}, 2018.

\bibitem{servia2017personal}
Sandra Servia-Rodriguez, Liang Wang, Jianxin~R Zhao, Richard Mortier, and Hamed
  Haddadi.
\newblock Personal model training under privacy constraints.
\newblock In {\em Proceedings of the 3rd ACM/IEEE International Conference on
  Internet-of-Things Design and Implementation}, Apr 2018.

\bibitem{hitaj2017deep}
Briland Hitaj, Giuseppe Ateniese, and Fernando Perez-Cruz.
\newblock Deep models under the {GAN}: information leakage from collaborative
  deep learning.
\newblock In {\em Proceedings of the ACM SIGSAC Conference on Computer and
  Communications Security}, pages 603--618, 2017.

\bibitem{greydanus2017learning}
Sam Greydanus.
\newblock Learning the enigma with recurrent neural networks.
\newblock {\em arXiv preprint arXiv:1708.07576}, 2017.

\bibitem{maghrebi2016breaking}
Houssem Maghrebi, Thibault Portigliatti, and Emmanuel Prouff.
\newblock Breaking cryptographic implementations using deep learning
  techniques.
\newblock In {\em International Conference on Security, Privacy, and Applied
  Cryptography Engineering}, pages 3--26. Springer, 2016.

\bibitem{liu2018genpass}
\color{black}{Liu, Yunyu and Xia, Zhiyang and Yi, Ping and Yao, Yao and Xie,
  Tiantian and Wang, Wei and Zhu, Ting}.
\newblock G{ENPass}: A general deep learning model for password guessing with
  {PCFG} rules and adversarial generation.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{ning2018deepmag}
{\color{blue}Ning, Rui and Wang, Cong and Xin, ChunSheng and Li, Jiang and Wu,
  Hongyi}.
\newblock {\color{blue}DeepMag: sniffing mobile apps in magnetic field through
  deep convolutional neural networks}.
\newblock In {\em {\color{blue}IEEE International Conference on Pervasive
  Computing and Communications (PerCom)}}, pages~{\color{blue}1--10},
  {\color{blue}2018}.

\bibitem{o2017deep}
Timothy~J O'Shea, Tugba Erpek, and T~Charles Clancy.
\newblock Deep learning based {MIMO} communications.
\newblock {\em arXiv preprint arXiv:1707.07980}, 2017.

\bibitem{borgerding2017amp}
Mark Borgerding, Philip Schniter, and Sundeep Rangan.
\newblock {AMP}-inspired deep networks for sparse linear inverse problems.
\newblock {\em IEEE Transactions on Signal Processing}, 2017.

\bibitem{fujihashi2018nonlinear}
\color{black}{Fujihashi, Takuya and Koike-Akino, Toshiaki and Watanabe, Takashi
  and Orlik, Philip V}.
\newblock Nonlinear equalization with deep learning for multi-purpose visual
  {MIMO} communications.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{rajendran2017distributed}
Sreeraj Rajendran, Wannes Meert, Domenico Giustiniano, Vincent Lenders, and
  Sofie Pollin.
\newblock Deep learning models for wireless signal classification with
  distributed low-cost spectrum sensors.
\newblock {\em IEEE Transactions on Cognitive Communications and Networking},
  2018.

\bibitem{west2017deep}
Nathan~E West and Tim O'Shea.
\newblock Deep architectures for modulation recognition.
\newblock In {\em IEEE International Symposium on Dynamic Spectrum Access
  Networks (DySPAN)}, pages 1--6, 2017.

\bibitem{o2016radio}
Timothy~J O'Shea, Latha Pemula, Dhruv Batra, and T~Charles Clancy.
\newblock Radio transformer networks: Attention models for learning to
  synchronize in wireless systems.
\newblock In {\em 50th Asilomar Conference on Signals, Systems and Computers},
  pages 662--666, 2016.

\bibitem{gante2018beamformed}
{\color{blue}Gante, Jo{\~a}o and Falc{\~a}o, Gabriel and Sousa, Leonel}.
\newblock {\color{blue}Beamformed Fingerprint Learning for Accurate Millimeter
  Wave Positioning}.
\newblock {\em {\color{blue}arXiv preprint arXiv:1804.04112}},
  {\color{blue}2018}.

\bibitem{alkhateeb2018deep}
{\color{blue}Alkhateeb, Ahmed and Alex, Sam and Varkey, Paul and Li, Ying and
  Qu, Qi and Tujkovic, Djordje}.
\newblock {\color{blue}Deep Learning Coordinated Beamforming for Highly-Mobile
  Millimeter Wave Systems}.
\newblock {\em {\color{blue}IEEE Access}},
  {\color{blue}6}:{\color{blue}37328--37348}, {\color{blue}2018}.

\bibitem{neumann2017deep}
David Neumann, Wolfgang Utschick, and Thomas Wiese.
\newblock Deep channel estimation.
\newblock In {\em Proceedings of 21th International ITG Workshop on Smart
  Antennas}, pages 1--6. VDE, 2017.

\bibitem{samuel2017deep}
Neev Samuel, Tzvi Diskin, and Ami Wiesel.
\newblock Deep {MIMO} detection.
\newblock {\em arXiv preprint arXiv:1706.01151}, 2017.

\bibitem{yan2017signal}
Xin Yan, Fei Long, Jingshuai Wang, Na~Fu, Weihua Ou, and Bin Liu.
\newblock Signal detection of {MIMO-OFDM} system based on auto encoder and
  extreme learning machine.
\newblock In {\em IEEE International Joint Conference on Neural Networks
  (IJCNN)}, pages 1602--1606, 2017.

\bibitem{timothy2017introduction}
Timothy O'Shea and Jakob Hoydis.
\newblock An introduction to deep learning for the physical layer.
\newblock {\em IEEE Transactions on Cognitive Communications and Networking},
  3(4):563--575, 2017.

\bibitem{jagannath2018artificial}
\color{black}{Jagannath, Jithin and Polosky, Nicholas and O'Connor, Daniel and
  Theagarajan, Lakshmi N and Sheaffer, Brendan and Foulke, Svetlana and
  Varshney, Pramod K}.
\newblock Artificial neural network based automatic modulation classification
  over a software defined radio testbed.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{o2016end}
Timothy~J O'Shea, Seth Hitefield, and Johnathan Corgan.
\newblock End-to-end radio traffic sequence recognition with recurrent neural
  networks.
\newblock In {\em IEEE Global Conference on Signal and Information Processing
  (GlobalSIP)}, pages 277--281, 2016.

\bibitem{o2016learning}
Timothy~J O'Shea, Kiran Karra, and T~Charles Clancy.
\newblock Learning to communicate: Channel auto-encoders, domain specific
  regularizers, and attention.
\newblock In {\em IEEE International Symposium on Signal Processing and
  Information Technology (ISSPIT)}, pages 223--228, 2016.

\bibitem{ye2018power}
\color{black}{Ye, Hao and Li, Geoffrey Ye and Juang, Biing-Hwang}.
\newblock Power of deep learning for channel estimation and signal detection in
  {OFDM} systems.
\newblock {\em IEEE Wireless Communications Letters}, 7(1):114--117,
  2018\color{black}.

\bibitem{liang2018exploiting}
\color{black}{Liang, Fei and Shen, Cong and Wu, Feng}.
\newblock Exploiting noise correlation for channel decoding with convolutional
  neural networks.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{lyu2018performance}
\color{black}{Lyu, Wei and Zhang, Zhaoyang and Jiao, Chunxu and Qin, Kangjian
  and Zhang, Huazi}.
\newblock Performance evaluation of channel decoding with deep neural networks.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{dorner2017deep}
Sebastian Dorner, Sebastian Cammerer, Jakob Hoydis, and Stephan ten Brink.
\newblock On deep learning-based communication over the air.
\newblock In {\em 51st IEEE Asilomar Conference on Signals, Systems, and
  Computers}, pages 1791--1795, 2017.

\bibitem{liao2018rayleigh}
{\color{blue}Liao, Run-Fa and Wen, Hong and Wu, Jinsong and Song, Huanhuan and
  Pan, Fei and Dong, Lian}.
\newblock {\color{blue}The Rayleigh Fading Channel Prediction via Deep
  Learning}.
\newblock {\em {\color{blue}Wireless Communications and Mobile Computing}},
  {\color{blue}2018}.

\bibitem{huang2018deep}
{\color{blue}Huang, Hongji and Yang, Jie and Song, Yiwei and Huang, Hao and
  Gui, Guan}.
\newblock {\color{blue}Deep Learning for Super-Resolution Channel Estimation
  and {DOA} Estimation based Massive {MIMO} System}.
\newblock {\em {\color{blue}IEEE Transactions on Vehicular Technology}},
  {\color{blue}2018}.

\bibitem{huang2018fully}
{\color{blue}Huang, Sihao and Lin, Haowen}.
\newblock {\color{blue}{Fully optical spacecraft communications: implementing
  an omnidirectional PV-cell receiver and 8 Mb/s LED visible light downlink
  with deep learning error correction}}.
\newblock {\em {\color{blue}IEEE Aerospace and Electronic Systems Magazine}},
  {\color{blue}33}({\color{blue}4}):{\color{blue}16--22}, {\color{blue}2018}.

\bibitem{qian2018wireless}
{\color{blue}Qian, Yuchen and Xing, Yuan and Dong, Liang}.
\newblock {\color{blue}Wireless transmission design with neural network for
  radio-frequency energy harvesting}.
\newblock In {\em {\color{blue}IEEE Wireless Communications and Networking
  Conference (WCNC)}}, pages~{\color{blue}1--6}, {\color{blue}2018}.

\bibitem{gonzalez2017network}
Roberto Gonzalez, Alberto Garcia-Duran, Filipe Manco, Mathias Niepert, and
  Pelayo Vallina.
\newblock Network data monetization using {Net2Vec}.
\newblock In {\em Proceedings of the ACM SIGCOMM Posters and Demos}, pages
  37--39, 2017.

\bibitem{kaminski2017neural}
Nichoas Kaminski, Irene Macaluso, Emanuele Di~Pascale, Avishek Nag, John Brady,
  Mark Kelly, Keith Nolan, Wael Guibene, and Linda Doyle.
\newblock A neural-network-based realization of in-network computation for the
  {Internet of Things}.
\newblock In {\em 2017 IEEE International Conference on Communications (ICC)},
  pages 1--6.

\bibitem{xiao2017secure}
Liang Xiao, Yanda Li, Guoan Han, Huaiyu Dai, and H~Vincent Poor.
\newblock A secure mobile crowdsensing game with deep reinforcement learning.
\newblock {\em IEEE Transactions on Information Forensics and Security}, 2017.

\bibitem{luong2018optimal}
\color{black}{Luong, Nguyen Cong and Xiong, Zehui and Wang, Ping and Niyato,
  Dusit}.
\newblock Optimal auction for edge computing resource management in mobile
  blockchain networks: A deep learning approach.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{gulati2018deep}
\color{black}{Gulati, Amuleen and Aujla, Gagangeet Singh and Chaudhary, Rajat
  and Kumar, Neeraj and Obaidat, Mohammad S}.
\newblock Deep learning-based content centric data dissemination scheme for
  {Internet of Vehicles}.
\newblock In {\em IEEE International Conference on Communications (ICC)}, pages
  1--6, 2018\color{black}.

\bibitem{tsai2018caching}
{\color{blue}Tsai, Kuo Chun and Wang, Li Liliane and Han, Zhu}.
\newblock {\color{blue}Caching for Mobile Social Networks with Deep Learning:
  {Twitter} Analysis for 2016 {U.S.} Election}.
\newblock {\em {\color{blue}IEEE Transactions on Network Science and
  Engineering}}, {\color{blue}2018}.

\bibitem{ahmed2018recent}
{\color{blue}Ahmed, Ejaz and Yaqoob, Ibrar and Hashem, Ibrahim Abaker Targio
  and Shuja, Junaid and Imran, Muhammad and Guizani, Nadra and Bakhsh, Sheikh
  Tahir}.
\newblock {\color{blue}Recent Advances and Challenges in Mobile Big Data}.
\newblock {\em {\color{blue}IEEE Communications Magazine}},
  {\color{blue}56}({\color{blue}2}):{\color{blue}102--108}, {\color{blue}2018}.

\bibitem{yazti2014mobile}
Demetrios~Zeinalipour Yazti and Shonali Krishnaswamy.
\newblock Mobile big data analytics: research, practice, and opportunities.
\newblock In {\em 15th IEEE International Conference on Mobile Data Management
  (MDM)}, volume~1, pages 1--2, 2014.

\bibitem{naboulsi2016large}
Diala Naboulsi, Marco Fiore, Stephane Ribot, and Razvan Stanica.
\newblock Large-scale mobile traffic analysis: a survey.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 18(1):124--161, 2016.

\bibitem{ngiam2011multimodal}
Jiquan Ngiam, Aditya Khosla, Mingyu Kim, Juhan Nam, Honglak Lee, and Andrew~Y
  Ng.
\newblock Multimodal deep learning.
\newblock In {\em Proceedings of the 28th international conference on machine
  learning (ICML)}, pages 689--696, 2011.

\bibitem{alawe2018improving}
{\color{blue}Alawe, Imad and Ksentini, Adlen and Hadjadj-Aoul, Yassine and
  Bertin, Philippe}.
\newblock {\color{blue}Improving traffic forecasting for {5G} core network
  scalability: A Machine Learning approach}.
\newblock {\em {\color{blue}IEEE Network}},
  {\color{blue}32}({\color{blue}6}):{\color{blue}42--49}, {\color{blue}2018}.

\bibitem{aceto2018mobile}
\color{black}{Aceto, Giuseppe and Ciuonzo, Domenico and Montieri, Antonio and
  Pescap{\'e}, Antonio}.
\newblock Mobile encrypted traffic classification using deep learning.
\newblock In {\em 2nd IEEE Network Traffic Measurement and Analysis
  Conference}, 2018\color{black}.

\bibitem{al2015internet}
Ala Al-Fuqaha, Mohsen Guizani, Mehdi Mohammadi, Mohammed Aledhari, and Moussa
  Ayyash.
\newblock Internet of things: A survey on enabling technologies, protocols, and
  applications.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 17(4):2347--2376,
  2015.

\bibitem{seneviratne2017survey}
Suranga Seneviratne, Yining Hu, Tham Nguyen, Guohao Lan, Sara Khalifa, Kanchana
  Thilakarathna, Mahbub Hassan, and Aruna Seneviratne.
\newblock A survey of wearable devices and challenges.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 19(4):2573--2620,
  2017.

\bibitem{li2018learning}
He~Li, Kaoru Ota, and Mianxiong Dong.
\newblock Learning {IoT} in edge: Deep learning for the {Internet of Things}
  with edge computing.
\newblock {\em IEEE Network}, 32(1):96--101, 2018.

\bibitem{lane2015early}
Nicholas~D Lane, Sourav Bhattacharya, Petko Georgiev, Claudio Forlivesi, and
  Fahim Kawsar.
\newblock An early resource characterization of deep learning on wearables,
  smartphones and internet-of-things devices.
\newblock In {\em Proceedings of the ACM International Workshop on Internet of
  Things towards Applications}, pages 7--12, 2015.

\bibitem{ravi2017deep}
Daniele Rav{\`\i}, Charence Wong, Fani Deligianni, Melissa Berthelot, Javier
  Andreu-Perez, Benny Lo, and Guang-Zhong Yang.
\newblock Deep learning for health informatics.
\newblock {\em IEEE journal of biomedical and health informatics}, 21(1):4--21,
  2017.

\bibitem{miotto2017deep}
Riccardo Miotto, Fei Wang, Shuang Wang, Xiaoqian Jiang, and Joel~T Dudley.
\newblock Deep learning for healthcare: review, opportunities and challenges.
\newblock {\em Briefings in Bioinformatics}, 2017.

\bibitem{ronao2016human}
Charissa~Ann Ronao and Sung-Bae Cho.
\newblock Human activity recognition with smartphone sensors using deep
  learning neural networks.
\newblock {\em Expert Systems with Applications}, 59:235--244, 2016.

\bibitem{wang2017deep}
Jindong Wang, Yiqiang Chen, Shuji Hao, Xiaohui Peng, and Lisha Hu.
\newblock Deep learning for sensor-based activity recognition: A survey.
\newblock {\em Pattern Recognition Letters}, 2018.

\bibitem{ran2017delivering}
Xukan Ran, Haoliang Chen, Zhenming Liu, and Jiasi Chen.
\newblock Delivering deep learning to mobile devices via offloading.
\newblock In {\em Proceedings of the ACM Workshop on Virtual Reality and
  Augmented Reality Network}, pages 42--47, 2017.

\bibitem{vyas2017survey}
Vishakha~V Vyas, KH~Walse, and RV~Dharaskar.
\newblock A survey on human activity recognition using smartphone.
\newblock {\em International Journal}, 5(3), 2017.

\bibitem{zen2014deep}
Heiga Zen and Andrew Senior.
\newblock Deep mixture density networks for acoustic modeling in statistical
  parametric speech synthesis.
\newblock In {\em IEEE International Conference on Acoustics, Speech and Signal
  Processing (ICASSP)}, pages 3844--3848, 2014.

\bibitem{zhao2016urban}
Kai Zhao, Sasu Tarkoma, Siyuan Liu, and Huy Vo.
\newblock Urban human mobility data mining: An overview.
\newblock In {\em IEEE International Conference on Big Data (Big Data)}, pages
  1911--1920, 2016.

\bibitem{yang2017neural2}
Cheng Yang, Maosong Sun, Wayne~Xin Zhao, Zhiyuan Liu, and Edward~Y Chang.
\newblock A neural network approach to jointly modeling social networks and
  mobile trajectories.
\newblock {\em ACM Transactions on Information Systems (TOIS)}, 35(4):36, 2017.

\bibitem{graves2014neural}
{\color{blue}Graves, Alex and Wayne, Greg and Danihelka, Ivo}.
\newblock {\color{blue}Neural turing machines}.
\newblock {\em {\color{blue}arXiv preprint arXiv:1410.5401}},
  {\color{blue}2014}.

\bibitem{xia2017indoor}
Shixiong Xia, Yi~Liu, Guan Yuan, Mingjun Zhu, and Zhaohui Wang.
\newblock Indoor fingerprint positioning based on {Wi-Fi}: An overview.
\newblock {\em ISPRS International Journal of Geo-Information}, 6(5):135, 2017.

\bibitem{davidson2016survey}
Pavel Davidson and Robert Pich{\'e}.
\newblock A survey of selected indoor positioning methods for smartphones.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 19(2):1347--1370,
  2017.

\bibitem{xiao2012fifs}
Jiang Xiao, Kaishun Wu, Youwen Yi, and Lionel~M Ni.
\newblock {FIFS}: Fine-grained indoor fingerprinting system.
\newblock In {\em 21st International Conference on Computer Communications and
  Networks (ICCCN)}, pages 1--7, 2012.

\bibitem{youssef2005horus}
Moustafa Youssef and Ashok Agrawala.
\newblock The {H}orus {WLAN} location determination system.
\newblock In {\em Proceedings of the 3rd ACM international conference on Mobile
  systems, applications, and services}, pages 205--218, 2005.

\bibitem{brunato2005statistical}
Mauro Brunato and Roberto Battiti.
\newblock Statistical learning theory for location fingerprinting in wireless
  {LANs}.
\newblock {\em Computer Networks}, 47(6):825--845, 2005.

\bibitem{ho2016generative}
Jonathan Ho and Stefano Ermon.
\newblock Generative adversarial imitation learning.
\newblock In {\em Advances in Neural Information Processing Systems}, pages
  4565--4573, 2016.

\bibitem{zorzi2016cobanets}
Michele Zorzi, Andrea Zanella, Alberto Testolin, Michele De~Filippo De~Grazia,
  and Marco Zorzi.
\newblock {COBANETS}: A new paradigm for cognitive communications systems.
\newblock In {\em IEEE International Conference on Computing, Networking and
  Communications (ICNC)}, pages 1--7, 2016.

\bibitem{roopaei2017deep}
Mehdi Roopaei, Paul Rad, and Mo~Jamshidi.
\newblock Deep learning control for complex and large scale cloud systems.
\newblock {\em Intelligent Automation \& Soft Computing}, pages 1--3, 2017.

\bibitem{ferreira2018multi}
{\color{blue}Ferreira, Paulo Victor R and Paffenroth, Randy and Wyglinski,
  Alexander M and Hackett, Timothy M and Bil{\'e}n, Sven G and Reinhart,
  Richard C and Mortensen, Dale J}.
\newblock {\color{blue}Multi-objective Reinforcement Learning for Cognitive
  Satellite Communications using Deep Neural Network Ensembles}.
\newblock {\em {\color{blue}IEEE Journal on Selected Areas in Communications}},
  {\color{blue}2018}.

\bibitem{schaul2015prioritized}
Tom Schaul, John Quan, Ioannis Antonoglou, and David Silver.
\newblock Prioritized experience replay.
\newblock {\em International Conference on Learning Representations (ICLR)},
  2016.

\bibitem{shi2011iteratively}
Qingjiang Shi, Meisam Razaviyayn, Zhi-Quan Luo, and Chen He.
\newblock An iteratively weighted {MMSE} approach to distributed sum-utility
  maximization for a {MIMO} interfering broadcast channel.
\newblock {\em IEEE Transactions on Signal Processing}, 59(9):4331--4340, 2011.

\bibitem{buczak2016survey}
Anna~L Buczak and Erhan Guven.
\newblock A survey of data mining and machine learning methods for cyber
  security intrusion detection.
\newblock {\em IEEE Communications Surveys \& Tutorials}, 18(2):1153--1176,
  2016.

\bibitem{wang2018not}
{\color{blue}Wang, Ji and Zhang, Jianguo and Bao, Weidong and Zhu, Xiaomin and
  Cao, Bokai and Yu, Philip S}.
\newblock {\color{blue}Not just privacy: Improving performance of private deep
  learning in mobile cloud}.
\newblock In {\em {\color{blue}Proceedings of the 24th ACM SIGKDD International
  Conference on Knowledge Discovery \& Data Mining}},
  pages~{\color{blue}2407--2416}, {\color{blue}2018}.

\bibitem{kwon2017survey}
Donghwoon Kwon, Hyunjoo Kim, Jinoh Kim, Sang~C Suh, Ikkyun Kim, and Kuinam~J
  Kim.
\newblock A survey of deep learning-based network anomaly detection.
\newblock {\em Cluster Computing}, pages 1--13, 2017.

\bibitem{tavallaee2009detailed}
Mahbod Tavallaee, Ebrahim Bagheri, Wei Lu, and Ali~A Ghorbani.
\newblock A detailed analysis of the kdd cup 99 data set.
\newblock In {\em Computational Intelligence for Security and Defense
  Applications, 2009. CISDA 2009. IEEE Symposium on}, pages 1--6, 2009.

\bibitem{tam2017evolution}
Kimberly Tam, Ali Feizollah, Nor~Badrul Anuar, Rosli Salleh, and Lorenzo
  Cavallaro.
\newblock The evolution of android malware and {Android} analysis techniques.
\newblock {\em ACM Computing Surveys (CSUR)}, 49(4):76, 2017.

\bibitem{rodriguez2013survey}
Rafael~A Rodr{\'\i}guez-G{\'o}mez, Gabriel Maci{\'a}-Fern{\'a}ndez, and Pedro
  Garc{\'\i}a-Teodoro.
\newblock Survey and taxonomy of botnet research through life-cycle.
\newblock {\em ACM Computing Surveys (CSUR)}, 45(4):45, 2013.

\bibitem{liu2016collaborative}
Menghan Liu, Haotian Jiang, Jia Chen, Alaa Badokhon, Xuetao Wei, and Ming-Chun
  Huang.
\newblock A collaborative privacy-preserving deep learning system in
  distributed mobile environment.
\newblock In {\em IEEE International Conference on Computational Science and
  Computational Intelligence (CSCI)}, pages 192--197, 2016.

\bibitem{chopra2005learning}
Sumit Chopra, Raia Hadsell, and Yann LeCun.
\newblock Learning a similarity metric discriminatively, with application to
  face verification.
\newblock In {\em IEEE Conference on Computer Vision and Pattern Recognition
  (CVPR)}, volume~1, pages 539--546, 2005.

\bibitem{shamsabadi2018}
Ali~Shahin Shamsabadi, Hamed Haddadi, and Andrea Cavallaro.
\newblock Distributed one-class learning.
\newblock In {\em IEEE International Conference on Image Processing (ICIP)},
  2018.

\bibitem{hitaj2017passgan}
Briland Hitaj, Paolo Gasti, Giuseppe Ateniese, and Fernando Perez-Cruz.
\newblock Pass{GAN}: A deep learning approach for password guessing.
\newblock {\em arXiv preprint arXiv:1709.00440}, 2017.

\bibitem{ye2018channel}
{\color{blue}Ye, Hao and Li, Geoffrey Ye and Juang, Biing-Hwang Fred and
  Sivanesan, Kathiravetpillai}.
\newblock {\color{blue}Channel agnostic end-to-end learning based communication
  systems with conditional {GAN}}.
\newblock {\em {\color{blue}arXiv preprint arXiv:1807.00447}},
  {\color{blue}2018}.

\bibitem{gonzalez2017net2vec}
Roberto Gonzalez, Filipe Manco, Alberto Garcia-Duran, Jose Mendes, Felipe
  Huici, Saverio Niccolini, and Mathias Niepert.
\newblock {Net2Vec}: Deep learning for the network.
\newblock In {\em Proceedings of the ACM Workshop on Big Data Analytics and
  Machine Learning for Data Communication Networks}, pages 13--18, 2017.

\bibitem{wolpert1997no}
David~H Wolpert and William~G Macready.
\newblock No free lunch theorems for optimization.
\newblock {\em IEEE transactions on evolutionary computation}, 1(1):67--82,
  1997.

\bibitem{cheng2017survey}
Yu~Cheng, Duo Wang, Pan Zhou, and Tao Zhang.
\newblock Model compression and acceleration for deep neural networks: The
  principles, progress, and challenges.
\newblock {\em IEEE Signal Processing Magazine}, 35(1):126--136, 2018.

\bibitem{lane2017squeezing}
Nicholas~D Lane, Sourav Bhattacharya, Akhil Mathur, Petko Georgiev, Claudio
  Forlivesi, and Fahim Kawsar.
\newblock Squeezing deep learning into mobile and embedded devices.
\newblock {\em IEEE Pervasive Computing}, 16(3):82--88, 2017.

\bibitem{tang2017enabling}
Jie Tang, Dawei Sun, Shaoshan Liu, and Jean-Luc Gaudiot.
\newblock Enabling deep learning on {IoT} devices.
\newblock {\em Computer}, 50(10):92--96, 2017.

\bibitem{wang2018deep}
{\color{blue}Wang, Ji and Cao, Bokai and Yu, Philip and Sun, Lichao and Bao,
  Weidong and Zhu, Xiaomin}.
\newblock {\color{blue}Deep learning towards mobile applications}.
\newblock In {\em {\color{blue}38th IEEE International Conference on
  Distributed Computing Systems (ICDCS)}}, pages~{\color{blue}1385--1393},
  {\color{blue}2018}.

\bibitem{iandola2017squeezenet}
Forrest~N Iandola, Song Han, Matthew~W Moskewicz, Khalid Ashraf, William~J
  Dally, and Kurt Keutzer.
\newblock {SqueezeNet}: {AlexNet}-level accuracy with 50x fewer parameters and<
  0.5 {MB} model size.
\newblock {\em International Conference on Learning Representations (ICLR)},
  2017.

\bibitem{howard2017mobilenets}
Andrew~G Howard, Menglong Zhu, Bo~Chen, Dmitry Kalenichenko, Weijun Wang,
  Tobias Weyand, Marco Andreetto, and Hartwig Adam.
\newblock Mobilenets: Efficient convolutional neural networks for mobile vision
  applications.
\newblock {\em arXiv preprint arXiv:1704.04861}, 2017.

\bibitem{zhang2017shufflenet}
Xiangyu Zhang, Xinyu Zhou, Mengxiao Lin, and Jian Sun.
\newblock {ShuffleNet}: An extremely efficient convolutional neural network for
  mobile devices.
\newblock In {\em The IEEE Conference on Computer Vision and Pattern
  Recognition (CVPR)}, June 2018.

\bibitem{zhang2017tucker}
Qingchen Zhang, Laurence~T Yang, Xingang Liu, Zhikui Chen, and Peng Li.
\newblock A tucker deep computation model for mobile multimedia feature
  learning.
\newblock {\em ACM Transactions on Multimedia Computing, Communications, and
  Applications (TOMM)}, 13(3s):39, 2017.

\bibitem{cao2017mobirnn}
Qingqing Cao, Niranjan Balasubramanian, and Aruna Balasubramanian.
\newblock {MobiRNN}: Efficient recurrent neural network execution on mobile
  {GPU}.
\newblock In {\em Proceedings of the 1st ACM International Workshop on Deep
  Learning for Mobile Systems and Applications}, pages 1--6, 2017.

\bibitem{chen2016deep}
Chun-Fu Chen, Gwo~Giun Lee, Vincent Sritapan, and Ching-Yung Lin.
\newblock Deep convolutional neural network on {iOS} mobile devices.
\newblock In {\em IEEE International Workshop on Signal Processing Systems
  (SiPS)}, pages 130--135, 2016.

\bibitem{rallapalli2016very}
S~Rallapalli, H~Qiu, A~Bency, S~Karthikeyan, R~Govindan, B~Manjunath, and
  R~Urgaonkar.
\newblock Are very deep neural networks feasible on mobile devices.
\newblock {\em IEEE Transactions on Circuits and Systems for Video Technology},
  2016.

\bibitem{lane2016deepx}
Nicholas~D Lane, Sourav Bhattacharya, Petko Georgiev, Claudio Forlivesi, Lei
  Jiao, Lorena Qendro, and Fahim Kawsar.
\newblock {DeepX}: A software accelerator for low-power deep learning inference
  on mobile devices.
\newblock In {\em 15th ACM/IEEE International Conference on Information
  Processing in Sensor Networks (IPSN)}, pages 1--12, 2016.

\bibitem{huynh2017deepmon}
Loc~N Huynh, Rajesh~Krishna Balan, and Youngki Lee.
\newblock {DeepMon}: Building mobile {GPU} deep learning models for continuous
  vision applications.
\newblock In {\em Proceedings of the 15th ACM Annual International Conference
  on Mobile Systems, Applications, and Services}, pages 186--186, 2017.

\bibitem{wu2016quantized}
Jiaxiang Wu, Cong Leng, Yuhang Wang, Qinghao Hu, and Jian Cheng.
\newblock Quantized convolutional neural networks for mobile devices.
\newblock In {\em Proceedings of the IEEE Conference on Computer Vision and
  Pattern Recognition}, pages 4820--4828, 2016.

\bibitem{bhattacharya2016sparsification}
Sourav Bhattacharya and Nicholas~D Lane.
\newblock Sparsification and separation of deep learning layers for constrained
  resource inference on wearables.
\newblock In {\em Proceedings of the 14th ACM Conference on Embedded Network
  Sensor Systems CD-ROM}, pages 176--189, 2016.

\bibitem{cho2017mec}
Minsik Cho and Daniel Brand.
\newblock {MEC}: Memory-efficient convolution for deep neural network.
\newblock In {\em International Conference on Machine Learning (ICML)}, pages
  815--824, 2017.

\bibitem{guo2017pruning}
Jia Guo and Miodrag Potkonjak.
\newblock Pruning filters and classes: Towards on-device customization of
  convolutional neural networks.
\newblock In {\em Proceedings of the 1st ACM International Workshop on Deep
  Learning for Mobile Systems and Applications}, pages 13--17, 2017.

\bibitem{li2017fitcnn}
Shiming Li, Duo Liu, Chaoneng Xiang, Jianfeng Liu, Yingjian Ling, Tianjun Liao,
  and Liang Liang.
\newblock Fitcnn: A cloud-assisted lightweight convolutional neural network
  framework for mobile devices.
\newblock In {\em 23rd IEEE International Conference on Embedded and Real-Time
  Computing Systems and Applications (RTCSA)}, pages 1--6, 2017.

\bibitem{zen2016fast}
Heiga Zen, Yannis Agiomyrgiannakis, Niels Egberts, Fergus Henderson, and
  Przemys{\l}aw Szczepaniak.
\newblock Fast, compact, and high quality {LSTM-RNN} based statistical
  parametric speech synthesizers for mobile devices.
\newblock {\em arXiv preprint arXiv:1606.06061}, 2016.

\bibitem{falcao2017evaluation}
Gabriel Falcao, Lu{\'\i}s~A Alexandre, J~Marques, Xavier Fraz{\~a}o, and Joao
  Maria.
\newblock On the evaluation of energy-efficient deep learning using stacked
  autoencoders on mobile gpus.
\newblock In {\em 25th IEEE Euromicro International Conference on Parallel,
  Distributed and Network-based Processing}, pages 270--273, 2017.

\bibitem{fang2018nestdnn}
{\color{blue}Fang, Biyi and Zeng, Xiao and Zhang, Mi}.
\newblock {\color{blue}{NestDNN}: Resource-Aware Multi-Tenant On-Device Deep
  Learning for Continuous Mobile Vision}.
\newblock In {\em {\color{blue}Proceedings of the 24th ACM Annual International
  Conference on Mobile Computing and Networking}},
  pages~{\color{blue}115--127}, {\color{blue}2018}.

\bibitem{xu2018deepcache}
{\color{blue}Xu, Mengwei and Zhu, Mengze and Liu, Yunxin and Lin, Felix Xiaozhu
  and Liu, Xuanzhe}.
\newblock {\color{blue}{DeepCache}: Principled Cache for Mobile Deep Vision}.
\newblock In {\em {\color{blue}Proceedings of the 24th ACM Annual International
  Conference on Mobile Computing and Networking}},
  pages~{\color{blue}129--144}, {\color{blue}2018}.

\bibitem{liu2018ondemand}
{\color{blue}Liu, Sicong and Lin, Yingyan and Zhou, Zimu and Nan, Kaiming and
  Liu, Hui and Du, Junzhao}.
\newblock {\color{blue}On-Demand Deep Model Compression for Mobile Devices: A
  Usage-Driven Model Selection Framework}.
\newblock In {\em {\color{blue}Proceedings of the 16th ACM Annual International
  Conference on Mobile Systems, Applications, and Services}},
  pages~{\color{blue}389--400}, {\color{blue}2018}.

\bibitem{chen2018tvm}
{\color{blue}Chen, Tianqi and Moreau, Thierry and Jiang, Ziheng and Zheng,
  Lianmin and Yan, Eddie and Shen, Haichen and Cowan, Meghan and Wang, Leyuan
  and Hu, Yuwei and Ceze, Luis and others}.
\newblock {\color{blue}{TVM}: An Automated End-to-End Optimizing Compiler for
  Deep Learning}.
\newblock In {\em {\color{blue}13th USENIX Symposium on Operating Systems
  Design and Implementation (OSDI 18)}}, pages~{\color{blue}578--594},
  {\color{blue}2018}.

\bibitem{yao2018fastdeepiot}
{\color{blue}Yao, Shuochao and Zhao, Yiran and Shao, Huajie and Liu, ShengZhong
  and Liu, Dongxin and Su, Lu and Abdelzaher, Tarek}.
\newblock {\color{blue}{FastDeepIoT}: Towards Understanding and Optimizing
  Neural Network Execution Time on Mobile and Embedded Devices}.
\newblock In {\em {\color{blue}Proceedings of the 16th ACM Conference on
  Embedded Networked Sensor Systems}}, pages~{\color{blue}278--291},
  {\color{blue}2018}.

\bibitem{teerapittayanon2017distributed}
Surat Teerapittayanon, Bradley McDanel, and HT~Kung.
\newblock Distributed deep neural networks over the cloud, the edge and end
  devices.
\newblock In {\em 37th IEEE International Conference on Distributed Computing
  Systems (ICDCS)}, pages 328--339, 2017.

\bibitem{omidshafiei2017deep}
Shayegan Omidshafiei, Jason Pazis, Christopher Amato, Jonathan~P How, and John
  Vian.
\newblock Deep decentralized multi-task multi-agent reinforcement learning
  under partial observability.
\newblock In {\em International Conference on Machine Learning (ICML)}, pages
  2681--2690, 2017.

\bibitem{recht2011hogwild}
Benjamin Recht, Christopher Re, Stephen Wright, and Feng Niu.
\newblock Hogwild: A lock-free approach to parallelizing stochastic gradient
  descent.
\newblock In {\em Advances in neural information processing systems}, pages
  693--701, 2011.

\bibitem{goyal2017accurate}
Priya Goyal, Piotr Doll{\'a}r, Ross Girshick, Pieter Noordhuis, Lukasz
  Wesolowski, Aapo Kyrola, Andrew Tulloch, Yangqing Jia, and Kaiming He.
\newblock Accurate, large {Minibatch SGD}: Training imagenet in 1 hour.
\newblock {\em arXiv preprint arXiv:1706.02677}, 2017.

\bibitem{zhang2016asynchronous}
ShuaiZheng Ruiliang~Zhang and JamesT Kwok.
\newblock Asynchronous distributed semi-stochastic gradient optimization.
\newblock In {\em National Conference on Artificial Intelligence (AAAI)}, 2016.

\bibitem{hardy2017distributed}
Corentin Hardy, Erwan Le~Merrer, and Bruno Sericola.
\newblock Distributed deep learning on edge-devices: feasibility via adaptive
  compression.
\newblock In {\em 16th IEEE International Symposium on Network Computing and
  Applications (NCA)}, pages 1--8, 2017.

\bibitem{pmlr-v54-mcmahan17a}
Brendan McMahan, Eider Moore, Daniel Ramage, Seth Hampson, and Blaise~Aguera
  y~Arcas.
\newblock Communication-efficient learning of deep networks from decentralized
  data.
\newblock In {\em Proceedings of the 20th International Conference on
  Artificial Intelligence and Statistics}, volume~54, pages 1273--1282, Fort
  Lauderdale, FL, USA, 20--22 Apr 2017.

\bibitem{cryptoeprint:2017:281}
Keith Bonawitz, Vladimir Ivanov, Ben Kreuter, Antonio Marcedone, H.~Brendan
  McMahan, Sarvar Patel, Daniel Ramage, Aaron Segal, and Karn Seth.
\newblock Practical secure aggregation for privacy preserving machine learning.
\newblock Cryptology ePrint Archive, Report 2017/281, 2017.
\newblock \url{https://eprint.iacr.org/2017/281}.

\bibitem{gupta2016model}
Suyog Gupta, Wei Zhang, and Fei Wang.
\newblock Model accuracy and runtime tradeoff in distributed deep learning: A
  systematic study.
\newblock In {\em IEEE 16th International Conference on Data Mining (ICDM)},
  pages 171--180, 2016.

\bibitem{mcmahan2017federated}
B~McMahan and Daniel Ramage.
\newblock Federated learning: Collaborative machine learning without
  centralized training data.
\newblock {\em Google Research Blog}, 2017.

\bibitem{furno2017joint}
Angelo Fumo, Marco Fiore, and Razvan Stanica.
\newblock Joint spatial and temporal classification of mobile traffic demands.
\newblock In {\em IEEE Conference on Computer Communications}, pages 1--9,
  2017.

\bibitem{chen2016lifelong}
Zhiyuan Chen and Bing Liu.
\newblock Lifelong machine learning.
\newblock {\em Synthesis Lectures on Artificial Intelligence and Machine
  Learning}, 10(3):1--145, 2016.

\bibitem{lee2016dual}
Sang-Woo Lee, Chung-Yeon Lee, Dong-Hyun Kwak, Jiwon Kim, Jeonghee Kim, and
  Byoung-Tak Zhang.
\newblock Dual-memory deep learning architectures for lifelong learning of
  everyday human behaviors.
\newblock In {\em International Joint Conferences on Artificial Intelligence},
  pages 1669--1675, 2016.

\bibitem{graves2016hybrid}
Alex Graves, Greg Wayne, Malcolm Reynolds, Tim Harley, Ivo Danihelka, Agnieszka
  Grabska-Barwi{\'n}ska, Sergio~G{\'o}mez Colmenarejo, Edward Grefenstette,
  Tiago Ramalho, John Agapiou, et~al.
\newblock Hybrid computing using a neural network with dynamic external memory.
\newblock {\em Nature}, 538(7626):471--476, 2016.

\bibitem{parisi2017lifelong}
German~I Parisi, Jun Tani, Cornelius Weber, and Stefan Wermter.
\newblock Lifelong learning of human actions with deep neural network
  self-organization.
\newblock {\em Neural Networks}, 2017.

\bibitem{tessler2017deep}
Chen Tessler, Shahar Givony, Tom Zahavy, Daniel~J Mankowitz, and Shie Mannor.
\newblock A deep hierarchical approach to lifelong learning in {Minecraft}.
\newblock In {\em National Conference on Artificial Intelligence (AAAI)}, pages
  1553--1561, 2017.

\bibitem{lopez2018deep}
Daniel L{\'o}pez-S{\'a}nchez, Ang{\'e}lica~Gonz{\'a}lez Arrieta, and Juan~M
  Corchado.
\newblock Deep neural networks and transfer learning applied to multimedia web
  mining.
\newblock In {\em 14th International Conference Distributed Computing and
  Artificial Intelligence}, volume 620, page 124. Springer, 2018.

\bibitem{bacstuug2015transfer}
Ejder Ba{\c{s}}tu{\u{g}}, Mehdi Bennis, and M{\'e}rouane Debbah.
\newblock A transfer learning approach for cache-enabled wireless networks.
\newblock In {\em 13th IEEE International Symposium on Modeling and
  Optimization in Mobile, Ad Hoc, and Wireless Networks (WiOpt)}, pages
  161--166, 2015.

\bibitem{fei2006one}
Li~Fei-Fei, Rob Fergus, and Pietro Perona.
\newblock One-shot learning of object categories.
\newblock {\em IEEE transactions on pattern analysis and machine intelligence},
  28(4):594--611, 2006.

\bibitem{palatucci2009zero}
Mark Palatucci, Dean Pomerleau, Geoffrey~E Hinton, and Tom~M Mitchell.
\newblock Zero-shot learning with semantic output codes.
\newblock In {\em Advances in neural information processing systems}, pages
  1410--1418, 2009.

\bibitem{vinyals2016matching}
Oriol Vinyals, Charles Blundell, Tim Lillicrap, Daan Wierstra, et~al.
\newblock Matching networks for one shot learning.
\newblock In {\em Advances in Neural Information Processing Systems}, pages
  3630--3638, 2016.

\bibitem{changpinyo2016synthesized}
Soravit Changpinyo, Wei-Lun Chao, Boqing Gong, and Fei Sha.
\newblock Synthesized classifiers for zero-shot learning.
\newblock In {\em Proceedings of the IEEE Conference on Computer Vision and
  Pattern Recognition}, pages 5327--5336, 2016.

\bibitem{oh2017zero}
Junhyuk Oh, Satinder Singh, Honglak Lee, and Pushmeet Kohli.
\newblock Zero-shot task generalization with multi-task deep reinforcement
  learning.
\newblock In {\em International Conference on Machine Learning (ICML)}, pages
  2661--2670, 2017.

\bibitem{wang2015understanding}
Huandong Wang, Fengli Xu, Yong Li, Pengyu Zhang, and Depeng Jin.
\newblock Understanding mobile traffic patterns of large scale cellular towers
  in urban environment.
\newblock In {\em Proceedings of the ACM Internet Measurement Conference},
  pages 225--238, 2015.

\bibitem{marquez2017apps}
Cristina Marquez, Marco Gramaglia, Marco Fiore, Albert Banchs, Cezary
  Ziemlicki, and Zbigniew Smoreda.
\newblock Not all {Apps} are created equal: Analysis of spatiotemporal
  heterogeneity in nationwide mobile service usage.
\newblock In {\em Proceedings of the 13th ACM Conference on Emerging Networking
  Experiments and Technologies}, 2017.

\bibitem{barlacchi2015multi}
Gianni Barlacchi, Marco De~Nadai, Roberto Larcher, Antonio Casella, Cristiana
  Chitic, Giovanni Torrisi, Fabrizio Antonelli, Alessandro Vespignani, Alex
  Pentland, and Bruno Lepri.
\newblock A multi-source dataset of urban life in the city of {Milan} and the
  province of {Trentino}.
\newblock {\em Scientific data}, 2, 2015.

\bibitem{liu2015urban}
Liang Liu, Wangyang Wei, Dong Zhao, and Huadong Ma.
\newblock Urban resolution: New metric for measuring the quality of urban
  sensing.
\newblock {\em IEEE Transactions on Mobile Computing}, 14(12):2560--2575, 2015.

\bibitem{tikunov2007traffic}
Denis Tikunov and Toshikazu Nishimura.
\newblock Traffic prediction for mobile network using holt-winter's exponential
  smoothing.
\newblock In {\em 15th IEEE International Conference on Software,
  Telecommunications and Computer Networks}, pages 1--5, 2007.

\bibitem{Kim2011}
Hyun-Woo Kim, Jun-Hui Lee, Yong-Hoon Choi, Young-Uk Chung, and Hyukjoon Lee.
\newblock {Dynamic bandwidth provisioning using ARIMA-based traffic forecasting
  for Mobile WiMAX}.
\newblock {\em Computer Communications}, 34(1):99--106, 2011.

\bibitem{charles2017pointnet}
{\color{blue}Charles, R Qi and Su, Hao and Kaichun, Mo and Guibas, Leonidas J}.
\newblock {\color{blue}Pointnet: Deep learning on point sets for {3D}
  classification and segmentation}.
\newblock In {\em {\color{blue}IEEE Conference on Computer Vision and Pattern
  Recognition (CVPR)}}, pages~{\color{blue}77--85}, {\color{blue}2017}.

\bibitem{ioannidou2017deep}
Anastasia Ioannidou, Elisavet Chatzilari, Spiros Nikolopoulos, and Ioannis
  Kompatsiaris.
\newblock Deep learning advances in computer vision with {3D} data: A survey.
\newblock {\em ACM Computing Surveys (CSUR)}, 50(2):20, 2017.

\bibitem{scarselli2009graph}
{\color{blue}Scarselli, Franco and Gori, Marco and Tsoi, Ah Chung and
  Hagenbuchner, Markus and Monfardini, Gabriele}.
\newblock {\color{blue}The graph neural network model}.
\newblock {\em {\color{blue}IEEE Transactions on Neural Networks}},
  {\color{blue}20}({\color{blue}1}):{\color{blue}61--80}, {\color{blue}2009}.

\bibitem{yuan2017temporal}
{\color{blue}Yuan, Yuan and Liang, Xiaodan and Wang, Xiaolong and Yeung,
  Dit-Yan and Gupta, Abhinav}.
\newblock {\color{blue}Temporal Dynamic Graph LSTM for Action-Driven Video
  Object Detection.}
\newblock In {\em {\color{blue}IEEE International Conference on Computer Vision
  (ICCV)}}, pages~{\color{blue}1819--1828}, {\color{blue}2017}.

\bibitem{usama2017unsupervised}
Muhammad Usama, Junaid Qadir, Aunn Raza, Hunain Arif, Kok-Lim~Alvin Yau, Yehia
  Elkhatib, Amir Hussain, and Ala Al-Fuqaha.
\newblock Unsupervised machine learning for networking: Techniques,
  applications and research challenges.
\newblock {\em arXiv preprint arXiv:1709.06599}, 2017.

\bibitem{zhou2017anomaly}
Chong Zhou and Randy~C Paffenroth.
\newblock Anomaly detection with robust deep autoencoders.
\newblock In {\em Proceedings of the 23rd ACM SIGKDD International Conference
  on Knowledge Discovery and Data Mining}, pages 665--674, 2017.

\bibitem{abadi2016learning}
Mart{\'\i}n Abadi and David~G Andersen.
\newblock Learning to protect communications with adversarial neural
  cryptography.
\newblock {\em International Conference on Learning Representations (ICLR)},
  2017.

\bibitem{silver2017mastering}
Silver David, Julian Schrittwieser, Karen Simonyan, Ioannis Antonoglou, Aja
  Huang, Arthur Guez, Thomas Hubert, Lucas Baker, Matthew Lai, Adrian Bolton,
  Yutian Chen, Timothy Lillicrap, Fan Hui, Laurent Sifre, George van~den
  Driessche, Graepel Thore, and Demis Hassabis.
\newblock Mastering the game of {Go} without human knowledge.
\newblock {\em Nature}, 550(7676):354--359, 2017.

\bibitem{Silver1140}
{\color{blue}Silver, David and Hubert, Thomas and Schrittwieser, Julian and
  Antonoglou, Ioannis and Lai, Matthew and Guez, Arthur and Lanctot, Marc and
  Sifre, Laurent and Kumaran, Dharshan and Graepel, Thore and Lillicrap,
  Timothy and Simonyan, Karen and Hassabis, Demis}.
\newblock {\color{blue}A general reinforcement learning algorithm that masters
  chess, shogi, and {Go} through self-play}.
\newblock {\em {\color{blue}Science}},
  {\color{blue}362}({\color{blue}6419}):{\color{blue}1140--1144},
  {\color{blue}2018}.

\end{thebibliography}

